An Improved Model of Nonlinear Fiber Propagation in the Presence of Kerr Nonlinearity and Stimulated Raman Scattering

Ultra-wideband fiber optical transmission suffers from both Kerr nonlinearity and stimulated Raman scattering (SRS). Mathematical models that address the interplay between Kerr nonlinearity and SRS exist. These models are based on the Gaussian-noise (GN) and enhanced Gaussian noise (EGN) models. In this paper, we propose a modulation-format-dependent model, accounting for an enhanced link function, which is valid for non-identical spans where the fiber span loss and SRS gain/loss are not necessarily compensated for by the amplifier at the end of each span. A new signal power profile is also introduced, comprising the frequency-dependent fiber attenuation. The proposed analytical model takes all terms of nonlinear interference (NLI), including self-channel interference, cross-channel interference, and multi-channel interference, into account. It is also shown that the proposed model has the power to predict the NLI power with greater precision than the previous models can. Split-step Fourier simulations indicate that when both SRS and arbitrary modulation formats are considered, previous models may inaccurately predict the NLI power. This difference could be up to 4.3 dB for a 10.011 THz system with 1001 channels at 10 Gbaud.

==> ElasticFigs.tex <==
\begin{figure}
\centering
\definecolor{bluedark}{HTML}{244061}
\begin{tikzpicture}[scale=0.7]  
%\filldraw[fill=pink, draw=blue!20, thick] (1,2.5)--(1,1.8)--(1.8,1) -- (2.5,1)--(2.5,1.8)--(1.8,2.5)--cycle node at (1.5,2) {\scriptsize{COI}};
\def\mypath{(1,2.5)--(1,1.8)--(1.8,1) -- (2.5,1)--(2.5,1.8)--(1.8,2.5)--cycle};
\fill [fill=pink] \mypath;
\node at (1.35,2.2) {\scriptsize{SCI}};
\def\mypath{(3,4.8)--(4.8,3)-- (3,3)--cycle};
\fill [fill=pink] \mypath;
\def\mypath{(1,1) -- (1,0.8)--(0.8,1)--cycle};
\fill [fill=pink] \mypath;
%\filldraw[fill=bluedark, draw=blue!20, thick] (1,1.8) --(1.8,1)-- (1,1) --cycle;
%\filldraw[fill=bluedark, draw=blue!20, thick] (2.3,2.5)--(2.5,2.3)-- (2.5,1.8)--(1.8,2.5)--cycle;
\def\mypath{(1,1.8) --(1.8,1)-- (1,1) --cycle}
\fill [fill=bluedark] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;
\def\mypath{(2.3,2.5)--(2.5,2.3)-- (2.5,1.8)--(1.8,2.5)--cycle}
\fill [fill=bluedark] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;

%\filldraw[fill=black!50!green, draw=blue!20, thick] (2.5,2.3) --(2.5,2.5)-- (2.3,2.5) --cycle;
%\filldraw[fill=black!50!green, draw=blue!20, thick] (2.5,2.5) --(3,2.5)-- (3,3)--(2.5,3) --cycle;
%\filldraw[fill=black!50!green, draw=blue!20, thick] (4.8,3)-- (6,3)-- (6,3.8)--(3.7,6)--(3,6)--(3,4.8)--cycle;
%\filldraw[fill=black!50!green, draw=blue!20, thick] (6,3.8)--(6,4.3) --(4.3,6) --(3.7,6)--cycle;
%\filldraw[fill=black!50!green, draw=blue!20, thick] (6,4.3) --(6,4.8)--(4.8,6) --(4.3,6)--cycle;
%\filldraw[fill=black!50!green, draw=blue!20, thick] (6,4.8)--(4.8,6) --(5.8,6) --(6,5.8)--cycle;

\def\mypath{ (2.5,2.3) --(2.5,2.5)-- (2.3,2.5) --cycle}
\fill [fill=black!50!green] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;
\def\mypath{(2.5,2.5) --(3,2.5)-- (3,3)--(2.5,3) --cycle}
\fill [fill=black!50!green] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;
\def\mypath{(4.8,3)-- (6,3)-- (6,3.8)--(3.7,6)--(3,6)--(3,4.8)--cycle}
\fill [fill=black!50!green] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;
\def\mypath{(6,3.8)--(6,4.3) --(4.3,6) --(3.7,6)--cycle}
\fill [fill=black!50!green] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;
\def\mypath{ (6,4.3) --(6,4.8)--(4.8,6) --(4.3,6)--cycle}
\fill [fill=black!50!green] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;
\def\mypath{ (6,4.8)--(4.8,6) --(5.8,6) --(6,5.8)--cycle}
\fill [fill=black!50!green] \mypath;
%\pattern[pattern color=black!30,pattern=grid] \mypath;


\def\mypath{ (2.5,1.8)--(2.5,2.3)--(3,1.8) --(3,1.3) --cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{(3,1.8) --(3.7,1) --(6,1) --(6,1.8) -- (5.2,2.5)--(3,2.5)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{(6,1.8) -- (6.7,1)--(8,1)--(8,1.8)--(7.3,2.5)--(6,2.5)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{ (8.5,1.8)--(8.5,1.3)--(8,1.8)-- (8,2.3) --cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{(9,1.8)--(9,1.3)--(8.5,1.8)-- (8.5,2.3) --cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{(9,1.8)--(9.7,1)--(10,1)-- (10,1.75)--(9.3,2.5)--(9,2.5)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{ (1,1)--(1,1.75)--(0.3,2.5)--(0,2.5)--(0,1.75)--(0.7,1.05)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;

%\filldraw[fill=blue!40, pattern color=white,pattern= north east lines] (2.5,1.8)--(2.5,2.3)--(3,1.8) --(3,1.3) --cycle;
%%\filldraw[fill=blue!40, draw=blue!20, thick,pattern color=white,pattern=north east lines] (3,1.8) --(3.7,1) --(6,1) --(6,1.8) -- (5.2,2.5)--(3,2.5)--cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (6,1.8) -- (6.7,1)--(8,1)--(8,1.8)--(7.3,2.5)--(6,2.5)--cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (8.5,1.8)--(8.5,1.3)--(8,1.8)-- (8,2.3) --cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (9,1.8)--(9,1.3)--(8.5,1.8)-- (8.5,2.3) --cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (9,1.8)--(9.7,1)--(10,1)-- (10,1.75)--(9.3,2.5)--(9,2.5)--cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (1,1)--(1,1.75)--(0.3,2.5)--(0,2.5)--(0,1.75)--(0.7,1.05)--cycle;

\def\mypath{ (1.8,2.5)--(2.3,2.5)--(1.8,3) --(1.3,3) --cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(1.8,3) --(1,3.7) --(1,6) --(1.8,6) -- (2.5,5.2)--(2.5,3)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(1.8,6) -- (1,6.8)--(1,8)--(1.8,8)--(2.5,7.3)--(2.5,6)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{ (1.8,8.5)--(1.3,8.5)--(1.8,8)-- (2.3,8) --cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(1.8,9)--(1.3,9)--(1.8,8.5)-- (2.3,8.5) --cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(1.8,9)--(1,9.7)--(1,10)-- (1.75,10)--(2.5,9.3)--(2.5,9)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(1,1)--(1.75,1)--(2.5,0.3)--(2.5,0)--(1.75,0)--(1.05,0.7)--cycle}
\fill [fill=blue!40] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;

%\filldraw[fill=blue!40, draw=blue!20, thick] (1.8,2.5)--(2.3,2.5)--(1.8,3) --(1.3,3) --cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (1.8,3) --(1,3.7) --(1,6) --(1.8,6) -- (2.5,5.2)--(2.5,3)--cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (1.8,6) -- (1,6.8)--(1,8)--(1.8,8)--(2.5,7.3)--(2.5,6)--cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (1.8,8.5)--(1.3,8.5)--(1.8,8)-- (2.3,8) --cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (1.8,9)--(1.3,9)--(1.8,8.5)-- (2.3,8.5) --cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (1.8,9)--(1,9.7)--(1,10)-- (1.75,10)--(2.5,9.3)--(2.5,9)--cycle;
%\filldraw[fill=blue!40, draw=blue!20, thick] (1,1)--(1.75,1)--(2.5,0.3)--(2.5,0)--(1.75,0)--(1.05,0.7)--cycle;

%\filldraw[fill=red, draw=blue!20, thick] (3,2.5)--(3,3)--(4.8,3)--(5.2,2.5) --cycle;
%\filldraw[fill=red, draw=blue!20, thick] (6,2.5)--(6,3) --(6.7,3)--(7.3,2.5)--cycle;
%\filldraw[fill=red, draw=blue!20, thick] (9,2.5)--(9.3,2.5)--(9,2.8) --cycle;

\def\mypath{(3,2.5)--(3,3)--(4.8,3)--(5.2,2.5) --cycle}
\fill [fill=red] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{ (6,2.5)--(6,3) --(6.7,3)--(7.3,2.5)--cycle}
\fill [fill=red] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{ (9,2.5)--(9.3,2.5)--(9,2.8) --cycle}
\fill [fill=red] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;

%\filldraw[fill=yellow, draw=blue!20, thick] (2.5,3)--(3,3)--(3,4.8)--(2.5,5.2) --cycle;
%\filldraw[fill=yellow, draw=blue!20, thick] (2.5,6)--(3,6) --(3,6.7)--(2.5,7.3)--cycle;
%\filldraw[fill=yellow, draw=blue!20, thick] (2.5,9)--(2.5,9.3)--(2.8,9) --cycle;

\def\mypath{ (2.5,3)--(3,3)--(3,4.8)--(2.5,5.2) --cycle}
\fill [fill=yellow] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(2.5,6)--(3,6) --(3,6.7)--(2.5,7.3)--cycle}
\fill [fill=yellow] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(2.5,9)--(2.5,9.3)--(2.8,9) --cycle}
\fill [fill=yellow] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;


\def\mypath{ (3.7,1)--(6,1) -- (6,0)--(4.75,0)--cycle}
\fill [fill=red] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
\def\mypath{(6.7,1)--(8,1)--(8,0)--(7.75,0)--cycle}
\fill [fill=red] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
%\filldraw[fill=red, draw=blue!20, thick] (3.7,1)--(6,1) -- (6,0)--(4.75,0)--cycle;
%\filldraw[fill=red, draw=blue!20, thick] (6.7,1)--(8,1)--(8,0)--(7.75,0)--cycle;
\filldraw[fill=yellow, draw=blue!20, thick] (9.7,1)--(10,1)--(10,0.75)--cycle;
\filldraw[fill=yellow, draw=blue!20, thick] (2.5,0.3)--(2.5,0)--(2.75,0)--cycle;

\def\mypath{(1,3.7)--(1,6) -- (0,6)--(0,4.75)--cycle}
\fill [fill=yellow] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
\def\mypath{(1,6.7)--(1,8)--(0,8)--(0,7.75)--cycle}
\fill [fill=yellow] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
%\filldraw[fill=yellow, draw=blue!20, thick] (1,3.7)--(1,6) -- (0,6)--(0,4.75)--cycle;
%\filldraw[fill=yellow, draw=blue!20, thick] (1,6.7)--(1,8)--(0,8)--(0,7.75)--cycle;
\filldraw[fill=red, draw=blue!20, thick] (1,9.7)--(1,10)--(0.75,10)--cycle;
\filldraw[fill=red, draw=blue!20, thick] (0.3,2.5)--(0,2.5)--(0,2.75)--cycle;


%\filldraw[fill=blue!20, draw=blue!20, thick]  (1.2858,3)--(1,3.2858) --(1,2.5)-- (1.8,2.5)--cycle;
\def\mypath{(1.2858,3)--(1,3.2858) --(1,2.5)-- (1.8,2.5)--cycle}
\fill [fill=blue!20] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
%\filldraw[fill=blue!20, draw=blue!20, thick]  (3,1.2858)--(3.2858,1) --(2.5,1)-- (2.5,1.8)--cycle;
\def\mypath{(3,1.2858)--(3.2858,1) --(2.5,1)-- (2.5,1.8)--cycle}
\fill [fill=blue!20] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;
%\filldraw[fill=blue!20, draw=blue!20, thick]  (1.75,1)--(2.5,1)--(2.5,0.3)--cycle;
\def\mypath{ (1.75,1)--(2.5,1)--(2.5,0.3)--cycle}
\fill [fill=blue!20] \mypath;
%\pattern[pattern color=white,pattern=north east lines] \mypath;
%\filldraw[fill=blue!20, draw=blue!20, thick]  (1,1.75)--(1,2.5)--(0.3,2.5)--cycle;
\def\mypath{(1,1.75)--(1,2.5)--(0.3,2.5)--cycle}
\fill [fill=blue!20] \mypath;
%\pattern[pattern color=white,pattern=north west lines] \mypath;

 \draw[blue!5,dashed]
 (0,0)--(0,10);% -- (10,10)-- (10,0)--(0,0);
 \draw[blue!5,dashed]
 (10,0)--(0,0);
 \draw[ultra thick, blue!5]
 (1,0.7)--(1,10);
 \draw[ultra thick, blue!5]
 (2.5,0)--(2.5,9.2);
 \draw[ultra thick, blue!5]
 (3,0)--(3,8.7);
 \draw[ultra thick, blue!5]
 (6,0)--(6,5.8);
 \draw[ultra thick, blue!5]
 (8,0)--(8,3.7);
 \draw[ultra thick, blue!5]
 (8.5,0)--(8.5,3.3);
 \draw[ultra thick, blue!5]
 (9,0)--(9,2.7);
 
 
\node at (0.5,-0.5) {\tiny{$\nu_{1}$}};
\node at (1.75,-0.5) {\tiny{$\nu_{2}$}};
\node at (2.75,-0.5) {\tiny{$\nu_{3}$}};
\node at (4.5,-0.5) {\tiny{$\nu_{4}$}};
\node at (7,-0.5) {\tiny{$\nu_{5}$}};
\node at (8.15,-0.5) {\tiny{$\nu_{6}$}};
\node at (8.85,-0.5) {\tiny{$\nu_{7}$}};
\node at (9.75,-0.5) {\tiny{$\nu_{8}$}};
 \draw[ thick]
 (0.5,-0.1)--(0.5,0.1);
 \draw[ thick]
 (1.75,-0.1)--(1.75,0.1);
 \draw[ thick]
 (2.75,-0.1)--(2.75,0.1);
 \draw[ thick]
 (4.5,-0.1)--(4.5,0.1);
 \draw[ thick]
 (7,-0.1)--(7,0.1);
 \draw[ thick]
 (8.25,-0.1)--(8.25,0.1);
 \draw[ thick]
 (8.75,-0.1)--(8.75,0.1);
  \draw[ thick]
 (9.5,-0.1)--(9.5,0.1);

\node at (-0.5,0.5) {\tiny{$\nu_{1}$}};
\node at (-0.5,1.75) {\tiny{$\nu_{2}$}};
\node at (-0.5,2.75) {\tiny{$\nu_{3}$}};
\node at (-0.5,4.5) {\tiny{$\nu_{4}$}};
\node at (-0.5,7) {\tiny {$\nu_{5}$}};
\node at (-0.5,8.25) {\tiny{$\nu_{6}$}};
\node at (-0.5,8.75) {\tiny{$\nu_{7}$}};
\node at (-0.5,9.5) {\tiny {$\nu_{8}$}};
 \draw[ thick]
 (-0.1,0.5)--(0.1,0.5);
 \draw[ thick]
 (-0.1,1.75)--(0.1,1.75);
 \draw[ thick]
 (-0.1,2.75)--(0.1,2.75);
 \draw[ thick]
 (-0.1,4.5)--(0.1,4.5);
 \draw[ thick]
 (-0.1,7)--(0.1,7);
 \draw[ thick]
 (-0.1,8.25)--(0.1,8.25);
 \draw[ thick]
 (-0.1,8.75)--(0.1,8.75);
  \draw[ thick]
 (-0.1,9.5)--(0.1,9.5);
        
        
   \draw[ultra thick, blue!5]
 (0.7,1)--(10,1);
 \draw[ultra thick, blue!5]
 (0,2.5)--(9.2,2.5);
 \draw[ultra thick, blue!5]
 (0,3)--(8.7,3);
 \draw[ultra thick, blue!5]
 (0,6)--(5.8,6);
 \draw[ultra thick, blue!5]
 (0,8)--(3.7,8);
 \draw[ultra thick, blue!5]
 (0,8.5)--(3.3,8.5);
 \draw[ultra thick, blue!5]
 (0,9)--(2.7,9);      

 

  \draw[ultra thick, blue!5]
 (0,1.75)--(1.75,0);
 \draw[ultra thick, blue!5]
 (0,2.75)--(2.75,0);
 \draw[ultra thick, blue!5]
 (0,4.25)--(4.25,0);
 \draw[ultra thick, blue!5]
 (0,4.75)--(4.75,0);
 \draw[ultra thick, blue!5]
 (0,7.75)--(7.75,0);
 \draw[ultra thick, blue!5]
 (0,9.75)--(9.75,0);
 \draw[ultra thick, blue!5]
 (0.25,10)--(10,0.25);
 \draw[ultra thick, blue!5]
 (0.75,10)--(10,0.75);
 \draw[ultra thick, blue!5]
 (1.75,10)--(10,1.75);
 
% \draw[thick, blue!20,dashed]
%(0,0) --(0,1.75);
 %\draw[thick, blue!20,dashed]
%(0,0) --(1.75,0);
 %\draw[thick,blue!20,dashed]
%(0,1) --(0.7,1);
 %\draw[thick, blue!20,dashed]
%(1,0) --(1,0.7);

% \draw[ultra thick,white,dashed]
%(6,5.8) --(6,10);
 %\draw[ultra thick,white,dashed]
%(5.8,6) --(10,6);
 %\draw[ultra thick,white,dashed]
%(10,1.75) --(10,10);
 %\draw[ultra thick,white,dashed]
%(1.75,10) --(10,10);
 %\draw[ultra thick,white,dashed]
%(9,2.8)--(9,10);
 %\draw[ultra thick,white,dashed]
%(2.8,9)--(10,9); 
 %\draw[ultra thick,white,dashed]
%(8.5,3.3)--(8.5,10);
 % \draw[ultra thick,white,dashed]
%(3.3,8.5)--(10,8.5);
 %\draw[ultra thick,white,dashed]
%(8,3.8) --(8,10);
 %\draw[ultra thick,white,dashed]
%(3.8,8)--(10,8);


 \draw[ultra thick, blue]
 (0,1.75)--(0,10)--(0,10)--(1.75,10)--(1.75,10)--(10,1.75)-- (10,0)--(1.75,0)-- (0,1.75);
% \draw[ultra thick, blue]
% (1.725,0)--(10.04,0);
% \draw[ultra thick, blue]
% (0,1.75)--(1.75,0);
%  \draw[ultra thick, blue]
% (10,0)--(10,1.77);
%   \draw[ultra thick, blue]
% (0,10)--(1.75,10);
%  \draw[ultra thick, blue]
% (1.75,10)--(10,1.75);

\draw [ -latex,red, ultra thick, dashed] (1.75,-0.1) -- (1.75,11.5)node at (3.95,11.75) {axes of maximum FWM efficiency};
\draw [ -latex,red,ultra thick,dashed] (-0.1,1.75) -- (11,1.75);
%\draw [ -latex,blue!40, thick] (-0.6,0) -- (10.6,0)node at (10.9,0) {$f_1$};% {$\kappa_1$};
%\draw [ -latex,blue!40, thick] (0,-0.6) -- (0,10.6)node at (0,10.9) {$f_2$};% {$\kappa_2$};
%\draw [ -latex,blue!40, thick] (-0.6,-0.6) -- (10.5,10.5)node at (10.7,10.7){$f_3$};% {$\tilde{\kappa}$}; 
%\node at (1.2858,3) {};
\end{tikzpicture}
\caption{Demonstrating regions of the EGN model terms integrands, the GN model, and the correction terms of (\ref{EGN_elastic}), for an eight-channel fiber-optic spectrum (with different bandwidths and center frequencies) and its second channel as the COI. The central frequency of channel $i$ is denoted by $\nu_{i}$. Regions inside the ultra thick blue boundaries are referred to as integration regions. The white islands (polygons) are representing the regions, where NLI contribution to the COI is present only based on the GN model term, whereas the colored islands are contributing NLI to the COI based on both GN model and correction terms.}
\label{elast_demonstration}
\vspace{-0.5cm}
\end{figure}

==> Interpretation.tex <==
{\color{red}\section{Interpretation of the key result 
%and comparison with previous models
}\label{interpretation}

%The NLI PSD of channel $\kappa$ is computed (see \eqref{NLI_Power_Channel_Kappa}), by taking expectation of the product of the nonlinear electrical field of channel $\kappa$, i. e., $E_{\text{NLI,x},\kappa}$, and its complex conjugate, summed with the corresponding result for polarization y. The 3 spectral components $mf_0$, $nf_0$, and $kf_0$ of $E_{\text{NLI,x},\kappa}$ (see \eqref{NLI_elec_tot_detail}) in the limit of large signal period, i.e.,  ${f_0\rightarrow0}$, tend to three continuous frequencies of $f_1$,  $f_3-lR$, and $f_2$, resp, where $f_3=f_1+f_2-f$. %located in channels $\kappa_1$, $\kappa_2$, and $\kappa_1+\kappa_2-\kappa+l$, respectively. 
%Moreover, the summation over indices $i$, $m$, $n$, and $k$ will be replaced by integral with variables $f$, $f_1$, $f_2$, and $f_3$, respectively. 
%These three $f_1$, $f_2$, and $f_3$ spectral components of the nonlinear electrical field interact and produce an interfering harmonic at frequency $f$, located in the COI. 
%We now proceed with  interpretation of the different NLI terms introduced in \eqref{EGN_fixed} exploiting the same taxonomy used in \cite{Poggiolini2012,Pontus_JLT_modeling_2013}. Considering $G_{\text{NLI},\kappa}=\mathbb{E}\{E_{\text{NLI,x},\kappa}E^{*}_{\text{NLI,x},\kappa}\}$, the NLI PSD of the COI is computed by averaging over the product of a set of six spectral components, consisting of $f_1$, $f_2$, and $f_3$ %(shown on the vertical, horizontal, and diagonal axes, respectively) 
%from the nonlinear electrical field, i. e., $E_{\text{NLI,x},\kappa}$, and $f'_1$, $f'_2$, and $f'_3$ from its complex conjugate, 
%(similarly shown on the vertical, horizontal, and diagonal axes, respectively)
 %interacting to produce the nonlinear PSD spectral lines.
 
% We can compute all the NLI contributions on COI by means of \eqref{EGN_fixed}. The triple summation in this equation represents the integration regions with $(\kappa_1,\kappa_2,\kappa_1+\kappa_2-\kappa+l)$ coordinate, implying that the frequency pairs $(f_1,f_1')$, $(f_2,f_2')$, and $(f_3,f_3')$ are located in $\kappa_1$, $\kappa_2$, and $\tilde{\kappa}=\kappa_1+\kappa_2-\kappa+l$, resp. %These interfering frequencies can be located in different WDM channels, resulting in $D_\kappa$, $E_\kappa$, $F_\kappa$, $G_\kappa$, and $H_\kappa$ terms of \eqref{EGN_fixed}, which are triple, fourth-fold, fourth-fold, fourth-fold, and fifth-fold integrals, resp. 
%The integration regions can be demonstrated in [$f_1,f_2$] plane. For instance, in Fig.~\ref{LT} we assume five Nyquist channels can accommodate in the  WDM spectrum. The grid lines in the horizontal($f_1$) and vertical ($f_2$) axes are determined with the five channels border lines. To determine grid lines in the diagonal axis since $f_3=f_1+f_2-f$ and $f'_3= f_1'+f_2'-f$, one can first start with the grid line of the COI channel, using the intersection of the COI grid lines from the horizontal and vertical axes, then the other grid lines of diagonal axis are drawn by the corresponding channel spacings shrank by a factor of $\sqrt{2}$, driven from the coordinates geometry. 






\begin{figure}
\centering
%\begin{tikzpicture}[scale=0.6]
%\draw [postaction={decorate,draw=red!40,fill=red!40}]
%(-0.2-1.15-0.6,0+2) -- (-0.2-1.15+1+0.6,0+2) --(-0.2-1.15+1+0.6,0.75+2)--(-0.2-1.15-0.6,0.75+2)node at (-0.2-1.15+1+0.6,-0.5+2) {\footnotesize{$\frac{R}{2}$}}node at (-0.2-1.4-1+0.6,-0.5+2) {\footnotesize{$-\frac{R}{2}$}};
%\draw [-latex,red, thick] (-0.975-0.5-1.15,0+2) -- (-0.6+3.5-0.55-1.15,0+2) node at (-0.6+3.5-0.55-1,-0.2+2) {$f$};
%\draw [-latex,dashed] (-0.2-1.15+1/2,0+2.25-2.25+2) -- (-0.2-1.15+1/2,0+2+1.7-2.25+2) node at (-0.2-1.15+1/2,0+2+1.7-2+2) {\footnotesize{$f=0$}};
%\draw [postaction={decorate,draw=red!40,fill=red!40}]
%(-0.2-1.15-0.6+1,0+2) -- (-0.2-1.15+1+0.6+1,0+2) --(-0.2-1.15+1+0.6+1,0.75+2)--(-0.2-1.15-0.6+1,0.75+2);
%\end{tikzpicture}
%\begin{tikzpicture}[scale=0.6]
%\node at (-2,-2){a)};
 %\draw[thick, blue!20]
 %(0,2)--(1,2) -- (2,1)-- (2,0)--(1,0)--(0,1)--(0,2);
 %\draw[thick, blue!20]
 %(1.1,2) -- (2,1.1)--(2,2)--(1.1,2);
 %\draw[thick, blue!20]
 %(0,0) -- (0,0.9)--(0.9,0)--(0,0);
  %  \def\mypath{ (0,0) -- (0,0.9)--(0.9,0)--(0,0)}
%\fill[purple]\mypath;

 
 
% \draw[thick, blue!20]
 %(2.1,2)--(3.1,2) -- (4.1,1)-- (4.1,0)--(3.1,0)--(2.1,1)--(2.1,2);
 %\draw[thick, blue!20]
 %(3.2,2) -- (4.1,1.1)--(4.1,2)--(3.2,2);
 %\draw[thick, blue!20]
 %(2.1,0) -- (2.1,0.9)--(3,0)--(2.1,0);
  %   \def\mypath{ (2.1,0) -- (2.1,0.9)--(3,0)--(2.1,0)}
 %\fill[purple]\mypath;
 
 
 %\draw[thick, blue!20]
 %(4.2,2)--(5.2,2) -- (6.2,1)-- (6.2,0)--(5.2,0)--(4.2,1)--(4.2,2);
 %\draw[thick, blue!20]
 %(5.3,2) -- (6.2,1.1)--(6.2,2)--(5.3,2);
  %  \def\mypath{ (5.3,2) -- (6.2,1.1)--(6.2,2)--(5.3,2)}
% \mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 %\draw[thick, blue!20]
 %(4.2,0) -- (4.2,0.9)--(5.1,0)--(4.2,0);
  % \def\mypath{(4.2,0) -- (4.2,0.9)--(5.1,0)--(4.2,0)}
% \fill[purple]\mypath;

 
 %\draw[thick, blue!20]
 %(6.3,2)--(7.3,2) -- (8.3,1)-- (8.3,0)--(7.3,0)--(6.3,1)--(6.3,2);
  %   \def\mypath{ (6.3,2)--(7.3,2) -- (8.3,1)-- (8.3,0)--(7.3,0)--(6.3,1)--(6.3,2)}
%\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 %\draw[thick, blue!20]
 %(6.3,0) -- (6.3,0.9)--(7.2,0)--(6.3,0);
  %  \def\mypath{ (6.3,0) -- (6.3,0.9)--(7.2,0)--(6.3,0)}
 %\fill[purple]\mypath;

 
 %%%%%%%%
% \draw [ -latex,red!100, thick, dashed] (-0.2,-1) -- (10.2,-1) 
%\node at ( 7.3,-1.1) [inner sep=0pt,minimum size=2mm,circle,fill=red!100] (3){\scriptsize {}};

%\draw[thick, blue!20]
 %(0,-0.1)--(1,-0.1) -- (2,-1.1)-- (2,-2.1)--(1,-2.1)--(0,-1.1)--(0,-0.1);
  %\def\mypath{ (0,-0.1)--(1,-0.1) -- (2,-1.1)-- (2,-2.1)--(1,-2.1)--(0,-1.1)--(0,-0.1)}
%\fill[purple] \mypath;

 
 %\draw[thick, blue!20]
 %(1.1,-0.1) -- (2,-1)--(2,-0.1)--(1.1,-0.1);
  %\def\mypath{  (1.1,-0.1) -- (2,-1)--(2,-0.1)--(1.1,-0.1)}
%\mypath;

    
 %\draw[thick, blue!20]
 %(2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1);
 %\def\mypath{ (2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1)}
%\fill[purple] \mypath;
%\pattern[color=white,pattern=horizontal lines] \mypath;
 %   \def\mypath{ (2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1)}
%\fill[purple] \mypath;
%\pattern[pattern color=purple,pattern=horizontal lines] \mypath;

 %\draw[thick, blue!20]
 %(3.2,-0.1) -- (4.1,-1)--(4.1,-0.1)--(3.2,-0.1);
 %\draw[thick, blue!20]
 %(2.1,-2.1) -- (2.1,-1.2)--(3,-2.1)--(2.1,-2.1);
 
 %\draw[thick, blue!20]
 %(4.2,-0.1)--(5.2,-0.1) -- (6.2,-1.1)-- (6.2,-2.1)--(5.2,-2.1)--(4.2,-1.1)--(4.2,-0.1);
 %  \def\mypath{ (4.2,-0.1)--(5.2,-0.1) -- (6.2,-1.1)-- (6.2,-2.1)--(5.2,-2.1)--(4.2,-1.1)--(4.2,-0.1)}
%\fill[purple] \mypath;
%\pattern[pattern color=purple,pattern=horizontal lines] \mypath;

 %\draw[thick, blue!20]
 %(5.3,-0.1) -- (6.2,-1)--(6.2,-0.1)--(5.3,-0.1);
 %\def\mypath{ (5.3,-0.1) -- (6.2,-1)--(6.2,-0.1)--(5.3,-0.1)}
%\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 %\draw[thick, blue!20]
 %(4.2,-2.1) -- (4.2,-1.2)--(5.1,-2.1)--(4.2,-2.1);
 
 %\draw[thick, blue!20, fill=red]
 %(6.3,-0.1)--(7.3,-0.1) -- (8.3,-1.1)-- (8.3,-2.1)--(7.3,-2.1)--(6.3,-1.1)--(6.3,-0.1)node at (6.8,-0.5) [black]{SCI} node at (7.8,-1.5) [black]{\scriptsize{COI}};
  %  \def\mypath{ (6.3,-0.1)--(7.3,-0.1) -- (8.3,-1.1)-- (8.3,-2.1)--(7.3,-2.1)--(6.3,-1.1)--(6.3,-0.1)}
%\fill [fill=white] \mypath;
%\pattern[pattern color=red,pattern=dots] \mypath;

 %\draw[thick, blue!20, fill=black!40!green]
 %(7.4,-0.1) -- (8.3,-1)--(8.3,-0.1)--(7.4,-0.1);
%\def\mypath{ (7.4,-0.1) -- (8.3,-1)--(8.3,-0.1)--(7.4,-0.1)}
%\fill [fill=black!40!green] \mypath;
%\pattern[pattern color=white,pattern=grid] \mypath;
 
 %\draw[thick, blue!20, fill=black!40!green]
% (6.3,-2.1) -- (6.3,-1.2)--(7.2,-2.1)--(6.3,-2.1);
 %\def\mypath{ (6.3,-2.1) -- (6.3,-1.2)--(7.2,-2.1)--(6.3,-2.1)}
%\fill [fill=black!40!green] \mypath;
%\pattern[pattern color=white,pattern=grid] \mypath;
 
 %\draw[thick, blue!20, fill=red]%pink balla
 %(8.4,0) -- (8.4,0.9)--(9.3,0)--(8.4,0);
  %\def\mypath{ (8.4,0) -- (8.4,0.9)--(9.3,0)--(8.4,0)}
%\fill [fill=white] \mypath;
%\pattern[pattern color=red,pattern=dots] \mypath;
 
%\draw[thick, blue!20]
 %(8.4,-0.1)--(9.4,-0.1) -- (10.4,-1.1)-- (10.4,-2.1)--(9.4,-2.1)--(8.4,-1.1)--(8.4,-0.1);
  %  \def\mypath{ (8.4,-0.1)--(9.4,-0.1) -- (10.4,-1.1)-- (10.4,-2.1)--(9.4,-2.1)--(8.4,-1.1)--(8.4,-0.1)}
% \fill[purple]\mypath;
%\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
%\draw[thick, blue!20]
% (9.5,-0.1) -- (10.4,-1)--(10.4,-0.1)--(9.5,-0.1);
%\draw[thick, blue!20]
 %(8.4,-2.1) -- (8.4,-1.2)--(9.3,-2.1)--(8.4,-2.1);
  % \def\mypath{  (8.4,-2.1) -- (8.4,-1.2)--(9.3,-2.1)--(8.4,-2.1)}
 %\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %%%%%%%%%%
 %\draw[thick, blue!20]
 %(1.1,-2.2) -- (2,-3.1)--(2,-2.2)--(1.1,-2.2);
  % \def\mypath{ (1.1,-2.2) -- (2,-3.1)--(2,-2.2)--(1.1,-2.2)}
%\fill[purple]\mypath;
%\pattern[pattern color=purple,pattern=horizontal lines]\mypath;

 
 %\draw[thick, blue!20]
 %(2.1,-2.2)--(3.1,-2.2) -- (4.1,-3.2)-- (4.1,-4.2)--(3.1,-4.2)--(2.1,-3.2)--(2.1,-2.2);
 %\draw[thick, blue!20]
 %(3.2,-2.2) -- (4.1,-3.1)--(4.1,-2.2)--(3.2,-2.2);
 % \def\mypath{ (3.2,-2.2) -- (4.1,-3.1)--(4.1,-2.2)--(3.2,-2.2)}
%\fill[purple]\mypath;
%\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
 
 %\draw[thick, blue!20, fill=black!40!green]
 %(4.2,-2.2)--(5.2,-2.2) -- (6.2,-3.2)-- (6.2,-4.2)--(5.2,-4.2)--(4.2,-3.2)--(4.2,-2.2);
  %  \def\mypath{ (4.2,-2.2)--(5.2,-2.2) -- (6.2,-3.2)-- (6.2,-4.2)--(5.2,-4.2)--(4.2,-3.2)--(4.2,-2.2)}
%\fill [fill=black!40!green] \mypath;
%\pattern[pattern color=white,pattern=grid] \mypath;
 
 %\draw[thick, blue!20, fill=red]
 %(5.3,-2.2) -- (6.2,-3.1)--(6.2,-2.2)--(5.3,-2.2);
  % \def\mypath{(5.3,-2.2) -- (6.2,-3.1)--(6.2,-2.2)--(5.3,-2.2)}
%\fill [fill=white] \mypath;
%\pattern[pattern color=red,pattern=dots] \mypath;
 
% \draw[thick, blue!20, fill=black!40!green]
 %(4.2,-4.2) -- (4.2,-3.3)--(5.1,-4.2)--(4.2,-4.2);
  %\def\mypath{ (4.2,-4.2) -- (4.2,-3.3)--(5.1,-4.2)--(4.2,-4.2)}
%\fill [fill=black!40!green] \mypath;
%\pattern[pattern color=white,pattern=grid] \mypath;
 
 
 %\draw[thick, blue!20]
 %(6.3,-2.2)--(7.3,-2.2) -- (8.3,-3.2)-- (8.3,-4.2)--(7.3,-4.2)--(6.3,-3.2)--(6.3,-2.2);
 %\def\mypath{ (6.3,-2.2)--(7.3,-2.2) -- (8.3,-3.2)-- (8.3,-4.2)--(7.3,-4.2)--(6.3,-3.2)--(6.3,-2.2)}
% \mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
% \draw[thick, blue!20]
 %(7.4,-2.2) -- (8.3,-3.1)--(8.3,-2.2)--(7.4,-2.2);
 %\def\mypath{ (7.4,-2.2) -- (8.3,-3.1)--(8.3,-2.2)--(7.4,-2.2)}
%\fill[purple]\mypath;
%\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
 
 %\draw[thick, blue!20]
 %(6.3,-4.2) -- (6.3,-3.3)--(7.2,-4.2)--(6.3,-4.2);
 
%\draw[thick, blue!20]
 %(8.4,-2.2)--(9.4,-2.2) -- (10.4,-3.2)-- (10.4,-4.2)--(9.4,-4.2)--(8.4,-3.2)--(8.4,-2.2);
%\draw[thick, blue!20]
 %(9.5,-2.2) -- (10.4,-3.1)--(10.4,-2.2)--(9.5,-2.2);
 %\def\mypath{(9.5,-2.2) -- (10.4,-3.1)--(10.4,-2.2)--(9.5,-2.2)}
 %\fill[purple]\mypath;
%\pattern[pattern color=purple,pattern=horizontal lines]\mypath;
 
%\draw[thick, blue!20]
 %(8.4,-4.2) -- (8.4,-3.3)--(9.3,-4.2)--(8.4,-4.2);
%\def\mypath{ (8.4,-4.2) -- (8.4,-3.3)--(9.3,-4.2)--(8.4,-4.2)}
 %\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %%%%%%%%%%

 %\draw[thick, blue!20, fill=black!40!green]
 %(3.2,-4.3) -- (4.1,-5.2)--(4.1,-4.3)--(3.2,-4.3);
  %    \def\mypath{ (3.2,-4.3) -- (4.1,-5.2)--(4.1,-4.3)--(3.2,-4.3)}
%\fill [fill=black!40!green] \mypath;
%\pattern[pattern color=white,pattern=grid] \mypath;
 
 
 %\draw[thick, blue!20]
 %(4.2,-4.3)--(5.2,-4.3) -- (6.2,-5.3)-- (6.2,-6.3)--(5.2,-6.3)--(4.2,-5.3)--(4.2,-4.3);
 %\draw[thick, blue!20]
 %(5.3,-4.3) -- (6.2,-5.2)--(6.2,-4.3)--(5.3,-4.3);
  %   \def\mypath{(5.3,-4.3) -- (6.2,-5.2)--(6.2,-4.3)--(5.3,-4.3)}
%\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 
 %\draw[thick, blue!20]
 %(6.3,-4.3)--(7.3,-4.3) -- (8.3,-5.3)-- (8.3,-6.3)--(7.3,-6.3)--(6.3,-5.3)--(6.3,-4.3);
  %  \def\mypath{ (6.3,-4.3)--(7.3,-4.3) -- (8.3,-5.3)-- (8.3,-6.3)--(7.3,-6.3)--(6.3,-5.3)--(6.3,-4.3)}
%\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 %\draw[thick, blue!20]
 %(7.4,-4.3) -- (8.3,-5.2)--(8.3,-4.3)--(7.4,-4.3);
 %\draw[thick, blue!20]
 %(6.3,-6.3) -- (6.3,-5.4)--(7.2,-6.3)--(6.3,-6.3);
 
%\draw[thick, blue!20]
 %(8.4,-4.3)--(9.4,-4.3) -- (10.4,-5.3)-- (10.4,-6.3)--(9.4,-6.3)--(8.4,-5.3)--(8.4,-4.3);

 
%\draw[thick, blue!20]
 %(9.5,-4.3) -- (10.4,-5.2)--(10.4,-4.3)--(9.5,-4.3);
%\draw[thick, blue!20]
 %(8.4,-6.3) -- (8.4,-5.4)--(9.3,-6.3)--(8.4,-6.3);
  %\def\mypath{ (8.4,-6.3) -- (8.4,-5.4)--(9.3,-6.3)--(8.4,-6.3)}
%\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %%%%%%%%%%

 %\draw[thick, blue!20]
 %(5.3,-6.4) -- (6.2,-7.3)--(6.2,-6.4)--(5.3,-6.4);
 %\def\mypath{  (5.3,-6.4) -- (6.2,-7.3)--(6.2,-6.4)--(5.3,-6.4)}
%\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %\draw[thick, blue!20]
 %(6.3,-6.4)--(7.3,-6.4) -- (8.3,-7.4)-- (8.3,-8.4)--(7.3,-8.4)--(6.3,-7.4)--(6.3,-6.4);
  %\def\mypath{ (6.3,-6.4)--(7.3,-6.4) -- (8.3,-7.4)-- (8.3,-8.4)--(7.3,-8.4)--(6.3,-7.4)--(6.3,-6.4)}\fill[blue];
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 %\draw[thick, blue!20]
 %(7.4,-6.4) -- (8.3,-7.3)--(8.3,-6.4)--(7.4,-6.4);
 
%\draw[thick, blue!20]
 %(8.4,-6.4)--(9.4,-6.4) -- (10.4,-7.4)-- (10.4,-8.4)--(9.4,-8.4)--(8.4,-7.4)--(8.4,-6.4);
%\draw[thick, blue!20]
% (9.5,-6.4) -- (10.4,-7.3)--(10.4,-6.4)--(9.5,-6.4);
%\draw[thick, blue!20]
 %(8.4,-8.4) -- (8.4,-7.5)--(9.3,-8.4)--(8.4,-8.4);
  %\def\mypath{(8.4,-8.4) -- (8.4,-7.5)--(9.3,-8.4)--(8.4,-8.4)}
%\mypath;
%\pattern[pattern color=blue,pattern=vertical lines] \mypath;

%\draw[thick, blue!20]
%(9.5,-6.4) -- (10.4,-7.3)--(10.4,-6.4)--cycle;

 
 
% \draw [ -latex,red, ultra thick, dashed] (-0.2,-1.1) -- (11.7,-1.1);
%\draw [ -latex,red,ultra thick,dashed] (7.3,-8.6) -- (7.3,3.8)node at (7.3,4.2) {axes of maximum FWM efficiency};

% \draw [ -latex,blue!50, thick] (-0.2-1,-3.2-5.2) -- (11.2,-3.2-5.2) node at (11.5,-3.4-5) {\tiny$ f_1$};
 
 % \draw [ -latex,blue!50, dashed] (-0.2-1,-3.2-5.3) -- (12.5,-3.2-5.3) node at (12.7,-3.2-5) {\small$\kappa_1$};
 
%\draw [ -latex,blue!50, thick] (0,-8.6-1) -- (0,3) node at (0,3.3) {\tiny$f_2$};

%\draw [ -latex,blue!50, dashed] (-0.1,-8.6-1) -- (-0.1,4) node at (-0.1,4.3) {\small$\kappa_2$};

%\draw [ -latex,blue!50, thick] (2.4-3,-6-3) -- (10.5,2.1) node at (10.5,2.5) {\tiny$ f_1+f_2$};


%\draw [ -latex,blue!50, dashed] (2.4-3+0.05,-6-3-0.05) -- (11+0.3,2.8-0.05) node at (11+0.3,3.3-0.05) {\small$\tilde{\kappa}$};

% \draw[thick, blue!40, fill=blue!40]
% (1.25,-4) -- (1.25,-3.75)--(1.5,-3.75)--(1.5,-4)-- (1.25,-4) node at (0.2,-3.87) [black]{XCI X1};
% 
% \draw[thick, blue!20, fill=blue!20]
% (1.25,-4.7) -- (1.25,-4.45)--(1.5,-4.45)--(1.5,-4.7)-- (1.25,-4.7)node at (0.2,-4.6) [black]{XCI X2};
% 
%\draw[thick, black!50!blue, fill=black!50!blue]
% (1.25,-5.4) -- (1.25,-5.15)--(1.5,-5.15)--(1.5,-5.4)-- (1.25,-5.4)node at (0.2,-5.34) [black]{XCI X3};
%
%\draw[thick, pink, fill=pink]
% (1.25,-6.1) -- (1.25,-5.85)--(1.5,-5.85)--(1.5,-6.1)-- (1.25,-6.1)node at (0.2,-6.08) [black]{XCI X4};
% 
% %%%%%
%  \draw[thick, black, fill=white]
% (1.75,-6.75) -- (1.75,-6.5)--(2,-6.5)--(2,-6.75)-- (1.75,-6.75) node at (3.2,-6.6) [black]{MCI M0};
% 
%  \draw[thick, yellow, fill=yellow]
% (1.75,-7.45) -- (1.75,-7.2)--(2,-7.2)--(2,-7.45)-- (1.75,-7.45)node at (3.2,-7.34) [black]{MCI M1};
% 
%  \draw[thick, red, fill=red]
% (1.75,-8.15) -- (1.75,-7.9)--(2,-7.9)--(2,-8.15)-- (1.75,-8.15)node at (3.2,-8.08) [black]{MCI M2};
%
%\draw[thick, black!50!green, fill=black!50!green]
% (1.75,-8.85) -- (1.75,-8.6)--(2,-8.6)--(2,-8.85)-- (1.75,-8.85)node at (3.2,-8.82) [black]{MCI M3};
%\node at (0.9,1){\scriptsize{(1,5,2)}};
%\node at (-1,-2){a)};

 %\draw[thick, blue!20,fill=purple]{ 
 %(1+0.75,-4-6.5) -- (1+0.75,-3-6.5)--(2+0.75,-3-6.5)--(2+0.75,-4-6.5)-- cycle node at (2.3,-4.2-5) [black]{\footnotesize{$E_\kappa$}}};
 %\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
 %\draw[thick, blue!20]{ (1+0.75+1.75,-4-6.5) -- (1+0.75+1.75,-3-6.5)--(2+0.75+1.75,-3-6.5)--(2+0.75+1.75,-4-6.5)-- cycle};
 %\def\mypath{ (1+0.75+1.75,-4-6.5) -- (1+0.75+1.75,-3-6.5)--(2+0.75+1.75,-3-6.5)--(2+0.75+1.75,-4-6.5)-- cycle node at  (2.3+1.75,-4.2-5) [black]{\footnotesize{$F_\kappa$}}};
 %\pattern[pattern color=blue,pattern=vertical lines] \mypath;
 
% \draw[thick, blue!20,fill=black!40!green]{(1+0.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-4-6.5)-- cycle node at (2.3+1.75+1.75,-4.2-5) [black]{\footnotesize{$G_\kappa$}}};
 % \def\mypath{ (1+0.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75,-4-6.5)-- cycle};
  %   \pattern[pattern color=white,pattern=grid] \mypath;
  
  
 %\draw[thick, blue!20]{ (1+0.75+1.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-4-6.5)-- cycle node at (2.3+1.75+1.75+1.75,-4.2-5) [black]{\footnotesize{$H_\kappa$}}};
  %\def\mypath{(1+0.75+1.75+1.75+1.75,-4-6.5) -- (1+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-3-6.5)--(2+0.75+1.75+1.75+1.75,-4-6.5)-- cycle};
%\pattern[pattern color=red,pattern=dots] \mypath;
 
 
%\end{tikzpicture}

\begin{tikzpicture}[scale=0.6]
%
%\node at (-1,-2){b)};
 \draw[thick, blue!20]
 (0,2)--(1,2) -- (2,1)-- (2,0)--(1,0)--(0,1)--(0,2);
 \draw[thick, blue!20]
 (1.1,2) -- (2,1.1)--(2,2)--(1.1,2);
 \draw[thick, blue!20, fill=yellow]
 (0,0) -- (0,0.9)--(0.9,0)--(0,0);
 
 \draw[thick, blue!20]
 (2.1,2)--(3.1,2) -- (4.1,1)-- (4.1,0)--(3.1,0)--(2.1,1)--(2.1,2);
 \draw[thick, blue!20]
 (3.2,2) -- (4.1,1.1)--(4.1,2)--(3.2,2);
 \draw[thick, blue!20, fill=yellow]
 (2.1,0) -- (2.1,0.9)--(3,0)--(2.1,0);
 
 \draw[thick, blue!20]
 (4.2,2)--(5.2,2) -- (6.2,1)-- (6.2,0)--(5.2,0)--(4.2,1)--(4.2,2);
 \draw[thick, blue!20, fill=yellow]
 (5.3,2) -- (6.2,1.1)--(6.2,2)--(5.3,2);
 \draw[thick, blue!20, fill=yellow]
 (4.2,0) -- (4.2,0.9)--(5.1,0)--(4.2,0);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,2)--(7.3,2) -- (8.3,1)-- (8.3,0)--(7.3,0)--(6.3,1)--(6.3,2);
 \draw[thick, blue!20, fill=blue!20]
 (6.3,0) -- (6.3,0.9)--(7.2,0)--(6.3,0);
 %%%%%%%%
% \draw [ -latex,red!100, thick, dashed] (-0.2,-1) -- (10.2,-1) 
%\node at ( 7.3,-1.1) [inner sep=0pt,minimum size=2mm,circle,fill=red!100] (3){\scriptsize {}};

\draw[thick, blue!20, fill=blue!40]
 (0,-0.1)--(1,-0.1) -- (2,-1.1)-- (2,-2.1)--(1,-2.1)--(0,-1.1)--(0,-0.1);
 \draw[thick, blue!20]
 (1.1,-0.1) -- (2,-1)--(2,-0.1)--(1.1,-0.1);
 
 \draw[thick, blue!20, fill=blue!40]
 (2.1,-0.1)--(3.1,-0.1) -- (4.1,-1.1)-- (4.1,-2.1)--(3.1,-2.1)--(2.1,-1.1)--(2.1,-0.1);
 \draw[thick, blue!20]
 (3.2,-0.1) -- (4.1,-1)--(4.1,-0.1)--(3.2,-0.1);
 \draw[thick, blue!20]
 (2.1,-2.1) -- (2.1,-1.2)--(3,-2.1)--(2.1,-2.1);
 
 \draw[thick, blue!20, fill=blue!40]
 (4.2,-0.1)--(5.2,-0.1) -- (6.2,-1.1)-- (6.2,-2.1)--(5.2,-2.1)--(4.2,-1.1)--(4.2,-0.1);
 \draw[thick, blue!20, fill=blue!20]
 (5.3,-0.1) -- (6.2,-1)--(6.2,-0.1)--(5.3,-0.1);
 \draw[thick, blue!20]
 (4.2,-2.1) -- (4.2,-1.2)--(5.1,-2.1)--(4.2,-2.1);
 
 \draw[thick, blue!20, fill=pink]
 (6.3,-0.1)--(7.3,-0.1) -- (8.3,-1.1)-- (8.3,-2.1)--(7.3,-2.1)--(6.3,-1.1)--(6.3,-0.1) node at (6.9,-0.8) [black]{\scriptsize{COI}};
 \draw[thick, blue!20, fill=black!50!blue]
 (7.4,-0.1) -- (8.3,-1)--(8.3,-0.1)--(7.4,-0.1);
 \draw[thick, blue!20, fill=black!50!blue]
 (6.3,-2.1) -- (6.3,-1.2)--(7.2,-2.1)--(6.3,-2.1);
 \draw[thick, blue!20, fill=pink]%pink balla
 (8.4,0) -- (8.4,0.9)--(9.3,0)--(8.4,0);
 
\draw[thick, blue!20, fill=blue!40]
 (8.4,-0.1)--(9.4,-0.1) -- (10.4,-1.1)-- (10.4,-2.1)--(9.4,-2.1)--(8.4,-1.1)--(8.4,-0.1);
%\draw[thick, blue!20]
% (9.5,-0.1) -- (10.4,-1)--(10.4,-0.1)--(9.5,-0.1);
\draw[thick, blue!20, fill=blue!20]
 (8.4,-2.1) -- (8.4,-1.2)--(9.3,-2.1)--(8.4,-2.1);
 %%%%%%%%%%
 \draw[thick, blue!20, fill=red]
 (1.1,-2.2) -- (2,-3.1)--(2,-2.2)--(1.1,-2.2);

 
 \draw[thick, blue!20]
 (2.1,-2.2)--(3.1,-2.2) -- (4.1,-3.2)-- (4.1,-4.2)--(3.1,-4.2)--(2.1,-3.2)--(2.1,-2.2);
 \draw[thick, blue!20, fill=red]
 (3.2,-2.2) -- (4.1,-3.1)--(4.1,-2.2)--(3.2,-2.2);
 
 \draw[thick, blue!20, fill=black!40!green]
 (4.2,-2.2)--(5.2,-2.2) -- (6.2,-3.2)-- (6.2,-4.2)--(5.2,-4.2)--(4.2,-3.2)--(4.2,-2.2);
 \draw[thick, blue!20, fill=pink]
 (5.3,-2.2) -- (6.2,-3.1)--(6.2,-2.2)--(5.3,-2.2);
 \draw[thick, blue!20, fill=black!40!green]
 (4.2,-4.2) -- (4.2,-3.3)--(5.1,-4.2)--(4.2,-4.2);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,-2.2)--(7.3,-2.2) -- (8.3,-3.2)-- (8.3,-4.2)--(7.3,-4.2)--(6.3,-3.2)--(6.3,-2.2);
 \draw[thick, blue!20, fill=blue!20]
 (7.4,-2.2) -- (8.3,-3.1)--(8.3,-2.2)--(7.4,-2.2);
 \draw[thick, blue!20]
 (6.3,-4.2) -- (6.3,-3.3)--(7.2,-4.2)--(6.3,-4.2);
 
\draw[thick, blue!20]
 (8.4,-2.2)--(9.4,-2.2) -- (10.4,-3.2)-- (10.4,-4.2)--(9.4,-4.2)--(8.4,-3.2)--(8.4,-2.2);
\draw[thick, blue!20, fill=yellow]
 (9.5,-2.2) -- (10.4,-3.1)--(10.4,-2.2)--(9.5,-2.2);
\draw[thick, blue!20, fill=yellow]
 (8.4,-4.2) -- (8.4,-3.3)--(9.3,-4.2)--(8.4,-4.2);
 %%%%%%%%%%

 \draw[thick, blue!20, fill=black!40!green]
 (3.2,-4.3) -- (4.1,-5.2)--(4.1,-4.3)--(3.2,-4.3);
 
 \draw[thick, blue!20]
 (4.2,-4.3)--(5.2,-4.3) -- (6.2,-5.3)-- (6.2,-6.3)--(5.2,-6.3)--(4.2,-5.3)--(4.2,-4.3);
 \draw[thick, blue!20, fill=red]
 (5.3,-4.3) -- (6.2,-5.2)--(6.2,-4.3)--(5.3,-4.3);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,-4.3)--(7.3,-4.3) -- (8.3,-5.3)-- (8.3,-6.3)--(7.3,-6.3)--(6.3,-5.3)--(6.3,-4.3);
 \draw[thick, blue!20]
 (7.4,-4.3) -- (8.3,-5.2)--(8.3,-4.3)--(7.4,-4.3);
 \draw[thick, blue!20]
 (6.3,-6.3) -- (6.3,-5.4)--(7.2,-6.3)--(6.3,-6.3);
 
\draw[thick, blue!20]
 (8.4,-4.3)--(9.4,-4.3) -- (10.4,-5.3)-- (10.4,-6.3)--(9.4,-6.3)--(8.4,-5.3)--(8.4,-4.3);
\draw[thick, blue!20]
 (9.5,-4.3) -- (10.4,-5.2)--(10.4,-4.3)--(9.5,-4.3);
\draw[thick, blue!20, fill=yellow]
 (8.4,-6.3) -- (8.4,-5.4)--(9.3,-6.3)--(8.4,-6.3);
 %%%%%%%%%%

 \draw[thick, blue!20, fill=red]
 (5.3,-6.4) -- (6.2,-7.3)--(6.2,-6.4)--(5.3,-6.4);
 
 \draw[thick, blue!20, fill=blue!40]
 (6.3,-6.4)--(7.3,-6.4) -- (8.3,-7.4)-- (8.3,-8.4)--(7.3,-8.4)--(6.3,-7.4)--(6.3,-6.4);
 \draw[thick, blue!20]
 (7.4,-6.4) -- (8.3,-7.3)--(8.3,-6.4)--(7.4,-6.4);
 
\draw[thick, blue!20]
 (8.4,-6.4)--(9.4,-6.4) -- (10.4,-7.4)-- (10.4,-8.4)--(9.4,-8.4)--(8.4,-7.4)--(8.4,-6.4);
\draw[thick, blue!20]
 (9.5,-6.4) -- (10.4,-7.3)--(10.4,-6.4)--(9.5,-6.4);
\draw[thick, blue!20, fill=yellow]
 (8.4,-8.4) -- (8.4,-7.5)--(9.3,-8.4)--(8.4,-8.4);
 
 
% \draw [ -latex,red, ultra thick, dashed] (-0.2,-1.1) -- (11.7,-1.1);
%\draw [ -latex,red,ultra thick,dashed] (7.3,-8.6) -- (7.3,3.8)node at (7.3,4.2) {axes of maximum FWM efficiency};

\draw [ -latex,blue!50, thick] (-0.2-1,-3.2-5.2) -- (11.2,-3.2-5.2) node at (11.5,-3.4-5) {\tiny$ f_1$};
 
 % \draw [ -latex,blue!50, dashed] (-0.2-1,-3.2-5.3) -- (12.5,-3.2-5.3) node at (12.7,-3.2-5) {\small$\kappa_1$};
 
\draw [ -latex,blue!50, thick] (0+5.5,-8.6-1) -- (0+5.5,3) node at (0+5.5,3.3) {\tiny$f_2$};

%\draw [ -latex,blue!50, dashed] (-0.1,-8.6-1) -- (-0.1,4) node at (-0.1,4.3) {\small$\kappa_2$};

\draw [ -latex,blue!50, thick] (2.4-3,-6-3) -- (10.5,2.1) node at (10.5,2.5) {\tiny$ f_1+f_2$};


%\draw [ -latex,blue!50, dashed] (2.4-3+0.05,-6-3-0.05) -- (11+0.3,2.8-0.05) node at (11+0.3,3.3-0.05) {\small$\tilde{\kappa}$};

 \draw[thick, blue!40, fill=blue!40]
 (1.25+3,-4-6) -- (1.25+3,-3.75-6)--(1.5+3,-3.75-6)--(1.5+3,-4-6)-- (1.25+3,-4-6) node at (0.2+3,-3.87-6) [black]{XCI X1};
 
 \draw[thick, blue!20, fill=blue!20]
 (1.25+3,-4.7-6) -- (1.25+3,-4.45-6)--(1.5+3,-4.45-6)--(1.5+3,-4.7-6)-- (1.25+3,-4.7-6)node at (0.2+3,-4.6-6) [black]{XCI X2};
 
\draw[thick, black!50!blue, fill=black!50!blue]
 (1.25+3,-5.4-6) -- (1.25+3,-5.15-6)--(1.5+3,-5.15-6)--(1.5+3,-5.4-6)-- (1.25+3,-5.4-6)node at (0.2+3,-5.34-6) [black]{XCI X3};

\draw[thick, pink, fill=pink]
 (1.25+3,-6.1-6) -- (1.25+3,-5.85-6)--(1.5+3,-5.85-6)--(1.5+3,-6.1-6)-- (1.25+3,-6.1-6)node at (-0.4+3,-6.08-6) [black]{SCI, XCI X4};
 
 %%%%%
  \draw[thick, black, fill=white]
 (1.75+5,-6.75-3.25) -- (1.75+5,-6.5-3.25)--(2+5,-6.5-3.25)--(2+5,-6.75-3.25)-- (1.75+5,-6.75-3.25) node at (3.2+5,-6.6-3.25) [black]{MCI M0};
 
  \draw[thick, yellow, fill=yellow]
 (1.75+5,-7.45-3.25) -- (1.75+5,-7.2-3.25)--(2+5,-7.2-3.25)--(2+5,-7.45-3.25)-- (1.75+5,-7.45-3.25)node at (3.2+5,-7.34-3.25) [black]{MCI M1};
 
  \draw[thick, red, fill=red]
 (1.75+5,-8.15-3.25) -- (1.75+5,-7.9-3.25)--(2+5,-7.9-3.25)--(2+5,-8.15-3.25)-- (1.75+5,-8.15-3.25)node at (3.2+5,-8.08-3.25) [black]{MCI M2};

\draw[thick, black!50!green, fill=black!50!green]
 (1.75+5,-8.85-3.25) -- (1.75+5,-8.6-3.25)--(2+5,-8.6-3.25)--(2+5,-8.85-3.25)-- (1.75+5,-8.85-3.25)node at (3.2+5,-8.82-3.25) [black]{MCI M3};
 
\node at (0.9,1.15) [black]{\#};
\end{tikzpicture}
\caption{
Demonstrating regions of the EGN model terms integrands, the GN model, and the correction terms of (\ref{EGN_fixed}), for a five-channel fiber-optic spectrum (rectangular Nyquist) and its fourth channel as the COI ($\kappa=4$). The white islands (polygons) are representing the regions, where NLI contribution to the COI is present only based on the GN model term, whereas the colored islands are contributing NLI to the COI based on both GN model and correction terms. $l=-1$ and $l=+1$ indicate the lower and upper triangle islands, resp, while $l=0$ indicates the lozenge shape islands.
}
\label{LT}
\end{figure}

%Here for a fiber-optic link with five spectrum channels ($M$ = 5), where the fourth channel ($\kappa=4$) is assumed to be the COI, islands with different colors and patterns are illustrated in Fig.~\ref{LT}, indicating the areas of spectral components where their interaction gives rise to a certain NLI, either the GN model term or one of the correction terms on the COI. For instance, the island, marked with ``(1, 5, 2)", indicates the NLI contribution on the COI caused by the nonlinear interaction among the spectral components $(f_1,f_1')$, $(f_2,f_2')$, and $(f_1+f_2-f,f_1'+f_2'-f)$ located in channels $1$, $5$, and $2$, respectively, producing a PSD spectral line at frequency $f$ of the COI (channel 4). As seen in Fig.~\ref{LT}, these islands categorized into white and colored islands, where the white islands only produce the GN model term and the colored islands generate both GN model and correction terms.  It is worth mentioning that $l=0$ is demonstrates the lozenge-shaped islands, while $l=\pm 1$ demonstrates the triangle islands. The five introduced terms in \eqref{EGN_fixed} represent the nonlinear interaction between the spectral components $f_1, f_1', f_2, f_2', f_1+f_2-f, f_1'+f_2'-f$ from different island, producing the NLI contributions on the COI (frequency $f$). In the following, we shed more light on these terms as well as their corresponding originating islands.

%\subsection{The GN Model term--$D_{\kappa}$}

%The GN model term, denoted by $D_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the GN model NLI contribution coefficient on the COI from all the islands (either white islands consisting of only GN model term or the other colored islands with both GN model and correction terms). In fact, this NLI contribution is caused by nonlinear interaction between the spectral lines when the pairs $(f_1,f_1')$, $(f_2,f_2')$, and $(f_3,f_3')$ are located in (i) three different channels, (ii) only two of these pairs are located in the same channel, while the third pair is located in a different channel, or (iii) all the three pairs are located in the same channel. Since in all the above cases each pair is described with only a single spectral line, i. e., $f_1=f_1'$, $f_2=f_2'$, and $f_3=f'_3$, this nonlinear interaction gives rise to the second order moments of the involved channels $\kappa_1$, $\kappa_1+\kappa_2-\kappa+l$, and ${\kappa_2}$ transmit symbols.

%\subsection{The first EGN correction term--$E_{\kappa}$}

%The first EGN correction term denoted by $E_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the NLI contribution coefficient on the COI stems from the islands with the same channel as the COI as well as the adjacent channel of the COI in the $f_2$ axis, fulfilling the condition of $\kappa_1=\kappa_1+\kappa_2-\kappa+l$. These islands are colored with purple in Fig.~\ref{LT}(a), categorized in the following two groups: 

%\begin{enumerate}[(i)]
%\item
%The  lozenge-shaped islands ($l=0$) filled with blue in Fig. \ref{LT} (b) where spectral lines $f_2$ and $f'_2$ are located in the the same channel as the COI, while spectral lines $f_1$, $f'_1$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
%\item
%The triangle islands ($l=\pm 1$) filled with red, light blue and yellow in Fig. \ref{LT}(b) where spectral lines $f_2$ and $f'_2$ are co-located in the adjacent channels of the COI, while spectral lines $f_1$, $f'_1$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
%\end{enumerate}
%The NLI contribution caused by nonlinear interaction between the spectral pair components leads to the second and fourth order moments of the two involved channels transmit symbols.  

%\subsection{The second EGN correction term--$F_{\kappa}$}

%The second EGN correction term denoted by $F_{\kappa}$ (see Table~\ref{DEFGH}) represents the NLI contribution coefficient on the COI from the islands with the same channel as the COI as well as the adjacent channels of the COI in the $f_1$ axis, fulfilling the condition of $\kappa_2=\kappa_1+\kappa_2-\kappa+l$. These islands are marked with blue vertical lines pattern in Fig.~\ref{LT} (a), categorized in the following two groups: 

%\begin{enumerate}[(i)]
%\item
%The lozenge-shaped islands filled with blue in Fig. \ref{LT}(b) where spectral lines $f_1$ and $f'_1$ are located in the the same channel as the COI, while spectral lines $f_2$, $f'_2$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
%\item
%The triangle islands filled with red, light blue and yellow in Fig. \ref{LT}(b) where spectral lines $f_1$ and $f'_1$ are co-located in the adjacent channels of the COI, while spectral lines $f_2$, $f'_2$, $f_3$, and $f_3'$ are co-located in a single interfering channel.
%\end{enumerate}
%The NLI contribution caused by nonlinear interaction between the spectral components pairs leads to the second and fourth order moments of the two involved channels transmit symbols. 

%\subsection{The third EGN correction term--$G_{\kappa}$}

%The third EGN correction term denoted by $G_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the NLI contribution on the COI from the islands with the same channel on  $f_1$ and $f_2$ axes, i.e., fulfilling the condition of $\kappa_1=\kappa_2$. These islands are marked with green grid pattern in Fig.~\ref{LT} (a), categorized in the following two groups: 

%\begin{enumerate}[(i)]
%\item
%The lozenge-shaped and triangle islands filled with green in Fig.~\ref{LT} (b) where spectral lines pairs $(f_1,f'_1)$ and $(f_2,f'_2)$ are located in a certain interfering channel, while the last pair $(f_3,f'_3)$ located in the channel adjacent to this channel.
%\item
%The triangle islands filled with dark blue in Fig. \ref{LT} (b) are the subset of the previous category where spectral lines pairs $(f_1,f'_1)$ and $(f_2,f'_2)$ are located in the same channel as the COI.
%\end{enumerate}
%Therefore, the NLI contribution caused by nonlinear interaction between the spectral pair components leads to second and fourth order moments of the two involved channels transmit symbols. 

%\subsection{The fourth EGN correction term--$H_{\kappa}$}
%The last EGN correction term denoted by $H_{\kappa}$ (see Tabel~\ref{DEFGH}) represents the NLI contribution coefficient on the COI from the islands with the same channel on all the axes, i.e., $\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l$. In these islands, marked with dotted pattern in Fig.~\ref{LT} (a) or equivalently filled pink in Fig.~\ref{LT} (b), the six spectral lines with the assumption of $\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l$ results in six order moments of the involved channel transmit symbols. Here $l=0$ and $l=\pm 1$ indicate the COI and the pink triangle-shaped islands, respectively.


%\section{Interpretation of SCI, XCI, and MCI  contributions}\label{interpretation_NLIN_contribution}
Our main goal, in this section, is to show how {\it{Theorem}}~\ref{main.result} formulates all the NLI terms outright. Before embarking upon the detailed description of the key result, we notice that the same terminology as in \cite[Fig.~7]{carena2014egn} is used in this section. Eq.~\eqref{EGN_fixed} is introduced to evaluate the NLI power on the COI, caused by the following three types of interference: 
\begin{enumerate}[(i)]
\item SCI: The NLI is produced by the COI on itself, i.e., all the interfering spectral components are located in the COI
\item XCI: The NLI is generated by the interfering spectral components located in two different channels, of which one is the COI and another is an interfering channel
\item MCI: The NLI is created by the interfering spectral components located in three or four different channels 
\end{enumerate}
The nonlinear integration regions, shown Fig.~\ref{LT}, would have to be taken into account when the link supports 5 Nyquist rectangular channels and the COI is the fourth channel. The triple summation in \eqref{EGN_fixed} represents these integration regions, with $(\kappa_1,\kappa_2,\kappa_1+\kappa_2-\kappa+l)$ coordinate, implying that the frequencies $f_1$, $f_2$, and $f_1+f_2-f$ are located in $\kappa_1$, $\kappa_2$, and $\kappa_1+\kappa_2-\kappa+l$, resp. We proceed by analyzing the NLI terms.
%As shown in Fig.~\ref{LT}, XCI terms can be categorized into X1 (blue lozenge-shaped islands), X2 (light blue triangle-shaped islands around COI), X3 (dark blue triangle-shaped islands around COI), and X4 (pink triangle-shaped islands) terms. Among these nonlinear terms X1 terms are dominant, also called XPM nonlinear effects. In fact, the XPM terms are the result of nonlinear interaction of spectral pair components $(f_1,f_1')$, $(f_2,f_2')$, and $(f_1+f_2-f,f_1'+f_2'-f)$ when one of these pairs are located in the COI and the other two pairs are co-located in a different interfering channel. As shown in Fig.~\ref{LT}(b), the MCI nonlinear contributions are classified in four M0, M1 M2, and M3 groups. Using the above classification of the nonlinear interference types, we show here how these NLI contributions can be obtained from (\ref{EGN_fixed}).    
\subsubsection{SCI}
The SCI contribution to the NLI is obtained from \eqref{EGN_fixed} when $\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l=\kappa$, leading to $l=0$ and $\kappa_1=\kappa_2=\kappa$ in (\ref{EGN_fixed}). In Fig.~\ref{LT}, for instance, the SCI term, shown as a pink lozenge-shaped island, is obtained from \eqref{EGN_fixed} while $M=2$, $\kappa=\kappa_1=\kappa_2=4$, and $l=0$.
%To obtain an expression for the SCI contributed NLI, we need to consider the NLI caused by the  the COI on itself, leading to solely keep the terms in \eqref{EGN_fixed} generated by spectral lines located in the COI. Therefore, one may need to consider $\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l=\kappa$, leading to $l=0$ and $\kappa_1=\kappa_2=\kappa$ in (\ref{EGN_fixed}). 

\subsubsection{XCI}
As shown in Fig.~\ref{LT}, the XCI terms can be categorized into X1, X2, X3, and X4. We only give the procedure of calculating the X1 term. The same is true for the others. 
%To compute the XCI terms through (\ref{EGN_fixed}), we proceed with the above addressed four types of XCI as follows: 
%\begin{enumerate}
%\item [X1:] 
%The first XCI nonlinear contributions, 
The X1 nonlinear contribution, originated from the nonlinear interaction between $\kappa$ and $\kappa_1$, can be obtained from \eqref{EGN_fixed}  %considering islands with \{$\kappa_1=\kappa_1+\kappa_2-\kappa+l\neq \kappa$, $\kappa_2 = \kappa$\} and \{$\kappa_2=\kappa_1+\kappa_2-\kappa+l\neq \kappa$, $\kappa_1 = \kappa$\}, to realize the above mentioned XPM nonlinear interaction scenarios. Equivalently, we have 
when $\kappa_2=\kappa$, $l=0$ and \{$\kappa_1=\kappa$, $l=0$\}, meaning that
%As a simple example, the XPM NLI contribution on channel $\kappa$ stems from interfering channel $\kappa1$ is obtained by summing up as  
\eqlab{}
{
\sigma_{\text{NLI,},\kappa,\text{XPM}}^{2}=&D_{\kappa}(\kappa_1,\kappa,0)+D_{\kappa}(\kappa,\kappa_2,0)\nonumber\\&+\Phi_{\kappa_1}E_\kappa(\kappa_1,\kappa,0)+\Phi_{\kappa_2}F_\kappa(\kappa,\kappa_2,0).
%+\Phi_{\kappa_1}F_\kappa(\kappa,\kappa_1,0).
}

%\item [X2:] The second XCI type nonlinear contribution can be obtained by considering islands with \{$\kappa_1=\kappa_1+\kappa_2-\kappa+l= \kappa$, $\kappa_2 \neq \kappa$\} and \{$\kappa_2=\kappa_1+\kappa_2-\kappa+l= \kappa$, $\kappa_1 \neq\kappa$\}. Equivalently, this nonlinear term caused by the interfering channel located at the left of the COI can be computed using \eqref{EGN_fixed} by considering islands with \{$l=1$, $\kappa_1=\kappa$,  $\kappa_2=\kappa-1$\} and \{$l=1$, $\kappa_2=\kappa$, $\kappa_1 =\kappa-1$\}. For instance, when channel $\kappa_1=\kappa-1$ at the left side of the COI ($l=1$) is interfering on the COI, the X2 terms is summed up as  
%\eqlab{}
%{
%\sigma_{\text{X2},\kappa}^{2}=&D_{\kappa}(\kappa,\kappa-1,1)+D_{\kappa}(\kappa-1,\kappa,1)+\nonumber\\&\Phi_{\kappa}E_\kappa(\kappa,\kappa-1,1)+\Phi_{\kappa}F_\kappa(\kappa-1,\kappa,1).
%}
%For the X2 nonlinear term originated from the interfering channel located at the right of the COI ($l=-1$), we have
 %\eqlab{}
%{
%\sigma_{\text{X2},\kappa}^{2}=&D_{\kappa}(\kappa,\kappa+1,-1)+D_{\kappa}(\kappa+1,\kappa,-1)+\nonumber\\&\Phi_{\kappa}E_\kappa(\kappa,\kappa+1,-1)+\Phi_{\kappa}F_\kappa(\kappa+1,\kappa,-1).
%}
%We notice here that $l=-1$ and $l=1$ represent the lower and upper triangle islands of each lozenge-shaped islands, respectively. 
%\item [X3:] The third XCI type nonlinear contribution can be obtained by considering islands with \{$\kappa_1= \kappa_2=\kappa$, $\kappa_1+\kappa_2-\kappa+l= \kappa-1$\} and \{$\kappa_1= \kappa_2=\kappa$, $\kappa_1+\kappa_2-\kappa+l=\kappa+1$\}. Equivalently, this nonlinear term can be obtained from \eqref{EGN_fixed} by considering islands originating X3 terms \{$l=-1$, $\kappa_1=\kappa_2=\kappa$\} and  \{$l=1$, $\kappa_1=\kappa_2=\kappa$\}, resulting in 
%\eqlab{}
%{
%\sigma_{\text{X3},\kappa}^{2}=D_{\kappa}(\kappa,\kappa,-1)+\Phi_{\kappa}G_\kappa(\kappa,\kappa,-1)
%} 
%and 
%\eqlab{}
%{
%\sigma_{\text{X3},\kappa}^{2}=D_{\kappa}(\kappa,\kappa,+1)+\Phi_{\kappa}G_\kappa(\kappa,\kappa,+1),
%}
%respectively, for the above simple example.

%\item [X4:] This nonlinear term  originated from islands with \{$\kappa_1= \kappa_2=\kappa_1+\kappa_2-\kappa+l= \kappa-1$\} and \{$\kappa_1= \kappa_2=\kappa_1+\kappa_2-\kappa+l= \kappa+1$\} or equivalently can be obtained from \eqref{EGN_fixed} by considering islands with \{$l=1$, $\kappa_1=\kappa_2=\kappa-1$\} and \{$l=-1$, $\kappa_1=\kappa_2=\kappa+1$\}, respectively, resulting in 
% \eqlab{}
%{
%&\sigma_{\text{X4},\kappa}^{2}=D_{\kappa}(\kappa-1,\kappa-1,1)+\Phi_{\kappa-1}\nonumber\\&E_\kappa(\kappa-1,\kappa-1,+1)+\Phi_{\kappa-1}F_\kappa(\kappa-1,\kappa-1,+1)+\nonumber\\&\Phi_{\kappa-1}G_{\kappa-1}(\kappa-1,\kappa-1,+1)+\Psi_{\kappa_1-1}\nonumber\\&H_\kappa(\kappa-1,\kappa-1,+1),
%}
%and 
 %\eqlab{}
%{
%&\sigma_{\text{X4},\kappa}^{2}=D_{\kappa}(\kappa+1,\kappa+1,-1)+\Phi_{\kappa+1}\nonumber\\&E_\kappa(\kappa+1,\kappa+1,-1)+\Phi_{\kappa+1}F_\kappa(\kappa+1,\kappa+1,-1)+\nonumber\\&\Phi_{\kappa+1}G_\kappa(\kappa+1,\kappa+1,-1)+\Psi_{\kappa+1}\nonumber\\&H_\kappa(\kappa+1,\kappa+1,-1),
%}
%respectively, for the simple example.
%\end{enumerate}
\subsubsection{MCI} 
We can see in Fig.~\ref{LT} that the MCI contributions come from M0, M1, M2, and M4 islands. In what fallows, we only describe how \eqref{EGN_fixed} will give rise to M0. Analogous expression can be held for the rest of MCI terms.

%To address this NLI contribution, we proceed with four types of MCI as follows: 
%\begin{enumerate}
%\item [M0:] 
The M0 NLI effect is originated form interfering spectral components located in four different channels, i.e.,  $\kappa_1\neq \kappa_2\neq\kappa_1+\kappa_2-\kappa+l\neq\kappa$. For example, the impact of the white lozenge-shaped island, marked \# in Fig.~\ref{LT}, on the NLI is obtained from \eqref{EGN_fixed} when $\kappa_1=1$, $\kappa_2=5$, $\kappa_1+\kappa_2-\kappa+l=2$, and $\kappa=4$.}%, and $\kappa_2\neq\kappa_1+\kappa_2-\kappa+l$. 
%In other words, the M0 nonlinear contributions can be obtained from \eqref{EGN_fixed} considering islands with ($\kappa_1,\kappa_2$, $l$), where $\kappa_1\neq\kappa_2$, $\kappa\neq\kappa_2+l$, $\kappa\neq\kappa_1+l$.}
%\end{enumerate}}
%\item [M12:] The M1 and M2 NLI effects are originated form interfering spectral components located in two different channels (which are different from the COI), i. e.,  ($\kappa_1$, $\kappa_2$, $\kappa_1+\kappa_2-\kappa+l$), where \{$\kappa_1=\kappa_1+\kappa_2-\kappa+l\neq\kappa_2$, $\kappa_1\neq\kappa$, $\kappa_2\neq\kappa$\} and \{$\kappa_2=\kappa_1+\kappa_2-\kappa+l\neq\kappa_1$, $\kappa_2\neq\kappa$, $\kappa_1\neq\kappa$\}. As a simple example,
%the M1 and M2 nonlinear contributions can be obtained from \eqref{EGN_fixed} by considering islands with \{$l=-1$, $\kappa_2=\kappa+1\neq\kappa_1$, $\kappa_1\neq\kappa$\}, \{$l=1$, $\kappa_2=\kappa-1\neq\kappa_1$, $\kappa_1\neq\kappa$\}, \{$l=-1$, $\kappa_1=\kappa+1\neq\kappa_2$, $\kappa_2\neq\kappa$\}, and \{$l=1$, $\kappa_1=\kappa-1\neq\kappa_2$, $\kappa_2\neq\kappa$\} in  Fig.~\ref{LT} (b). In this case, the M1 and M2 terms are summing up as   
%\eqlab{}
%{
%&\sigma_{\text{M1,M2},\kappa}^{2}=D_{\kappa}(\kappa_1,\kappa_1+1,-1)+D_{\kappa}(\kappa_1,\kappa-1,1)\nonumber\\&+\Phi_{\kappa_1}E_\kappa(\kappa_1,\kappa_1+1,-1)+\Phi_{\kappa_1-1}F_\kappa(\kappa_1,\kappa-1,1)\nonumber\\&+D_{\kappa}(\kappa+1,\kappa_2,-1)+D_{\kappa}(\kappa-1,\kappa_2,1)\nonumber\\&+\Phi_{\kappa_1}E_\kappa(\kappa_1,\kappa-1,1)+\Phi_{\kappa-2}F_\kappa(\kappa-1,\kappa_2,1).
%}
 
%\item [M3:]This last MCI term contributions can be obtained from \eqref{EGN_fixed} by considering islands with \{$\kappa_1=\kappa_2$, $\kappa_1+\kappa_2-\kappa+l>\kappa+1$, $\kappa_1+\kappa_2-\kappa+l<\kappa-1$\}. Equivalently, the M3 nonlinear contribution can be obtained from \eqref{EGN_fixed} by considering islands with \{$l=0$, $\kappa_1=\kappa_2$, $|\kappa-\kappa_1+\kappa_2-\kappa+l|>1$\}, \{$l=-1$, $\kappa_1=\kappa_2$, $|\kappa-\kappa_1+\kappa_2-\kappa+l|>1$\}, \{$l=1$, $\kappa_1=\kappa_2$, $|\kappa-\kappa_1+\kappa_2-\kappa+l|>1$\} in Fig.~\ref{LT}(b). For the example with two interfering channels located at the left of COI, where channels $\kappa_1$ and $\kappa_1+\kappa_2-\kappa+l=\kappa-2$ are interfering on the COI, and two interfering channels at the right of COI, namely channels $\kappa_1$ and $\kappa_1+\kappa_2-\kappa+l=\kappa+2$ are interfering on the COI, the M3 terms are summing up as 
%\eqlab{}
%{
%&\sigma_{\text{M3},\kappa}^{2}=D_{\kappa}(\kappa-1,\kappa-1,0)+\Phi_{\kappa-1}G_\kappa(\kappa-1,\kappa-1,0)\nonumber\\&+D_{\kappa}(\kappa+1,\kappa+1,0)+\Phi_{\kappa+1}G_\kappa(\kappa+1,\kappa+1,0).
%}
%\end{enumerate}
%\subsection{Comparison with previously introduced SRS models}

%\subsubsection{The frequency domain SRS GN model proposed by Semrau et. al \cite{semrau2018gaussian}}

%Interestingly, the terms $E_\kappa$, $F_\kappa$, $G_\kappa$, and $H_\kappa$ in this model are manifesting as correction terms to the GN model. More precisely, by considering the Gaussian assumption, the EGN model boils down to the GN model \cite{semrau2018gaussian}, resulting in disappearance of these correction terms and solely retaining the term ${D}_\kappa$.

%\subsubsection{The modulation format dependent model proposed by Semrau et. al \cite{semrau2019modulation}}

%Authors of \cite{semrau2019modulation} considered only SCI for  Gaussian signals and XPM for non-Gaussian signal. The SCI term for Gaussian signal therefore obtained through \eqref{EGN_fixed} by ignoring $E_\kappa$, $F_\kappa$, $G_\kappa$, and $H_\kappa$ terms and the interpretation of SCI described in the previous section. The XPM term for non-Gaussian signal is obtained from \eqref{EGN_fixed} by means of the interpretation presented in the previous section.

%\subsubsection{The frequency domain EGN model introduced by Carena et. al \cite{carena2014egn}}

%This model can be reduced to the EGN model presented in \cite{carena2014egn}, which is valid for C-band transmission, by putting $C_r\rightarrow 0$ and $\beta_3\rightarrow 0$ in $\mu(\cdot)$ and $\Phi(\cdot)$, resulting in 
%\eqlab{mu_identical_nosrs}
%{
%&\mu(f_1,f_2,f)=\gamma\frac{1-e^{-2\alpha L}e^{j4\pi^{2}\beta_{2} (f_1-f)(f_2-f)L}}{2\alpha-j4\pi^{2}\beta_{2}(f_1-f)(f_2-f)}.
%}

%\subsubsection{The time domain EGN model introduced by Dar et. al \cite{dar2013properties}}

%The closed form expression for the XPM nonlinear term along with a correction term which takes into account the non-Gaussianity of signal was proposed in \cite[Eqs.(25)--(27)]{dar2013properties}. The extraction of this equation through (\ref{EGN_fixed}) completely coincides with the extraction of X1 terms explained in the previous section with \eqref{mu_identical_nosrs}.

%Fig.~\ref{fig_MDS} shows the NLC of WDM channels  propagated within a link that composed of three different spans, namely two SMF fibers with different lengths and one non-zero dispersion shifted fiber (NZDSF) fiber.
%\section{Conclusion}\label{conclusion}
%An alternative EGN model expression was derived in order to take into account the combined nonlinear effects of SRS and Kerr-nonlinearity for lumped amplification systems with constant attenuation coefficient. The derived model is capable of accounting for the frequency dependent attenuation coefficient. This model can be applied for systems including both C and L bands, namely optical bandwidths beyond Stokes shift, and hybrid amplification systems as well. It was shown that the NLI being increased for channels endure net SRS gain and being decreased for channels endure net SRS loss. Moreover, we found that the nonlinear interference (NLI) varience deviation is increased and decreased exponentially, for low frequency and high frequency channels when the input launch power increases. On the other hand, the NLI variance deviations remain invariable except for high launch powers.

%The model is accurate for a wide range of modulation formats. Indeed, we remove the Gaussianity assumption of signal to derive an exact modulation format dependent EGN model in the presence of SRS. We show that Gaussian modulation experiences higher NLI than the other modulation formats, i.e., SRS GN model overestimates the nonlinear interference.
%The general EGN model has opened up a new horizon for efficient optimization of ultra-widebands systems.


==> Lemma1.2.tex <==
\section{Proof of Theorem \ref{main.result}}\label{AppendixB}

This appendix contains two sections. In the first section, we derive the nonlinear electrical field in \eqref{MAN_NLI_sol} at the end of a link with multiple different spans. The second section provides the derivation of the NLI PSD in \eqref{SpecDensityDP_Def}, which is then used to compute the nonlinear power via \eqref{NLI_Power_Channel_Kappa}.
%This appendix addresses derivation of the the NLI power of a certain channel \eqref{NLI_Power_Channel_Kappa}, starting from the NLI PSD on polarization x \eqref{G_x_Def}.
%\eqlab{G_x_Def}
%{
%G_{\small{\text{NLI}},\text{x},\kappa}(f)=\mathbb{E}\big\{E_{\text{x},\kappa}^{(1)}(f)\text{e}^{(1)*}_{\text{x},\kappa}(f)\big\},
%}
 %where $E_{\text{x},\kappa}^{(1)}(f)$ is provided assuming that the nonlinear electrical filed of each span propagates solely linearly until arrives at the output of the link. This assumption is driven by the perturbation approach. The linear propagation of the nonlinear electrical fields of the different link spans at the receiver are summed up coherently.
 \subsection{Nonlinear Electrical Field}% at the end of fiber}
 
In this section we first derive the nonlinear electrical field at the end of first span (Lemma~\ref{NLI_field_first_span} ahead). We then extend it to multiple different spans (Lemma~\ref{multiple.span.extention} ahead).
\begin{lemma}[Nonlinear Field: First Span]\label{NLI_field_first_span}
The nonlinear electrical field at the end of the first span of length $L_1$ is given by
\begin{equation}\label{NLIN_expression}
\begin{split}
&E_{\text{x},\kappa}^{(1)}(L_{1},f)=-j\gamma\frac{8}{9}f_0^{3/2}\text{e}^{\tilde{\Gamma}(L_{1},f)}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta(f-if_0-(\kappa-l)R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k),
\end{split}
\end{equation}
where  
 \begin{equation}\label{Zeta_ENL}
 \begin{split}
\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k)=&\int_{0}^{L_{1}}\text{d}z'\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}\\&\cdot \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
\end{split}
\end{equation}
in which
\begin{equation}\label{varrho}
\begin{split}
&\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')=\rho(z',mf_0+\kappa_1 R)\\&\cdot\frac{\rho(z',nf_0+(\kappa_1+\kappa_2-\kappa+l)R)\rho(z',kf_0+\kappa_2 R)}{\rho(z',(m+k-n)f_0+(\kappa-l)R)},
\end{split}
\end{equation}
and
 \begin{equation}\label{phi}
 \begin{split}
&\phi_{m,n,k}(\kappa_1,\kappa_2,\kappa)=4\pi^{2}\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\Big[\beta_{2,1}+\pi\beta_{3,1}\\&\cdot\big[(m+k)f_0+(\kappa_1 +\kappa_2 )R\big]\Big]z',
\end{split}
 \end{equation}
 where $\tilde{\Gamma}(\cdot)$, $\xi$, and $\rho(\cdot)$ defined in \eqref{gamma.tilde}, \eqref{FourierSerisCoef1}, and \eqref{rho}, respectively.
\end{lemma}
\begin{IEEEproof}
The nonlinear electrical field ${\boldsymbol{E}}^{(1)}(z,f)$ is given by \eqref{MAN_NLI_sol}, which depends on the Kerr term ${\boldsymbol{Q}}(z,f)$ in \eqref{F_kerr}, which in turn depends on the linear solution of the Manakov equation ${\boldsymbol{E}}^{(0)}(z,f)$. The x-polarization part of the latter can be expressed as
\eqlab{Lin_electrical_z}{
E_{\text{x}}^{(0)}(z,f)=\sqrt{f_0}\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa=1}^{M}\sum_{n=-\infty}^{\infty}\xi_{\text{x},\kappa,n}\delta(f-nf_0-\kappa R),
}
where we used \eqref{FouierSeries} in \eqref{E_input} and in \eqref{MAN_LIN_sol}.

By using \eqref{Lin_electrical_z} into \eqref{F_kerr}  yields
\eqlab{eq_6_1}{
&Q_{\text{x},\kappa}(z,f)=-j\gamma\frac{8}{9}\Big[\nonumber\\
&f_0\Big(\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}\xi_{\text{x},\kappa_1,m}\delta(f-mf_0-\kappa_1R)\Big)\nonumber\\
&*\Big(\text{e}^{\tilde{\Gamma}^*(z,f)}\sum_{\kappa'=1}^{M}\sum_{n=-\infty}^{\infty}\xi^*_{\text{x},\kappa',n}\delta(-f-nf_0-\kappa'R)\Big)+ \nonumber\\
&f_0\Big(\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}\xi_{\text{y},\kappa_1,m}\delta(f-mf_0-\kappa_1R)\Big)\nonumber\\
&\Big(\text{e}^{\tilde{\Gamma}^*(z,f)}\sum_{\kappa'=1}^{M}\sum_{m=-\infty}^{\infty}\xi^*_{\text{y},\kappa',n}\delta(-f-nf_0-\kappa'R)\Big)\Big]*\nonumber\\
&\sqrt{f_0}\Big(\text{e}^{\tilde{\Gamma}(z,f)}\sum_{\kappa_2=1}^{M}\sum_{k=-\infty}^{\infty}\xi_{\text{x},\kappa_2,k}\delta(f-kf_0-\kappa_2R)\Big).
}
We now use the property
\eqlab{delta.property}{
&a(f)\delta(f-f_a)*b(f)\delta(-f-f_b)*c(f)\delta(f-f_c)=\nonumber\\&a(f_a)b(f_b)c(f_c)\delta(f-(f_a-f_b+f_c)),
}
to express \eqref{eq_6_1} as
\begin{equation}\label{eq_6_1_1}
\begin{split}
&Q_{\text{x},\kappa}(z,f)=-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{\kappa'=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{ m=-\infty}^{\infty}\sum_{n=-\infty}^{\infty}\sum_{ k=-\infty}^{\infty}\\&\cdot\delta\big(f-(m-n+k)f_0-(\kappa_1-\kappa'+\kappa_2) R\big)\\&\cdot\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+\kappa' R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
\end{split}
\end{equation}
We are interested in the NLI in channel $\kappa$, which imposes the  constraint on the interfering  frequency $if_0+\tau R$ 
%Similar to \cite{carena2014egn,MecozziEssiambre2012,Pontus_JLT_modeling_2013} we remove the triplets 
%where $m=n$ and $n=k$ because they create bias and non-fluctuating terms (see Lemma~\ref{bias.terms} ahead in the next section). We therefore define the non-bias triplets as
\begin{equation}\label{si}
\mathcal{S}_i=\left\{(m,n,k)\in\mathbb{Z}^3:\kappa R-\frac{R}{2}\leq if_0+\tau R\leq \kappa R+\frac{R}{2}\right\},
\end{equation}
where $i=m-n+k$ and $\tau=\kappa_1-\kappa'+\kappa_2$.
%\eqlab{f.constraint}{
%\kappa R-R/2\leq f \leq\kappa R +R/2.} 
In other words, for given values of $\kappa_1,\kappa',\kappa_2$,  only certain values of $m,n,k$ are allowed, namely those in the set $\mathcal{S}_i$.
 Using \eqref{si}, \eqref{eq_6_1_1} is expressed as
\begin{equation}\label{eq_6_si}
\begin{split}
&Q_{\text{NLI,x},\kappa}(z,f)=
-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{N}\sum_{\kappa'=1}^{N}\sum_{\kappa_2=1}^{N}\sum_{i=-\infty}^{\infty}\\
&\cdot\delta(f-if_0-\tau R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}+\\
&\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa',n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\
&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+\kappa' R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
\end{split}
\end{equation}
%Since $-R/2\leq nf_0\leq R/2$, we find that $-3/2R\leq(m-n+k)f_0\leq3/2R$, and hence
%According to \eqref{FouierSeries}--\eqref{f0.constraint} given in Sec.~\ref{preliminaries},  $nf_0+\kappa R$ is a frequency component within channel $\kappa$. The same is true for \eqref{eq_6_1} in which $mf_0+\kappa_1R$, $nf_0+\kappa'R$, and $kf_0+\kappa_2R$ are the frequency components within channels $\kappa_1$, $\kappa'$, and $\kappa_2$, respectively, where
The expression \eqref{FourierSerisCoef1} shows that $nf_0+\kappa R$ corresponds to the frequency components within channel $\kappa$. Because of this, $nf_0$ should satisfy \eqref{f0.constraint}. A similar interpretation can be used on $mf_0+\kappa_1R$, $nf_0+\kappa'R$, and $kf_0+\kappa_2R$ in \eqref{eq_6_1}, and thus,
\begin{align*}
-\frac{R}{2}\leq mf_0 \leq \frac{R}{2},\quad
-\frac{R}{2}\leq nf_0 \leq\frac{R}{2},\quad
-\frac{R}{2}\leq kf_0 \leq\frac{R}{2}.
\end{align*}
By combining these inequalities we get $-3/2R\leq(m-n+k)f_0 \leq3/2R$, which implies that
%We now combine \eqref{f0.constraint} and \eqref{f.constraint} to obtain $-3/2R\leq(m-n+k)f_0\leq3/2R$ [THIS IS NOT TRUE. PLEASE FIX IT. What equations do you combine to get $-3/2R\leq(m-n+k)f_0\leq3/2R$?]
\begin{equation}\label{interference_limit}
-\frac{3}{2}R
+\tau R \leq if_0+\tau R \leq \frac{3}{2}R
+\tau R.
\end{equation}
Combining the inequalities in the definition of the set $\mathcal{S}_i$ in \eqref{si} with \eqref{interference_limit}, we obtain\footnote{To obtain \eqref{boundary.kappa'}, we use the fact that for any $a,b,c,x
\in\mathbb{R}$ the two inequalities $b-a/2\leq x \leq b+a/2$ and $-3a/2+c\leq x \leq 3a/2+c$, imply that $b>-2a+c$ and $b<2a+c$.}
% \begin{equation}\label{interfernce_bound}
% \begin{split}
% &\kappa R+\frac{R}{2}>-\frac{3}{2}R
% +(\kappa_1-\kappa'+\kappa_2)R,\\&\kappa R-\frac{R}{2}<\frac{3}{2}R
% +(\kappa_1-\kappa'+\kappa_2)R,
% \end{split}
% \end{equation}
% and thus,
\eqlab{boundary.kappa'}{
&\kappa-2<\kappa_1-\kappa'+\kappa_2<\kappa+2.
}
The expression in \eqref{boundary.kappa'} in turn implies that for given values of $\kappa,\kappa_1,$ and $\kappa_2$, $\kappa'$ can only take the following three values
\eqlab{kappa'.l}{
\kappa'=\kappa_1+\kappa_2-\kappa+l, \quad l=-1,0,1.%\\&
%\kappa'=\kappa_1+\kappa_2-\kappa+0,\\&
%\kappa'=\kappa_1+\kappa_2-\kappa+1,
}
% thereby 
% (\ref{eq_6_si}) which has the overall form
% \eqlab{eq_6_si_alternative1}{
% Q_{\text{NLI,x},\kappa}(z,f)=\sum_{\kappa_1=1}^{N}\sum_{\kappa'=1}^{N}\sum_{\kappa_2=1}^{N}X_{\kappa_1}(z,f)Y_{\kappa'}(z,f)Z_{\kappa_2}(z,f),
% }
% can be written as
% \eqlab{eq_6_si_alternative2}{
% Q_{\text{NLI,x},\kappa}(z,f)=&\sum_{\kappa_1=1}^{N}\sum_{\kappa_2=1}^{N}\sum_{\l=-1}^{1}X_{\kappa_1}(z,f)Y_{\kappa_1+\kappa_2-\kappa+l}(z,f)\nonumber\\&Z_{\kappa_2}(z,f),
% }
Using \eqref{kappa'.l}, we express \eqref{eq_6_si} as
\begin{equation}\label{qx_2}
\begin{split}
&Q_{\text{x},\kappa}(z,f)=-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
\end{split}
\end{equation}
%and its y-polarization counterpart is
%\footnote{Without loss of generality we indexed the second terms of \eqref{qx_2} and \eqref{qy_2} in the following form
%\eqlab{indexing}{
%&\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k},\nonumber\\&
%\xi_{\text{y},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k},
%}
%because in the next section we show that to calculate the NLI PSD the first and second terms of \eqref{indexing} result in 
%\eqlab{indexing.moments1}{
%&\mathbb{E}\{\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{y},\kappa_1,m}^{*}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}\}\nonumber\\&\cdot\mathbb{E}\{\xi_{\text{x},\kappa_2,k}\xi_{\text{x},\kappa_2,k}^{*}\},
%}
%and
%\eqlab{indexing.moments2}{
%&\mathbb{E}\{\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1,m'}^{*}\}\cdot\nonumber\\&\mathbb{E}\{\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n'}^{*}\xi_{\text{x},\kappa_1,k}\xi_{\text{x},\kappa_1,k'}^{*}\},
%}
%respectively. As can be seen in \eqref{indexing.moments1} the second expectation, which yields the second order moments, is taken over channel $\kappa_2$, whereas in \eqref{indexing.moments2} the first expectation that results in the second order moments, is taken over channel $\kappa_1$.
%}
%\begin{equation}\label{qy_2}
%\begin{split}
%&Q_{\text{y},\kappa}(z,f)=-j\gamma\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{y},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}(z,mf_0+\kappa_1 R)+\tilde{\Gamma}^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}(z,kf_0+\kappa_2 R)}.
%\end{split}
%\end{equation}
We now use \eqref{qx_2} in \eqref{MAN_NLI_sol} to obtain the nonlinear electrical field on x-polarization at the end of the first fiber span of length $L_{1}$, which gives
%\eqref{NLIN_expression_x_1}.
%\eqref{NLIN_expression}.
%\begin{figure*}
%\small
\begin{equation}\label{NLIN_expression_x_1}
\begin{split}
&E_{\text{x},\kappa}^{(1)}(L_{1},f)=-j\gamma\frac{8}{9}f_0^{3/2}\text{e}^{\tilde{\Gamma}(L_{1},f)}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta(f-if_0-(\kappa-l)R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}
\Big)\int_{0}^{L_1}\text{d}z'\\&\cdot \text{e}^{\tilde{\Gamma}(z',mf_0+\kappa_1 R)}\cdot\text{e}^{\tilde{\Gamma}^*(z',nf_0+(\kappa_1+\kappa_2-\kappa+l) R)}\\&\cdot\text{e}^{\tilde{\Gamma}(z',kf_0+\kappa_2 R)}\cdot\text{e}^{-\tilde{\Gamma}(z',(m-n+k)f_0+(\kappa-l)R)},
\end{split}
\end{equation}
where in the last exponential we replaced $f$ by $(m-n+k)f_0+(\kappa-l)R$ due to the delta function $\delta(f-if_0-(\kappa-l)R)$ multiplying the sum and integral in \eqref{NLIN_expression_x_1}. 

The last part of the proof is to show that the integral in \eqref{NLIN_expression_x_1} can be expressed as \eqref{Zeta_ENL} and \eqref{varrho}. We do this by first 
%\hrulefill
%\end{figure*}
substituting \eqref{gamma} into \eqref{gamma.tilde}, and taking exponentials on both sides of the resulting equation gives
% we have
% \eqlab{gamma.tilde.expansion}{
% \tilde{\Gamma}(z,f)=\int_{0}^{z}\text{d}z'\Big[\frac{g(z',f)}{2}+j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3\Big],
% }
% and therefore,
\begin{align}
\label{exp.gamma.tilde.expansion}
\text{e}^{\tilde{\Gamma}(z,f)}&=\text{e}^{\frac{1}{2}\int_{0}^{z}\text{d}z'g(z',f)}\cdot\text{e}^{\int_{0}^{z}\text{d}z'[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]}\\
\label{exp.gamma.tilde.expansion.2}
&=\sqrt{\rho(z,f)} \cdot\text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z}
\end{align}
where the first term in \eqref{exp.gamma.tilde.expansion.2} follows from the definition of the normalized signal power profile definition in \eqref{rho.1} and the second from the fact that $\beta_{2,1}$ and $\beta_{3,1}$ are $z$-indepent.% the first term is equal to
%\eqlab{first.term.gamma.tilde}{
%\text{e}^{\int_{0}^{z}\text{d}z'\frac{g(z',f)}{2}}=, %\quad \text{and}\nonumber\\&
%\text{e}^{-\int_{0}^{z}\text{d}z'\frac{g(z',f)}{2}}=\frac{1}{\sqrt{\rho(z,f)}},
%}

%and the second term is 
%\eqlab{second.third.exp.gamma.tilde}{
%\text{e}^{\int_{0}^{z}\text{d}z'[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]}=\text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z}.
%%}
%By inserting \eqref{first.term.gamma.tilde} and \eqref{second.third.exp.gamma.tilde} into \eqref{exp.gamma.tilde.expansion}, we get
%\eqlab{exp.gamma.tilde.expansion.2}{
%\text{e}^{\tilde{\Gamma}(z,f)}=\sqrt{\rho(z,f)}\cdot \text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z},
%}

We now use \eqref{exp.gamma.tilde.expansion.2} to express the integral in \eqref{NLIN_expression_x_1} as
\eqlab{last.four.terms.exp.gamma}{
&\int_{0}^{L_1}\text{d}z'\text{e}^{\tilde{\Gamma}(z',mf_0+\kappa_1 R)}\cdot\text{e}^{\tilde{\Gamma}^*(z',nf_0+(\kappa_1+\kappa_2-\kappa+l) R)}\nonumber\\&\cdot\text{e}^{\tilde{\Gamma}(z',kf_0+\kappa_2 R)}\cdot\text{e}^{-\tilde{\Gamma}(z',(m-n+k)f_0+(\kappa-l)R)}=\nonumber\\&
\int_{0}^{L_1}\text{d}z'\sqrt{\rho(z',mf_0+\kappa_1 R)}\nonumber\\&\cdot\frac{\sqrt{\rho(z',nf_0+(\kappa_1+\kappa_2-\kappa+l)R)}\sqrt{\rho(z',kf_0+\kappa_2 R)}}{\sqrt{\rho(z',(m-n+k)f_0+(\kappa-l)R)}}\nonumber\\&\cdot
\text{e}^{[j2\pi^{2}\beta_{2,1} (mf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}(mf_0+\kappa_1R)^3]z'}
\nonumber\\&
\text{e}^{[-j2\pi^{2}\beta_{2,1} (nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}-j\frac{4}{3}\pi^3 \beta_{3,1}(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^3]z'}
\nonumber\\&
\text{e}^{[j2\pi^{2}\beta_{2,1} (kf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}(kf_0+\kappa_2R)^3]z'}
\nonumber\\&
\text{e}^{[-j2\pi^{2}\beta_{2,1} (( m-n+k)f_0+(\kappa-l)R)^{2}-j\frac{4}{3}\pi^3 \beta_{3,1}((m-n+k)f_0+(\kappa-l)R)^3]z'}.
}
% in which we are using the fact that
% \eqlab{exp.gamma.tilde.expansion.3.minus}{
% \text{e}^{-\tilde{\Gamma}(z,f)}= \frac{\text{e}^{[j2\pi^{2}\beta_{2,1} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,1}f^3]z}}{\sqrt{\rho(z,f)}}.
% }
We recognize the $\rho(\cdot)$ terms in the right hand side of \eqref{last.four.terms.exp.gamma} as $\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}$,
% \eqlab{last.four.terms.exp.gamma.rho.terms}{
% &
% \sqrt{\rho(z',mf_0+\kappa_1 R)}\cdot\sqrt{\rho(z',nf_0+(\kappa_1+\kappa_2-\kappa+l)}\nonumber\\&\cdot\frac{\sqrt{\rho(z',kf_0+\kappa_2 R)}}{\sqrt{\rho(z',(m-n+k)f_0+(\kappa-l)R)}}=\nonumber\\&\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
% }
where $\varrho(\cdot)$ is given by \eqref{varrho}. In view of \eqref{Zeta_ENL}, the last step in the proof is therefore to show that
%Considering \eqref{rho}, it is straightforward that
%\eqlab{e.rho}{
%&\text{e}^{\int_{0}^{z’}\text{d}z” \frac{g(z”,mf_0+\kappa_1R)}{2}
%+\int_{0}^{z’}\text{d}z” \frac{g(z”,mf_0+\kappa_1R)}{2}+\int_{0}^{z’}\text{d}z” \frac{g(z”,mf_0+\kappa_1R)}{2}}\nonumber\\&\cdot
%\text{e}^{\int_{0}^{z’}\text{d}z” \frac{g(z”,(m-n+k)f_0+(\kappa-l)R)}{2}
%}
%\nonumber\\&=\int_{0}^{L_{1}}\text{d}z'\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
%}
%where $\varrho(\cdot)$ is given by \eqref{varrho}.
%On the other hand, using the fact that
%\eqlab{beta2.beta3.expansion}{
%& A^2-B^2+C^2-(A-B+C)^2=\nonumber\\&
%2(A-B)(C-B),\nonumber\\&
%A^3-B^3+C^3-(A-B+C)^3=\nonumber\\&3(A+C)(A-B)(C-B),
%}
%it is found that
the arguments of the four exponentials in \eqref{last.four.terms.exp.gamma} corresponds to \eqref{phi}. We do this by first grouping the quadratic and cubic terms in the exponentials in \eqref{last.four.terms.exp.gamma} as
\eqlab{beta2.beta3.expon}{
%&\text{e}^{[j2\pi^{2}\beta_2 (mf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_3(mf_0+\kappa_1R)^3]z’}
%\nonumber\\&
%\text{e}^{[-j2\pi^{2}\beta_2 (nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}-j\frac{4}{3}\pi^3 \beta_3(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^3]z’}
%\nonumber\\&
%\text{e}^{[j2\pi^{2}\beta_2 (kf_0+\kappa_1R)^{2}+j\frac{4}{3}\pi^3 \beta_3(kf_0+\kappa_2R)^3]z’}
%\nonumber\\&
%&\text{e}^{[-j2\pi^{2}\beta_2 (( m-n+k)f_0+(\kappa-l)R)^{2}-j\frac{4}{3}\pi^3 \beta_3( m-n+k)f_0+(\kappa-l)R)^3]z’}\nonumber\\&=
&\text{exp}\Big(j2\pi^{2}\beta_{2,1}z'\Big[ (mf_0+\kappa_1R)^{2}- (nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}\nonumber\\&+ (kf_0+\kappa_1R)^{2}- (( m-n+k)f_0+(\kappa-l)R)^{2}\Big]\Big)\nonumber\\&\cdot
\text{exp}\Big(j\frac{4}{3}\pi^3 \beta_{3,1}z'\Big[(mf_0+\kappa_1R)^3-\nonumber\\&(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^3+(kf_0+\kappa_2R)^3\nonumber\\&-( m-n+k)f_0+(\kappa-l)R)^3\Big]\Big).
}
We now use the equality
\begin{align*}
& A^2-B^2+C^2-(A-B+C)^2=
2(A-B)(C-B),
\end{align*}
to express the first exponential term in \eqref{beta2.beta3.expon} as
\eqlab{first.exponential.beta2}{
&\text{exp}\Big(j4\pi^{2}\beta_{2,1}z'\Big[ 
\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\nonumber\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\Big]\Big).
}
We also use
\begin{align*}
A^3-B^3+C^3-&(A-B+C)^3\\
&=3(A-B)(C-B)(A+C),
\end{align*}
to express the second exponential term in \eqref{beta2.beta3.expon} as
\eqlab{second.exponential.beta2}{
&\text{exp}\Big(j4\pi^3\beta_{3,1}z'\Big[\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\nonumber\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\nonumber\\&\cdot\Big((m+k)f_0+(\kappa_1 +\kappa_2 )R\Big)\Big]\Big).
}
The proof is completed by multiplying \eqref{first.exponential.beta2} and  \eqref{second.exponential.beta2} yielding the required exponential in \eqref{phi}.

%terms of %\eqref{beta2.beta3.expon}, 
%we find that \eqref{beta2.beta3.expon} can be rewritten as
% \eqlab{e.phi}{
%  \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
%  }
% %\text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}
% where $\phi(\cdot)$ is given by \eqref{phi}, and hence \eqref{last.four.terms.exp.gamma} is expressed as \eqref{Zeta_ENL}
% As a result, replacing the integral term of \eqref{NLIN_expression_x_1} (i.e., \eqref{last.four.terms.exp.gamma.rho.terms}) by \eqref{Zeta_ENL}  results in \eqref{NLIN_expression}.
%Now, considering \eqref{e.rho}, \eqref{beta2.beta3.expon}, and \eqref{exp.expression} and substituting \eqref{exp.expression} in \eqref{NLIN_expression_x_1}, we obtain \eqref{NLIN_expression}. 
%This completes the proof.
\end{IEEEproof}
%\begin{equation}\label{NLIN_expression}
%\begin{split}
%&E_{\text{x},\kappa}^{(1)}(L_{1},f)=-j\gamma\frac{8}{9}f_0^{3/2}\text{e}^{\tilde{\Gamma}(L_{1},f)}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\cdot\delta(f-if_0-(\kappa-l)R)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k),
%\end{split}
%\end{equation}
%where  
% \begin{equation}\label{Zeta_ENL}
% \begin{split}
%\zeta_{\kappa_1,\kappa_2,\kappa}(m,n,k)=&\int_{0}^{L_{1}}\text{d}\varsigma\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,\varsigma)}\\&\cdot \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,\varsigma)},
%\end{split}
%\end{equation}
%in which
%\begin{equation}
%\begin{split}
%&\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,\varsigma)=\rho(\varsigma,mf_0+\kappa_1 R)\\&\cdot\rho(\varsigma,nf_0+(\kappa_1+\kappa_2-\kappa+l)R)\rho(\varsigma,kf_0+\kappa_2 R)\\&\cdot\frac{1}{\rho(\varsigma,(m+k-n)f_0+(\kappa-l)R)},
%\end{split}
%\end{equation}
%with
%\begin{equation}
%\rho(z,f)=\text{e}^{\int_{0}^{z}\text{d}z' g(z',f)},
%\end{equation}
%and
 %\begin{equation}\label{phi}
 %\begin{split}
%&\phi_{m,n,k}(\kappa_1,\kappa_2,\kappa)=4\pi^{2}\Big((m-n)f_0+(\kappa-\kappa_2-l)R\Big)\\&\cdot\Big((k-n)f_0+(\kappa-\kappa_1-l)R\Big)\Big[\beta_{2,1}+\pi\beta_{3,1}\\&\cdot(mf_0+kf_0+\kappa_1 R+\kappa_2 R)\Big]\varsigma.
%\end{split}
% \end{equation}

 We now extend Lemma~\ref{NLI_field_first_span} to multiple different spans.
 \begin{lemma}[Nonlinear Field: Multiple Spans]\label{multiple.span.extention}
 The total nonlinear electrical field at the end of a link with $N$ multiple different spans can be written as
%\subsubsection{Nonlinear Electrical Field}\label{nonlinear solution}
%\eqlab{E_f}
%{
%{\bf E}_{\text{LIN}}(0,f)=\sum_{\kappa=1}^{N}{\bf A}_{\kappa}(f).
%} 
%To compensate for the fiber attenuation, an Erbium doped fiber amplifier (EDFA) is exploited at the end of each span, e. g., an EDFA with a gain of $g_{s}$ at span $s$. The nonlinear electrical field of channel $\kappa$ on x-polarization (readily can be written for y-polarization as well), denoted by $E_{\text{NLI},\text{x},\kappa}$, at the output of the link, i. e., is computed after the last EDFA amplifier in the last span $N$, as depicted in Fig.~\ref{Multi_span}. The derivation details of $E_{\text{NLI},\text{x},\kappa}$ is provided in Appendix \ref{AppendixA}, resulting in 
\eqlab{NLI_elec_tot_detail}
{
&E_{\text{x},\kappa}^{(1)}({\scriptstyle{\sum_{s'=1}^{N}\!L_{s'}}},f)\!=\!-j\frac{8}{9}f_0^{3/2}  \sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\nonumber\\&\delta\big(f\!-\!if_0\!-(\kappa-l)\big)\!\!\sum_{m,n,k\in \mathcal{S}_i}
\big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}+\nonumber\\&\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\varsigma_{{\kappa_1},\kappa_2,\kappa}(m,n,k)\nonumber\\&\
\text{e}^{-j2\pi^{2}(if_0+(\kappa-1)R)^{2}\sum_{s=1}^{N}(\beta_{2,s}L_{s}+\frac{2}{3}\pi(if_0+(\kappa-1)R)L_{s})} ,
}
where $\sum_{s'=1}^{N}\!L_{s'}$ is the total length of link and
\eqlab{varsigma}
{
&\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,k)=\sum_{s=1}^{N}\gamma_{s}g_{s}^{1/2}\sqrt{\rho(z,if_0+(\kappa-l)R)}\nonumber\\&\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2}\prod_{s'=s}^{N}[g_{s'}\cdot\rho(L_{s'},f)]^{1/2}\zeta_{\kappa_1,\kappa_2,\kappa}^{s}(m,n,k)\nonumber\\&\text{exp}\Big(j4\pi^{2}\big((m-n)f_0+(\kappa-\kappa_2-l)R\big) \big((k-n)f_0+\nonumber\\&(\kappa-\kappa_1-l)R\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}+\pi[(m+k)f_0+\nonumber\\&(\kappa_1+\kappa_2)R]\beta_{3,s'}L_{s'}\Big),
}
in which
\eqlab{Zeta_ENL_s}{
\zeta^{s}_{\kappa_1,\kappa_2,\kappa}(m,n,k)=&\int_{0}^{L_{s}}\text{d}z'\sqrt{\varrho_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')}\\&\cdot \text{e}^{j\phi_{\kappa_1,\kappa_2,\kappa}(m,n,k,z')},
}
where $g_{s}$ is the gain of amplifier located at the end of span $s$, $\varrho(\cdot)$ and $\phi(\cdot)$ are given in \eqref{varrho} and \eqref{phi}, respectively.
\end{lemma}
 
 \begin{IEEEproof}
 To evaluate the nonlinear electrical field of channel $\kappa$ at the end of the link with multiple different spans, similar to \cite{Carena2012}, we assume that the nonlinear contributions that distort channel $\kappa$ in each span propagate linearly in the following spans until arrive at the receiver. 
%Two approaches can be attended to sum all these nonlinear contributions at the receiver. One may sum the nonlinear contributions generated in each span at the receiver in power, namely in incoherent manner, 
%while the other way which is considered in this paper,
We sum all the nonlinear contributions generated in each span at the receiver coherently. In other words, the nonlinear electrical field of channel $\kappa$ at the end of the link with $N$ different spans is equal to
\eqlab{NLI_elec_tot}
{
E_{\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f)=\sum_{s=1}^{N}E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f),
}
where $E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f)$ is the nonlinear electrical field of channel $\kappa$ at the receiver that generated in span $s$.
In order to evaluate the nonlinear electrical field of channel $\kappa$ that generated in span $s$, we assume that the signal propagates linearly in the first $s-1$  spans, namely the linear electrical field at the input of span $s$ is
\eqlab{LIN_elec_span}{
E_{s,\text{x}}^{(0)}({\scriptstyle\sum_{s'=1}^{s-1}L_{s'}},f)&=\prod_{s'=1}^{s-1}\sqrt{g_{s'}}\cdot\text{e}^{\tilde{\Gamma}_s(L_{s'},f)}E_{\text{x}}(0,f),
}
where
\eqlab{gamma.tilde.s}{
\tilde{\Gamma}_s(z,f)=\int_{0}^{z}\text{d}z'{\Gamma}_s(z',f),
}
in which
\begin{equation}\label{gamma.s}
{\Gamma}_s(z,f)=\frac{g(z,f)}{2}+j2\pi^{2}\beta_{2,s} f^{2}+j\frac{4}{3}\pi^3 \beta_{3,s}f^3. 
\end{equation}
and $E_{\text{x}}(0,f)$ is given by \eqref{E_input} and \eqref{FouierSeries}.
This equation represents that the electrical field that passes through $s-1$ spans simply influenced by dispersions of spans, span losses, and amplifier gains. The linear field in the span $s$ can then be written as
\eqlab{LIN_elec_z}{
&E_{s,\text{x}}^{(0)}(z,f)=\text{e}^{\tilde{\Gamma}_s(z,f)}E_{s,\text{x}}^{(0)}({\scriptstyle\sum_{n_s'=1}^{s-1}L_{s'}},f),
}
By inserting \eqref{LIN_elec_z} %$\text{e}^{\tilde{\Gamma}(z,f)}$ %from \eqref{exp.gamma.tilde.expansion} 
into \eqref{F_kerr},
%we obtain 
%\eqlab{Lin.elec.z.expansion}{
%&
%E_{s,\text{x}}^{(0)}(z,f)=\nonumber\\&\text{e}^{-j2\pi^{2} f^{2}[\sum_{s'=1}^{s-1}(\beta_{2,s}L_{s'}+\frac{2}{3}\pi f \beta_{3,s'}L_{s'})+(\beta_{2,s'}z+\frac{2}{3}\pi f \beta_{3,s'}z)]}\nonumber\\&\prod_{s'=1}^{s-1}g_{s'}^{1/2}\text{e}^{\alpha_{s'}L_{s'}}\cdot\sqrt{\rho(z,f)}E_{\text{x}}(0,f).
%}
%We now substitute \eqref{Lin.elec.z.expansion} into the Kerr term \eqref{F_kerr}, and
we get
\eqlab{Kerr-term2}
{
&{\boldsymbol{Q}}_s(z,f)=j\gamma_s\frac{8}{9}\Big[E_{s,\text{x}}^{(0)}(z,f)*E_{s,\text{x}}^{(0)\scriptsize{*}}(z,-f)+\nonumber\\&E_{s,\text{y}}^{(0)}(z,f)*E_{s,\text{y}}^{(0)\scriptsize{*}}(z,-f)\Big]*{\boldsymbol{E}_s}^{(0)}(z,f).
}
Using \eqref{kappa'.l} the Kerr term in span $s$ \eqref{Kerr-term2} can be expressed like \eqref{qx_2}, with two minor differences. One is the the product term in \eqref{kerr.ter.span.s}, which is responsible for taking into account the amplifiers' gain and loss of previous spans. The second is the last exponential term in \eqref{kerr.ter.span.s} which is responsible for taking into account the second and third order dispersion of the previous spans.
\begin{figure*}[t]
\scriptsize
\eqlab{kerr.ter.span.s}{
&Q_{s,\text{x},\kappa}(z,f)=-j\gamma_{s}\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2} %\text{e}^{\Gamma(z,if_0+(\kappa-l))}
\sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\delta\big(f\!-\!if_0\!-(\kappa-l)\big)\sum_{m,n,k\in \mathcal{S}_i}\big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\nonumber\\&+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\text{e}^{\tilde{\Gamma}_s(z,mf_0+\kappa_1 R)+\tilde{\Gamma}_s^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}_s(z,kf_0+\kappa_2 R)} \nonumber\\&
\cdot\text{e}^{-j2\pi^{2}\big((mf_0+\kappa_1R)^2-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}+(kf_0+\kappa_2R)^{2}\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}-j\frac{4}{3}\pi^{3}\big((mf_0+\kappa_1R)^3-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{3}+(kf_0+\kappa_2R)^{3}\big)\sum_{s'=1}^{s-1}\beta_{3,s'}L_{s'}}
}.
\hrulefill
\end{figure*}
%=\nonumber\\&
%-j\gamma_s\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}g_{s'}^{3/2}\text{e}^{-3\alpha_{s'}L_{s'}}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\\&\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\nonumber\\&\cdot \sqrt{\rho(z,(mf_0+\kappa_1R))}\sqrt{\rho(z,(nf_0+(\kappa_1+\kappa_2-\kappa+l)R))}\nonumber\\&\cdot\sqrt{\rho(z,(mf_0+\kappa_2R))},
%}
%\begin{equation}\label{kerr.ter.span.s}
%\begin{split}
%&Q_{s,\text{x},\kappa}(z,f)=-j\gamma_s\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}g_s^{3/2}\text{e}^{-3\alpha_sL_s}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\\&\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\sum_{m,n,k\in \mathcal{S}_i}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\\&\cdot\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\Big)\\&\cdot \text{e}^{\tilde{\Gamma}_s(z,mf_0+\kappa_1 R)+\tilde{\Gamma}_s^*(z,nf_0+(\kappa_1+\kappa_2-\kappa+l) R)+\tilde{\Gamma}_s(z,kf_0+\kappa_2 R)}.
%\end{split}
%\end{equation}
We now insert \eqref{kerr.ter.span.s} into (\ref{MAN_NLI_sol}) to find the nonlinear electrical field of channel $\kappa$ in span $s$, which is equal to
\eqref{NLI_elec_kappa_z}.
\begin{figure*}[t]
\scriptsize
\eqlab{NLI_elec_kappa_z}{
&E_{\text{NLI,\text{x}},\kappa}^{s}(z,f)=-j\gamma_{s}\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2}
\sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\delta\big(f\!-\!if_0\!-(\kappa-l)\big)\text{e}^{\Gamma(z,if_0+(\kappa-l))}\sum_{m,n,k\in \mathcal{S}_i}\big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\nonumber\\&+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\zeta^s_{\kappa_1,\kappa_2,\kappa}(m,n,k)\nonumber\\&
\text{e}^{-j2\pi^{2}\big((mf_0+\kappa_1R)^2-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}+(kf_0+\kappa_2R)^{2}\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}-j\frac{4}{3}\pi^{3}\big((mf_0+\kappa_1R)^3-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{3}+(kf_0+\kappa_2R)^{3}\big)\sum_{s'=1}^{s-1}\beta_{3,s'}L_{s'}}
}
\hrulefill
\end{figure*}.
Considering the amplifier gain at the end of span $s$, we have 
\eqlab{NLI_elec_kappa_end_ns}{
&E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{s}L_{s'}},f)=g_{s}^{1/2}E_{s,\text{x},\kappa}^{(1)}(z,f)|_{z=L_{s}}.
}
%where $\zeta^{n_s}$ for $\gamma_{n_s}$, $L_{n_s}$, and $\beta_{n_s}$ is in analogy with (\ref{Zeta_ENL}) for $\gamma$, $L_s$, and $\beta$. 
To evaluate the nonlinear electrical filed of channel $\kappa$ at the end of link, we assume the nonlinear electrical field that generated in each span propagate linearly in the following spans until receive at the receiver, namely
\eqlab{}{
&E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{N}L_{s'}},f)=\prod_{s'=s+1}^{N}[{g_{s'}\cdot\rho(L_{s'},f)}]^{1/2}\nonumber\\& \text{e}^{-j2\beta_2\pi^{2}L_s\big(if_0+(\kappa-l)\big)^{2}\sum_{s'=s+1}^{N}(\beta_{2,s'}L_{s'}+\frac{2}{3}\pi(if_0+(\kappa-l)\beta_{2,s'}L_{s'})}\nonumber\\&E_{s,\text{x},\kappa}^{(1)}({\scriptstyle\sum_{s'=1}^{s}L_{s'}},f),
}
and, hence, this equation is equal to \eqref{NLI_elec_kappa_end_ns}.
\begin{figure*}[t]
\scriptsize
\eqlab{NLI_elec_kappa_end_ns}{
&-j\gamma_{s}\frac{8}{9}f_0^{3/2}\prod_{s'=1}^{s-1}[g_{s'}\cdot\rho(L_{s'},f)]^{3/2}g_{s}^{1/2}\!\!\! \prod_{s'=s+1}^{N}\!\!\! [g_{s'}\cdot\rho(L_{s'},f)]^{1/2} \sum_{\kappa_1=1}^{M}
\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}
\sum_{i=-\infty}^{\infty}\delta\big(f\!-\!if_0\!-(\kappa-1)\big)\nonumber\\&\text{e}^{-j2\pi^{2}(if_0+(\kappa-l)R)^{2}\sum_{s'=1}^{N_s}(\beta_2L_{s'}+\frac{2}{3}\pi(if_0+(\kappa-l)R)\beta_{3,s'}L_{s'})}\!\!\!\!\! \nonumber\\&\sum_{m,n,k\in s_i}\!\!\!\!\! \big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,k}\big)\sqrt{\rho(L_{s},if_0+(\kappa-l))}\zeta^s_{\kappa_1,\kappa_2,\kappa}(m,n,k)\nonumber\\&
\text{e}^{-j2\pi^{2}\big((mf_0+\kappa_1R)^2-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{2}+(kf_0+\kappa_2R)^{2}\big)\sum_{s'=1}^{s-1}\beta_{2,s'}L_{s'}-j\frac{4}{3}\pi^{3}\big((mf_0+\kappa_1R)^3-(nf_0+(\kappa_1+\kappa_2-\kappa+l)R)^{3}+(kf_0+\kappa_2R)^{3}\big)\sum_{s'=1}^{s-1}\beta_{3,s'}L_{s'}
},
}
\hrulefill
\end{figure*}

 Based on (\ref{NLI_elec_tot}), the total nonlinear electrical field at the end of link can be written as \eqref{NLI_elec_tot_detail}. This completes the proof.
 \end{IEEEproof}
%As seen in this equation, the three spectral components $mf_0$, $kf_0$, and $mf_0+kf_0-if_0$ located in channels $\kappa_1$, $\kappa_2$, $\kappa_1+\kappa_2-\kappa+l$, respectively, interact with each other and produce the nonlinear interference at $if_0$. The efficiency of this non-degenerate four wave mixing (FWM), denoted by \eqref{Zeta_ENL}, is taking place among these spectral components.
%\section{Derivation of the NLI power}\label{AppendixB}
%This appendix addresses derivation of the the NLI power of a certain channel, starting from the NLI PSD on polarization x 
%\eqlab{G_x_Def}
%{
%G_{\text{\small{NLI}},\text{x},\kappa}(f)=\mathbb{E}\big\{E_{\text{NLI,x},\kappa}(f)\text{e}^{*}_{\text{NLI,x},\kappa}(f)\big\}.
%}

==> Redan2.tex <==

The self-polarization and cross-polarization NLI contributions are then computed, and by summing up these contributions together, the total NLI PSD is obtained. 
In what follows, some \textit{Lemma}s are provided, which will be extensively used throughout the section. \textit{Lemma}~\ref{cyclostationary.NLI.field} ahead shows that the nonlinear electrical field given in \textit{Lemma}~\ref{multiple.span.extention} is a cyclostationary process.
\begin{lemma}\label{cyclostationary.NLI.field}
The process $E_{\text{x},\kappa}^{(1)}(L,t)$, in general,  is cyclostationary
because its mean and autocorrelation function are periodic with period $T_0$, namely
\begin{align}\label{mean.nli.field}
    \mathbb{E}\{E_{\text{x},\kappa}^{(1)}(L,t+T_0)\}=\mathbb{E}\{E_{\text{x},\kappa}^{(1)}(L,t)\},
\end{align}
and
\begin{align}\label{autocorrelation.periodic}
  \mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t,t-\tau)=\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t+T_0,t+T_0-\tau),
\end{align}
where $\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t,t-\tau)$ is the autocorrelation function of $E_{\text{x},\kappa}^{(1)}(L,t)$.
\end{lemma}

\begin{IEEEproof}
The total nonlinear electrical field given in \eqref{NLI_elec_tot_detail} has the form
\eqlab{tot.nli.fild.periodic}{
E_{\text{x},\kappa}^{(1)}(L,f)=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}I_{i,l}\cdot\delta(f-if_0-(\kappa-l)R)
}
where
%\eqlab{i.second}{
%&I_{i,l}=\imath \frac{8f_0^{3/2}}{9}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{m,n,p\in \mathcal{S}_{i,l}}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,p}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,p}
%\Big)\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p),
%}
\eqlab{i.second}{
&I_{i,l}=\imath \frac{8f_0^{3/2}}{9}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{m,n,p\in \mathcal{S}_{i,l}}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,p}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,p}
\Big)\varsigma_{\kappa_1,\kappa_2,\kappa}%(m,n,p),
} 
and $\mathcal{T}_{\kappa,l} = \{(\kappa_1,\kappa_2) \in \{1,\ldots,M\}^2: 1\le \kappa_1+\kappa_2-\kappa+l \le M\}
$,
%The inverse Fourier transform of \eqref{tot.nli.fild.periodic} is
%\eqlab{tot.nli.fild.periodic.t}{
%E_{\text{x},\kappa}^{(1)}(L,t)=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}I_{i,l}\cdot\text{e}^{\imath 2\pi(if_0+(\kappa-l)R)t},
%}
%and its autocorrelation function is equal to
% \eqlab{auto.tot.nli.fild.periodic.t}{
% &\mathcal{R}_{E_{\text{x},\kappa}^{(1)}}(\tau)=\mathbb{E}\Big\{\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}I_{i,l}\cdot\text{e}^{\imath 2\pi(if_0+(\kappa-l)R)t}\nonumber\\&
% \cdot\sum_{l'=-1}^{1}\sum_{i'=-\infty}^{\infty}I_{i',l'}^*\cdot\text{e}^{-\imath 2\pi(i'f_0+(\kappa-l')R)(t-\tau)}
% \Big\}=\nonumber\\&
% \sum_{l=-1}^{1}\sum_{l'=-1}^{1}\sum_{i=-\infty}^{\infty}\sum_{i'=-\infty}^{\infty}\mathbb{E}\bigl\{I_{i,l}\cdot I_{i',l'}^*\bigr\}\text{e}^{\imath 2\pi(if_0-i'f_0-lR+l'R)t}
% \nonumber\\&\cdot\text{e}^{\imath 2\pi(i'f_0+(\kappa-l)R)\tau}.
% }
% The autocorrelation is not a function of $\tau$, and thus, $i=i'$ and $l=l'$. This gives
% \eqlab{auto.tot.nli.fild.periodic.t.final}{
% &\mathcal{R}_{E_{\text{x},\kappa}^{(1)}}(\tau)=
% \sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\bigl\{I_{i,l} I_{i,l}^*\bigr\}\cdot\text{e}^{\imath 2\pi(if_0+(\kappa-l)R)\tau}
% ,
% }
and the inverse Fourier transform of \eqref{tot.nli.fild.periodic} is
\eqlab{tot.nli.fild.periodic.f}{
\hat{E}_{\text{x},\kappa}^{(1)}(L,t)=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}I_{i,l}\cdot\text{e}^{\imath2\pi(if_0+(\kappa-l)R)t},
}
whose mean is  \begin{align}\label{I.mean}
\mathbb{E}\{\hat{E}_{\text{x},\kappa}^{(1)}(L,t)\}=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\}\cdot\text{e}^{\imath2\pi(if_0+(\kappa-l)R)t},
\end{align}
which is equal to
%\footnote{It is worth mentioning that $\mathbb{E}\{I_{i,l}\}$ is always zero.}
\begin{align}\label{I.mean.T0}
&\mathbb{E}\{\hat{E}_{\text{x},\kappa}^{(1)}(L,t+T_0)\}=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\}\\&\nonumber\cdot\text{e}^{\imath2\pi(if_0+(\kappa-l)R)(t+T_0)}.
\end{align}
This is because $\text{e}^{\imath2\pi(if_0+(\kappa-l)R)T_0}=1$, as $T_0=WT_s$.

We proceed by demonstrating the fact that the autocorrelation function of $E_{\text{x},\kappa}^{(1)}(L,t)$ is periodic. To do so, the autocorrelation function is written as
\eqlab{autocorrelation}{
\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t,t-\tau)=\mathbb{E}\{\hat{E}_{\text{x},\kappa}^{(1)}(L,t)\cdot \hat{E}_{\text{x},\kappa}^{(1) *}(L,t-\tau)\}.
}
%it is enough to show that 
%\begin{align}\label{autocorrelation.periodic}
 % \mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t,t-\tau)=\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t+T_0,t+T_0-\tau).
%\end{align}
By substituting \eqref{tot.nli.fild.periodic.f} into \eqref{autocorrelation} we get
\eqlab{autocorrelation.2}{
&\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t,t-\tau)=\mathbb{E}\Big\{\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}I_{i,l}\cdot\text{e}^{\imath2\pi(if_0+(\kappa-l)R)t}\nonumber\\&\cdot
\sum_{l'=-1}^{1}\sum_{i'=-\infty}^{\infty}I_{i',l'}^*\cdot\text{e}^{-\imath2\pi(i'f_0+(\kappa-l')R)(t-\tau)}\Big\}=\nonumber\\&
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\sum_{l'=-1}^{1}\sum_{i'=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\cdot I_{i',l'}^*\}\cdot\text{e}^{\imath2\pi(if_0-i'f_0-lR+l'R)t}\nonumber\\&\cdot\text{e}^{\imath2\pi(i'f_0+(\kappa-l')R)\tau},
}
in which 
\eqlab{i.second.conjugate}{
&I_{i',l'}^{*}=\imath \frac{8f_0^{3/2}}{9}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l'}}\sum_{m',n',p'\in \mathcal{S}_{i',l'}}\Big(\xi_{\text{x},\kappa_1',m}\xi_{\text{x},\kappa_1'+\kappa_2'-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2',p}+\xi_{\text{y},\kappa_1',m}\xi_{\text{y},\kappa_1'+\kappa_2'-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2',p}
\Big)\varsigma_{\kappa_1',\kappa_2',\kappa}.%(m,n,p),
}
Eq.~\eqref{autocorrelation.2} is periodic, as
\eqlab{autocorrelation.2.periodic}{
&\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t+T_0,t+T_0-\tau)=\nonumber\\&
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\sum_{l'=-1}^{1}\sum_{i'=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\cdot I_{i',l'}^*\}\cdot\text{e}^{\imath2\pi(if_0-i'f_0-lR+l'R)t}\nonumber\\&\cdot\text{e}^{\imath2\pi(if_0-i'f_0-lR+l'R)T_0}\cdot\text{e}^{\imath2\pi(i'f_0+(\kappa-l')R)\tau},
}
is equal to \eqref{autocorrelation.2}, due to the fact that $\text{e}^{\imath2\pi(if_0-i'f_0-lR+l'R)T_0}=1$.
We therefore find that the process \eqref{tot.nli.fild.periodic.f} is  cyclostationary. 
\end{IEEEproof}

We now deal with the expectation term in \eqref{autocorrelation.2.periodic}, say $\mathbb{E}\{I_{i,l}\cdot I_{i',l'}^*\}$.
Considering \eqref{i.second} and \eqref{i.second.conjugate} and using the fact that the symbols in the y polarization are independent from those in the x polarization, we have
\eqlab{G_x_lequall'}
{
&\mathbb{E}\bigl\{I_{i,l}\cdot I_{i',l'}^{*}\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l'}}\nonumber\\
&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i',l'}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')\nonumber\\
&\Big(\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\nonumber\\
%%%
&+\mathbb{E}\big\{\xi_{\text{x},\kappa_1,m}\xi^{*}_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\}\nonumber\\
%%
&+\mathbb{E}\big\{\xi^{*}_{\text{x},\kappa'_1,m'}\xi_{\text{x},\kappa'_1+\kappa'_2-\kappa+l',n'}\xi^{*}_{\text{x},\kappa'_2,p'}\xi_{\text{x},\kappa_2,p}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}\nonumber\\
%%
& +\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\Big).
}

\begin{lemma}\label{second.third.i.i*.zero}
The expectation terms
\begin{align}\label{second.term.I.I*}
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\},
\end{align}
and  
\begin{align}\label{third.term.I.I*}
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\},
\end{align}
given in \eqref{G_x_lequall'} are equal to zero, and therefore, \eqref{G_x_lequall'} is
\eqlab{G_x_lequall'.nonbias}
{
&\mathbb{E}\bigl\{I_{i,l}\cdot I_{i',l'}^{*}\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l'}}\nonumber\\
&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i',l'}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')\nonumber\\
&\Big(\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\nonumber\\
%%%
& +\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\Big).
}
\end{lemma}

\begin{IEEEproof}
Using \eqref{FourierSerisCoef1} we can express \eqref{second.term.I.I*} as
\begin{align}\label{independent.xi}
  & \mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\}=\\&\nonumber f_0S^*(m' f_0)S(n' f_0)\sum_{w_1=1}^{W}\sum_{w_2=1}^{W}\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l'},w_2}\}\\&\nonumber\cdot\text{e}^{\imath\frac{2\pi}{W}(m'w_1-n'w_2)}.
\end{align}
To evaluate \eqref{independent.xi}, the following three situations should be taken into consideration.
\begin{enumerate}
    \item {when $\kappa_1'\neq \kappa_1'+\kappa_2'-\kappa+l'$, the expectation term in \eqref{independent.xi} is equal to zero, namely
    \begin{align}
    &\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l'},w_2}\}=\\&\nonumber\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}\}\mathbb{E}\big\{{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l'},w_2}\}=0,
    \end{align}so \eqref{independent.xi} becomes zero.}
    %%
      \item {when $\kappa_1'= \kappa_1'+\kappa_2'-\kappa+l'$ and $m'\neq n'$,  \eqref{independent.xi} is 
\begin{align}\label{independent.xi.k1equalk2}
  &f_0S^*(m' f_0)S(n' f_0)\sum_{w_1=1}^{W}\sum_{w_2=1}^{W}\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'},w_2}\}\\&\nonumber\cdot\text{e}^{\imath\frac{2\pi}{W}(m'w_1-n'w_2)},
\end{align}
    in which for $w_1\neq w_2$ we have \begin{align}
  \mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'},w_2}\}=\mathbb{E}\big\{b^{*}_{\text{y},{\kappa_1'},w_1}\}\cdot\mathbb{E}\big\{b_{\text{y},{\kappa_1'},w_2}\}=0.
\end{align}
    Eq.~\eqref{independent.xi.k1equalk2} is therefore equal to
    \begin{align}\label{independent.xi.k1equalk2.w1equalw2}
  &f_0S^*(m' f_0)S(n' f_0)\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'}}|^2\}\cdot\sum_{w_1=1}^{W}\text{e}^{\imath\frac{2\pi}{W}(m'-n')w_1},
\end{align}
where we assume that the channel is stationary, i.e., $\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'}}|^2\}=\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'},w_i}|^2\}$. The summation term in \eqref{independent.xi.k1equalk2.w1equalw2} is equal to
\begin{align}
    \sum_{w_1=1}^{W}\text{e}^{\imath\frac{2\pi}{W}(m'-n')w_1}=
\left\{ \begin{array}{l}
    0 \quad m'\neq n' \;\;\text{and}\;\; m'-n'\neq pW\\
    W \quad m'-n'=pW
  \end{array} \right.
\end{align}
where $p$ is an integer. This implies that there is correlation between spectral lines which are $pWf_0=pR$ apart, namely multiples of symbol rate. Since for the Nyquist case there is no two spectral lines which are $R$ apart, we find that $p=0$. This means Eq.~\eqref{independent.xi.k1equalk2.w1equalw2} is always equal to zero as $m'\neq n'$.
    }
    %%
          \item {when $\kappa_1'= \kappa_1'+\kappa_2'-\kappa+l'$ and $m'=n'$, the situation is interpreted as a constant phase shift and does not belong to set $\mathcal{S}_{i,l}$
 given in \eqref{sil}, and should be ignored. 
    }
\end{enumerate}
The same procedure holds for $\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}$ given in \eqref{third.term.I.I*}. We hence find that these expectation terms are zero and \eqref{G_x_lequall'} is then equal to \eqref{G_x_lequall'.nonbias}.

\end{IEEEproof}

\begin{lemma}
For $l\neq l'$, \eqref{G_x_lequall'.nonbias} is equal to zero, and thus, the autocorrelation function \eqref{autocorrelation.2} can be written as
\begin{align}\label{autocorrelation.3}
&\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t,t-\tau)=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\sum_{i'=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\cdot I_{i',l}^*\}\\&\nonumber\cdot\text{e}^{\imath2\pi(if_0-i'f_0)t}\cdot\text{e}^{\imath2\pi(i'f_0+(\kappa-l)R)\tau}.
\end{align}
\end{lemma}

\begin{IEEEproof}
To evaluate the first expectation term in \eqref{G_x_lequall'.nonbias},
\eqlab{first.exp.l.equal.l'}{
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\},
}
we should consider  situations which result in the sixth, fourth, and second order moments.
\begin{itemize}
\item{Sixth order moment: This moment is generated when in \eqref{first.exp.l.equal.l'} all $\xi$s belong to the same channel, namely
\eqlab{situations.l.equal.l'.1}{
\!\!\!\!\!\kappa_1=\kappa_2=\kappa_1+\kappa_2-\kappa+l=\kappa_1'=\kappa_2'=\kappa_1'+\kappa_2'-\kappa+l'.
}
This occurs only when $l=l'$, otherwise we have
one $\xi$ which is located in different channel, 
and \eqref{first.exp.l.equal.l'} is equal to
\eqlab{first.exp.l.equal.l'.3}{
\!\!\!\!\!\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\mathbb{E}\{\xi_{\text{x},\small{\kappa_1+l'-l},n'}\}=0,}
since using \eqref{FourierSerisCoef1}
\begin{align}
 &\mathbb{E}\{\xi_{\text{x},\small{\kappa_1+l'-l},n'}\}=  
\sqrt{f_0}S(n' f_0)\sum_{w=1}^{W}\mathbb{E}\{{b}_{\text{x},{\kappa+l'-l},w}\}\\&\nonumber\cdot\text{e}^{-\imath\frac{2\pi}{W}n'w}=0,
\end{align}
as $\mathbb{E}\{{b}_{\text{x},{\kappa+l'-l},w}\}=0$.
}
\item{Products of the fourth and second order moments:
We have the following 15 situations
\begin{align}
&\label{first.exp.l.equal.l'.1}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\}\nonumber\\&\cdot\mathbb{E}\big\{\cancelto{0}{\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}}\big\},\\&
%%
\label{first.exp.l.equal.l'.2}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\}\\&\nonumber\cdot\cancelto{0}{\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}},\\&
%%
\label{first.exp.l.equal.l'.3}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\cancelto{0}{\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}}\big\},\\&
%%
\label{first.exp.l.equal.l'.4}\mathbb{E}\big\{\cancelto{0}{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\},\\&
%%
\label{first.exp.l.equal.l'.5}\cancelto{0}{\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_2},p}\big\}}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\},\\&
%%
\label{first.exp.l.equal.l'.6}\mathbb{E}\big\{\cancelto{0}{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\},\\&
%%
\label{first.exp.l.equal.l'.7}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\},\\&
%%
\label{first.exp.l.equal.l'.8}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\cancelto{0}{\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\}},\\&
%%
\label{first.exp.l.equal.l'.9}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2'},p'}\xi_{\text{x},\small{\kappa_2},p}\big\},\\&
%%
\label{first.exp.l.equal.l'.10}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_2},p}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\cancelto{0}{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}}\big\},\\&
%%
\label{first.exp.l.equal.l'.11}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\},\\&
%%
\label{first.exp.l.equal.l'.12}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\cancelto{0}{\xi^{*}_{\text{x},\small{\kappa_2'},p'}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}}\big\},\\&
%%
\label{first.exp.l.equal.l'.13}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\},\\&
%%
\label{first.exp.l.equal.l'.14}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\cancelto{0}{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}}\big\},\\&
%%
\label{first.exp.l.equal.l'.15}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2'},p'}\xi_{\text{x},\small{\kappa_1},m}\big\}.\\&\nonumber
%%
\end{align}
As can be seen the second order moment in \eqref{first.exp.l.equal.l'.7} is created when 
\begin{align}\label{sec.k.k'}
\kappa_2=\kappa_1'.
\end{align}
The fourth order moment in \eqref{first.exp.l.equal.l'.7} is also generated when
\eqlab{first.exp.l.equal.l'.1.fourth.order}{
\kappa_1=\kappa_1+\kappa_2-\kappa+l=\kappa_2=\kappa_1'+\kappa_2'-\kappa+l'=\kappa_2'.
}
This implies that \eqref{sec.k.k'} and \eqref{first.exp.l.equal.l'.1.fourth.order} are satisfied simultaneously when $l=l'$. 
The same is true for \eqref{first.exp.l.equal.l'.9}, \eqref{first.exp.l.equal.l'.11}, \eqref{first.exp.l.equal.l'.13}, and \eqref{first.exp.l.equal.l'.15}.
As shown in \textit{Lemma}~\ref{second.third.i.i*.zero}, the expectation terms given in \eqref{second.term.I.I*} and \eqref{third.term.I.I*} are zero. An identical argument holds for the second order expectation terms of
\eqref{first.exp.l.equal.l'.1}, \eqref{first.exp.l.equal.l'.3}, \eqref{first.exp.l.equal.l'.4}, and \eqref{first.exp.l.equal.l'.6}.
%%
Eqs.~\eqref{first.exp.l.equal.l'.2}, \eqref{first.exp.l.equal.l'.5}, \eqref{first.exp.l.equal.l'.8}, \eqref{first.exp.l.equal.l'.10}, \eqref{first.exp.l.equal.l'.12}, and \eqref{first.exp.l.equal.l'.14} are also equal to zero, for example, in order to compute the second order expectation term given in \eqref{first.exp.l.equal.l'.5}, the following two situations need to be considered.
\begin{enumerate}
    \item {$\kappa_1\neq \kappa_2$: In this regard, $\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_2},p}\big\}=\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\}\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\big\}=0$.}
    \item {$\kappa_1= \kappa_2$: This situation gives rise to  \eqlab{xi.power2}{
&\!\!\!\!\!\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_1},p}\big\}=\\&\nonumber {f_0}S(m f_0)S(p f_0)\sum_{w_1=1}^{W}\sum_{\substack{w_2=1\\w_1\neq w_2}}^{W}\cancelto{0}{\mathbb{E}\{{{b}}_{\text{x},{\kappa_1},w_1}{{b}}_{\text{x},{\kappa_1},w_2}\}}\\&\nonumber\!\!\!\!\!\cdot\text{e}^{-\imath\frac{2\pi}{W}(mw_1+pw_2)}+\\&\nonumber{f_0}S(m f_0)S(p f_0)\sum_{w_1=1}^{W}\mathbb{E}\{{{b}}_{\text{x},{\kappa_1},w_1}^2\}\text{e}^{-\imath\frac{4\pi}{W}(m+p)w_1},
 }
 in which the last term is also zero, since 
\eqlab{real.imagin.xi.pow.2}{
\mathbb{E}\{{{b}}^2_{\text{x},{\kappa_1},w_1}\}=&\mathbb{E}\{\Re^2\{{b_{\text{x},{\kappa_1},w_1}}\}\}-\mathbb{E}\{\Im^2\{{b_{\text{x},{\kappa_1},w_1}}\}\}+\nonumber\\&
2\imath\cdot\mathbb{E}\{\Re\{{b_{\text{x},{\kappa_1},w_1}}\}\}\mathbb{E}\{\Im\{{b_{\text{x},{\kappa_1},w_1}}\}\}=0,
}
where $\Re$ and $\Im$ represent the real and imaginary parts, and $\Re\{{b_{\text{x},{\kappa_1},w_1}}\}$ and $\Im\{{b_{\text{x},{\kappa_1},w_1}}\}$ are independent of one another. We can do the same procedure for $\mathbb{E}\big\{\xi^{*2}_{\text{x},\small{\kappa_1},m}\big\}$.}
\end{enumerate}
}
%%%%%%%%%%%%%%%%%%%%%%%
\item{Product of the second order moments:
In \textit{Lemma}~\ref{second.third.i.i*.zero}, we demonstrated that $\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\}$ and $\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}$ are always equal to zero. Analogous expressions hold for 
\begin{align}
   &\mathbb{E}\big\{\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_2,p}\big\}, \;\;\text{and}\\&\nonumber \mathbb{E}\big\{\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\xi_{y,\kappa_2',p'}^*\big\}.
\end{align}
Using this, and considering the fact that $\mathbb{E}\big\{\xi^2_{\text{x},\small{\kappa_1},m}\big\}=0$ and $\mathbb{E}\big\{\xi^{*2}_{\text{x},\small{\kappa_1},m}\big\}=0$ (see \eqref{xi.power2}),
we have the following two situations for product of second order moments
\begin{align}
   &\label{second.order.first.term.l.equal.l'.1}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}, \\&
   %%
   \label{second.order.first.term.l.equal.l'.2}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\}.
\end{align}
It is clear that situations \eqref{second.order.first.term.l.equal.l'.1} and \eqref{second.order.first.term.l.equal.l'.2} are non-zero when $l=l'$.}
\end{itemize}


To evaluate the second term in \eqref{G_x_lequall'.nonbias},
\begin{align}\label{second.term.l.equal.l'.psd}
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\},
\end{align}
we have to take into account the following situations.
\begin{itemize}
  \item{Product of the fourth and second order moments:
the second expectation term in \eqref{second.term.l.equal.l'.psd} is non-zero when $\kappa_2=\kappa_2'$. The first expectation term in \eqref{second.term.l.equal.l'.psd} results in the fourth order moment when 
\begin{align}\label{hgt}
    \kappa_1=\kappa_1'=\kappa_1+\kappa_2-\kappa+l=\kappa_1'+\kappa_2'-\kappa+l'.
\end{align}
Considering the fact that $\kappa_2=\kappa_2'$, it is found that the equality \eqref{hgt} is satisfied only when $l=l'$. } 
%%%%%%%%%%%%%%%%%%%%%%
\item{Product of the second order moments:
In this regard, the following expectation terms should be considered.
\begin{align}
    &\mathbb{E}\big\{\cancelto{0}{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}}\big\}\big\{\cancelto{0}{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}}\big\}\nonumber\\
%%
&\cdot\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\label{s.1},\\&
%%%%%
\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1',m'}\big\}\big\{\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}\big\}\nonumber\\
%%
&\cdot\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\label{s.2},\\&
%%%%
\mathbb{E}\big\{\cancelto{0}{\xi_{y,\kappa_1,m}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l',n'}}\big\}\big\{\cancelto{0}{\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}}\big\}\nonumber\\
%%
&\cdot\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\label{s.3},
\end{align}
Considering \textit{Lemma}~\ref{second.third.i.i*.zero}, it is clear that \eqref{s.1} is zero. Eq.~\eqref{s.3} is also zero for the reason stated in \eqref{xi.power2}. Eq.~\eqref{s.2} is non-zero only when $l=l'$.

}
\end{itemize}
It is therefore turned out that \eqref{autocorrelation.2} can be expressed as
\eqref{autocorrelation.3}. 
\end{IEEEproof}

\begin{lemma}\label{psd.I.square}
The PSD of \eqref{tot.nli.fild.periodic} is equal to
\eqlab{psd.tot.nli.fild.periodic.f.final}{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}\delta(f-if_0-(\kappa-l)R).
}
\end{lemma}

\begin{IEEEproof}
The average autocorrelation function of a cyclostatinary process is defined as the average of autocorrelation function over one period, namely 
\begin{align}\label{average.autocorrelation}
    \bar{\mathcal{R}}_{\hat{E}_{\text{x},\kappa}^{(1)}}(\tau)=\frac{1}{T_0}\int_{-T_0/2}^{T_0/2}\mathcal{R}_{\hat{E}_{\text{x},\kappa}^{(1)}}(t,t-\tau)\text{d}t.
\end{align}
Inserting \eqref{autocorrelation.3} into \eqref{average.autocorrelation} gives
\begin{align}\label{average.autocorrelation.2}
    &\bar{\mathcal{R}}_{\hat{E}_{\text{x},\kappa}^{(1)}}(\tau)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\sum_{i'=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\cdot I_{i',l}^*\}\nonumber\\&\cdot\text{e}^{\imath2\pi(i'f_0+(\kappa-l)R)\tau}\cdot\frac{1}{T_0}\int_{-T_0/2}^{T_0/2}\text{e}^{\imath2\pi(if_0-i'f_0)t}\text{d}t=\\&\nonumber
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\sum_{i'=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\cdot I_{i',l}^*\}\\&\nonumber\text{e}^{\imath2\pi(i'f_0+(\kappa-l)R)\tau}\cdot\frac{\sin\Big({2\pi(if_0-i'f_0)T_0/2\Big)}}{T_0\Big(\pi(if_0-i'f_0)\Big)}
.
\end{align}
We mentioned earlier in Sec~\ref{key_results} that the period of signal tends to infinity $T_0\rightarrow \infty$, and as a result \eqref{average.autocorrelation.2} will become
\begin{align}\label{average.autocorrelation.2.T0.infty}
    &\bar{\mathcal{R}}_{\hat{E}_{\text{x},\kappa}^{(1)}}(\tau)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\sum_{i'=-\infty}^{\infty}\mathbb{E}\{I_{i,l}\cdot I_{i',l}^*\}\nonumber\\&\cdot\text{e}^{\imath2\pi(i'f_0+(\kappa-l)R)\tau}\cdot\lim_{T_0\rightarrow \infty}\frac{\sin\Big({2\pi(if_0-i'f_0)T_0/2\Big)}}{T_0\Big(\pi(if_0-i'f_0)\Big)}
.
\end{align}
Since 
\begin{align}\label{limit.periodic.autocorrelation}
\lim_{T_0\rightarrow \infty}\frac{\sin\Big({2\pi(if_0-i'f_0)T_0/2\Big)}}{T_0\Big(\pi(if_0-i'f_0)\Big)}=0,
\end{align}
we find that \eqref{average.autocorrelation.2} is
always zero for $i\neq i'$. To be more specific, when $i=i'$ \eqref{average.autocorrelation.2} will no longer depend on $t$ and can be expressed as
\begin{align}\label{average.autocorrelation.3}
    &\bar{\mathcal{R}}_{\hat{E}_{\text{x},\kappa}^{(1)}}(\tau)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\{|I_{i,l}|^2\}\cdot\text{e}^{\imath2\pi(if_0+(\kappa-l)R)\tau},
\end{align}
and its Fourier transform results in PSD, namely \eqref{psd.tot.nli.fild.periodic.f.final}. 

\end{IEEEproof}

%\eqlab{psd.tot.nli.fild.periodic.f.final}{
%&G_{\text{\small{NLI}},\text{x},\kappa}(f)=
%\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}\delta(f-if_0-(\kappa-l)R).
%}
Using the fact that the symbols in the y polarization are independent from those in the x polarization
, we obtain from \eqref{i.second} 
\eqlab{G_x}
{
&\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l}}\nonumber\\
&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')\nonumber\\
&\Big(\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\nonumber\\
%%%
&+\mathbb{E}\big\{\xi_{\text{x},\kappa_1,m}\xi^{*}_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
%%
&+\mathbb{E}\big\{\xi^{*}_{\text{x},\kappa'_1,m'}\xi_{\text{x},\kappa'_1+\kappa'_2-\kappa+l,n'}\xi^{*}_{\text{x},\kappa'_2,p'}\xi_{\text{x},\kappa_2,p}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}\nonumber\\
%%
& +\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\Big).
} 
%where $\mathcal{S}^{\prime}_{i,l}$ is defined like $\mathcal{S}_{i,l}$ but replacing $m$, $n$ and $p$ with $m^{\prime}$, $n^{\prime}$ and $p^{\prime}$, respectively.  


==> redundant.tex <==
































By putting \eqref{momentum.expansion.2} and \eqref{cross-polarization NLI.2} into \eqref{Csp} and \eqref{Cxp}, resp., and then insert them into \eqref{G_x.noBias} we get
 \eqlab{G_x.noBias.2}
{
&\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}( \\&\nonumber \delta_{\kappa_1-\kappa_2}\delta_{\kappa_2-\kappa+l}\cdot A_6
   +\\&\nonumber
   %%
\delta_{\kappa_2-\kappa+l}\cdot B_{4,2}+\\&\nonumber
   %%\\&\nonumber
\delta_{\kappa_2-\kappa+l}\cdot C_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1-\kappa_2}\cdot D_{4,2}\\&\nonumber+
   %%
\delta_{\kappa_1-\kappa+l}\cdot E_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1-\kappa+l}\cdot F_{4,2}+\\&\nonumber
%%
\cdot
G_{2,2,2}+\\&\nonumber
%%
\cdot H_{2,2,2}+\\&\nonumber
%%
\delta_{\kappa_2-\kappa+l}'{X}_{1}+\\&\nonumber+
%%
\delta_{\kappa_2-\kappa+l}{X}_{2}),
}










\indent {\bf{Product of fourth and second order moments:}}
Regarding Appendix~\ref{fourth.second. moments.lneql'}, the following moments should be taken into account.
\begin{itemize}
\item{
\begin{align}
\label{first.exp.l.l.7}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\}.
\end{align}}
To form the fourth and second order moment, 
%%
\item{
\begin{align}\label{first.exp.l.l.9}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2'},p'}\xi_{\text{x},\small{\kappa_2},p}\big\},
\end{align}}
%%
\item{
\begin{align}
 \label{first.exp.l.l.11}
 &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l'},n'}\big\},   
\end{align}
}
%%
\item{
\begin{align}
    \label{first.exp.l.l.13}
    &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\},
\end{align}
}
%%
\item{
\begin{align}
    \label{first.exp.l.equal.l'.15}
    &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2'},p'}\xi_{\text{x},\small{\kappa_2},p}\big\}.
\end{align}
}
\end{itemize}


\indent{\bf{Product of second order moments:}} Considering Appendix~\ref{second.order.moments.l.neq.l'}, we should take into account the following situations.
\begin{itemize}
    \item {
       \begin{align}\label{second.order.first.term.l.l.1}
       &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}
       \end{align}
    }
    %%
     \item {
  \begin{align}\label{second.order.first.term.l.l.2}&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\big\} 
  \end{align}
       }
          
\end{itemize}










which gives rise to
       \eqlab{self.pol.exp.sixth.order.moment}{ \mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}.
 }
   



















Due to the bias or non-fluctuating terms and using the fact that $\mathbb{E}\big\{\xi^2_{\text{x},\small{\kappa_1},m}\big\}=0$,
we find that for evaluating \eqref{self.pol.exp}, we must consider the following two situations 
\begin{align}
&\label{cond_el.1}\kappa_1=\kappa_1',\quad \kappa_2=\kappa_2',\\&
\label{cond_el.6}
\kappa_1=\kappa_2',\quad \kappa_2=\kappa_1'.
\end{align}
For the first situation \eqref{cond_el.1}, \eqref{Csp} can be written as 
 \eqlab{G_x.noBias.nosum.prime.first}
{
&C_{\text{sp}}=\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\nonumber\\&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\nonumber\\&\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}.
}
To evaluate the self-polarization expectation term
\eqlab{first.situation.self.pol.exp}{
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\},
}
we need to take into consideration the following situations
\begin{align}
&\label{five.situations.first.term.1}\kappa_1\neq \kappa_1+\kappa_2-\kappa+l, \quad \kappa_2\neq \kappa_1+\kappa_2-\kappa+l,\quad \kappa_1\neq \kappa_2,\\&
\label{five.situations.first.term.2}\kappa_1= \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1\neq \kappa_2,\\&
\label{five.situations.first.term.3}\kappa_2= \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1\neq \kappa_2,\\&
\label{five.situations.first.term.4}\kappa_1\neq \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1= \kappa_2,\\&
\label{five.situations.first.term.5}\kappa_1= \kappa_1+\kappa_2-\kappa+l, \quad \kappa_1= \kappa_2,
\end{align}
where for the first situation \eqref{five.situations.first.term.1}, \eqref{first.situation.self.pol.exp} has the following form
\eqlab{first.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\nonumber\\&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}.
}
Using the second order moment given in \cite[Appendix~E]{carena2014accuracy}, \eqref{first.situation.self.pol} is reduced to
\begin{equation}\label{d'}
\begin{split}
&R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m-m'}R|S(nf_0)|^{2}\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}=D',
\end{split}
\end{equation}
and we call this term as $D'$. 
For the second situation \eqref{five.situations.first.term.2}, we can write \eqref{first.situation.self.pol.exp} as
\eqlab{second.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},n'}\big\}
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\},
}
and using the second and fourth order moments given in \cite[Appendix~E]{carena2014accuracy}, we can write \eqref{second.situation.self.pol} as
\begin{equation}\label{e'}
\begin{split}
&\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mn'm'n}\delta_{m-m'}\delta_{n-n'}+\\&Rf_0U_{mn'm'n}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}\Big)=E',
\end{split}
\end{equation}
and we call this term as $E'$, in which
\begin{equation}\label{P_e'}
\begin{split}
&U_{mn'm'n}=S_{\kappa_1}(mf_0)S^*_{\kappa_1}(nf_0)S^*_{\kappa_1}(m'f_0)S_{\kappa_1}(n'f_0).
\end{split}
\end{equation}
For the third situation \eqref{five.situations.first.term.3}, we can write \eqref{first.situation.self.pol.exp} as
\eqlab{third.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_2},n}\xi_{\text{x},\small{\kappa_2},n'}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\},
}
and following the same procedure that we did in \eqref{second.situation.self.pol}, \eqref{third.situation.self.pol} is expressed as
\eqlab{f'}{
&\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{x,\kappa_1}|^{2}\}\delta_{m-m'}\Big)\nonumber\\&\Big(R^{2}\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}U_{pn'p'n}\delta_{p-p'}\delta_{n-n'}+\\&Rf_0U_{pn'p'n}\delta_{p-n-p'+n'}\Big[\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}\Big]\Big)=F',
}
and we call this term as $F'$, where
\begin{equation}\label{P_f'}
\begin{split}
&U_{pn'p'n}=S_{\kappa_2}(pf_0)S^{*}_{\kappa_2}(nf_0)S^*_{\kappa_2}(p'f_0)S_{\kappa_2}(n'f_0).
\end{split}
\end{equation}
For the fourth situation \eqref{five.situations.first.term.4}, \eqref{first.situation.self.pol.exp} can be written as
\eqlab{fourth.situation.self.pol}{
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\},
}
and following the same procedure that we did in \eqref{second.situation.self.pol} and \eqref{third.situation.self.pol}, we get
\begin{equation}\label{g'}
\begin{split}
&\Big(2R^{2}\mathbb{E}^{2}\{|b_{x,\kappa_1}|^{2}\}U_{mp'm'p}\delta_{m-m'}
\delta_{p-p'}+\\&R f_0U_{mp'm'p}\delta_{m-m'-p'+p}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2Rf_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\\&\Big(R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}\Big)=G',
\end{split}
\end{equation}
and we call this term as $G'$. For the last situation \eqref{five.situations.first.term.5}, \eqref{first.situation.self.pol.exp} can be written as
\begin{equation}\label{h'}
\begin{split}
&H'=\Big(2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mnpm'n'p'}\delta_{m-m'}\delta_{n-n'}\delta_{p-p'}\Big)+\\&\Big(R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\\&
(4\delta_{m-m'}\delta_{p-n+n'-p'}+\delta_{n-n'}\delta_{m+p-m'-p'})\Big)+\Big(Rf_0\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\\&U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p'}\Big),
\end{split}
\end{equation}
where
\begin{equation}\label{P_ell}
\begin{split}
&U_{mnpm'n'p'}=\nonumber\\&
S_{\kappa_1}(mf_0)S^*_{\kappa_1}(nf_0)S_{\kappa_1}(pf_0)S^*_{\kappa_1}(m'f_0)S_{\kappa_1}(n'f_0)S^*_{\kappa_2}(p'f_0).
\end{split}
\end{equation}
Putting all these terms together (\eqref{d'}, \eqref{e'}, \eqref{f'}, \eqref{g'}, and \eqref{h'}), we can express \eqref{first.situation.self.pol.exp} as
\begin{equation}\label{fo1}
\begin{split}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}\\&=\\&\delta'_{\kappa_1-\kappa+l}\delta'_{\kappa_2-\kappa+l} \delta'_{\kappa-\kappa_2}D'+
\delta_{\kappa_2-\kappa+l}\delta'_{\kappa_1-\kappa_2}E'\\&+\delta_{\kappa_1-\kappa+l}\delta'_{\kappa_1-\kappa_2}F'+
\delta_{\kappa_1-\kappa_2}\delta'_{\kappa_1-\kappa+l}G'+\\&\delta_{\kappa_1-\kappa_2}\delta_{\kappa_1-\kappa_2-\kappa+l}H'.
\end{split}
\end{equation}

We proceed by evaluating  the second situation \eqref{cond_el.6}. For this situation, \eqref{G_x.noBias} can be written as 
 \eqlab{G_x.noBias.nosum.prime.second}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\sum_{i=-\infty}^{+\infty}\delta \big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\nonumber\\&\Big(\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\nonumber\\&\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}\Big),
}
and the self-polarization expectation term is equal to
\eqlab{first.situation}{
&
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}.
}
Following the same procedure that we did for the first situation \eqref{cond_el.1}, \eqref{first.situation} is equal to 
\begin{equation}\label{fo}
\begin{split}
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\\&=\\&\delta'_{\kappa_1-\kappa+l}\delta'_{\kappa_2-\kappa+l} \delta'_{\kappa-\kappa_2}{D}''+
\delta_{\kappa_2-\kappa+l}\delta'_{\kappa_1-\kappa_2}{E}''\\&+\delta_{\kappa_1-\kappa+l}\delta'_{\kappa_1-\kappa_2}{F}''+
\delta_{\kappa_1-\kappa_2}\delta'_{\kappa_1-\kappa+l}{G}'+\\&\delta_{\kappa_1-\kappa_2}\delta_{\kappa_1-\kappa_2-\kappa+l}{H}',
\end{split}
\end{equation}
where 
\begin{equation}\label{d''}
\begin{split}
&{D}''=R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m-p'}R|S(nf_0)|^{2}\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}R|S(pf_0)|^{2}\delta_{p-m'}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\},
\end{split}
\end{equation}
\begin{equation}\label{e''}
\begin{split}
&{E}''=\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mnp'n'}\delta_{m-p'}\delta_{n-n'}+\\&Rf_0U_{mnp'n'}\delta_{m-n-p'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{x,\kappa_2}|^{2}\}\delta_{p-m'}\Big)
\end{split}
\end{equation}
in which
\begin{equation}\label{P_e''}
\begin{split}
&U_{mnp'n'}=S(mf_0)S^*_{\kappa_1}(nf_0)S^{*}(p'f_0)S(n'f_0),
\end{split}
\end{equation}
and
\begin{equation}\label{f''}
\begin{split}
&{F}''=\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}U_{pnm'n'}\delta_{p-m'}\delta_{n-n'}+\\&Rf_0U_{pnm'n'}\delta_{p-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\Big)\\&\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m-p'}\Big),
\end{split}
\end{equation}
in which
\begin{equation}\label{P_f''}
\begin{split}
&U_{pnm'n'}=S(pf_0)S^*(nf_0)S^{*}(m'f_0)S(n'f_0).
\end{split}
\end{equation}
\subsubsection{Cross-polarization NLI contributions}\label{ap_b}
For analysis of the cross polarization NLI effects, i.e., 
  \eqlab{G_x.noBias.cross.pol.tot}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{\kappa_1'=1}^{M}\sum_{\kappa_2'=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\sum_{i=-\infty}^{+\infty}\delta \big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')\nonumber\\&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1,m}\xi_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_1',m'}\xi^{*}_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}.
}
To evaluate
\eqlab{srtm}{
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1,m}\xi_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_1',m'}\xi^{*}_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\},
}
we must evaluate just a non zero situation, namely
\eqlab{}
{
\kappa_1=\kappa'_1,\quad \kappa_2=\kappa'_2,
}
and, hence,  \eqref{srtm} is expressed as
\eqlab{c}{
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1,m}\xi_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi_{y,\kappa_1,m'}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n'}\big\}\nonumber\\&\cdot
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2,p'}\big\}.
}
Using the second and fourth order moments of $\xi$, we can express \eqref{c} as \eqlab{xcross.pol.term}{\delta'_{\kappa_2-\kappa+l}{X}_{\text{x}}+\delta_{\kappa_2-\kappa+l}{X}_{\text{x}}',
}
where
\eqlab{Xx}
{
&{X}_{\text{x}}=R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\delta_{m-m'}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n-n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'},
}
and
\eqlab{Xx'}
{
&{X}_{\text{x}}'=\Big(R^2 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2\delta_{m-m'}\delta_{n-n'}+\nonumber\\&Rf_0U_{mnm'n'}\delta_{m'-m-n'+n}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\Big)\nonumber\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}\Big),
}
where
\begin{equation}\label{P_e''}
\begin{split}
&U_{mnm'n'}=S(m'f_0)S^{*}(mf_0)S^{*}(n'f_0)S(nf_0).
\end{split}
\end{equation}
We can therefore write \eqref{G_x.noBias.cross.pol.tot} as
\eqlab{G_x.noBias.cross.pol.tot.sec}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}f_0^{3}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{\kappa_1'=1}^{M}\sum_{\kappa_2'=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\sum_{i=-\infty}^{+\infty}\delta \big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\nonumber\\&\delta'_{\kappa_2-\kappa+l}{X}_{\text{x}}+\delta_{\kappa_2-\kappa+l}{X}_{\text{x}}'.
}
\subsubsection{Total NLI PSD within polarization x}
Adding these NLI contributions (\eqref{fo1}, \eqref{fo}, and \eqref{xcross.pol.term}), we can write \eqref{G_x.noBias} as
\eqlab{G_x_d}
{
&G_{\text{\small{NLI},x},\kappa}(f)=\frac{64}{81}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{l=-1}^{1}\nonumber\\&\Big(\delta'_{\kappa_1-\kappa+l}\delta'_{\kappa_2-\kappa+l} \delta'_{\kappa_1-\kappa_2}\hat{D}+
\delta_{\kappa_2-\kappa+l}\delta'_{\kappa_1-\kappa_2}\hat{E}+\delta_{\kappa_1-\kappa+l}\nonumber\\&\delta'_{\kappa_1-\kappa_2}\hat{F}+
\delta_{\kappa_1-\kappa_2}\delta'_{\kappa_1-\kappa+l}\hat{G}+\delta_{\kappa_1-\kappa_2}\delta_{\kappa_1-\kappa+l}\hat{H}\Big),
}
where
\eqlab{DD'}
{
&\hat{D}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{D'}+\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{D''}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}\Bigg],
}
and
\eqlab{EE'}
{
&\hat{E}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{E'}+\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{E''}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}'\Bigg],
}
and
\eqlab{FF'}
{
&\hat{F}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{F'}+\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{F''}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}\Bigg],
}
and
\eqlab{GG'}
{
&\hat{G}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{G'}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}\Bigg],
}
and
\eqlab{HH'}
{
&\hat{H}=f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{H'}+\nonumber\\&
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{\text{x}}'\Bigg].
}
We can remove the summation over $(m',n',p')$ in \eqref{DD'} and, hence, we have
\eqlab{D.hat'.alt}
{
&\hat{D}=\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot\Big( R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot\Big( 
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big].
}
Since the single period of channel $h$ signal ${\boldsymbol{p}}_h(t)$ introduced in (\ref{PeriodicSignal_x}) and \eqref{PeriodicSignal_y} is chosen enough large, i.e., $f_0\rightarrow 0$, one may use in the limit continuous integral replacing discrete summation as
\eqlab{rim}
{
\lim_{f_0\rightarrow0}f_0\sum_{m}\Lambda(mf_0)=\int\text{d}f \Lambda(f).
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, we can rewrite \eqref{D.hat'.alt} in the continuous domain as
\eqlab{D.hat'.alt.continuous}
{
&\hat{D}=3\times\Big[\int_{-R/2}^{R/2}\text{d}f'\delta\big(f-f'-(\kappa-l)R\big)\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f'+f_2,f_2)|^2\nonumber\\&\cdot\Big( R|S(f_1)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(f_1-f'+f_2)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(f_2)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big].
}
Using the delta function property $A(f)\delta(f-f_0)=A(f_0)\delta(f-f_0)$, we get
\eqlab{D.hat'.alt.continuous.delta}
{
\hat{D}=&3\times\Big[\frac{P_{\kappa_1}}{2}\cdot \frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big].
}
We can write \eqref{EE'} as
\eqlab{E.hat'.alt}
{
&\hat{E}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^{2}\delta_{m-n-p'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&R^2f_0U_{mnm'n'}|S(pf_0)|^{2}\delta_{m-n-m'+n'}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}

Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, %and Letting $f_0\rightarrow 0$, \eqref{E.hat'.alt} is expressed as
we get
\eqlab{E.hat'.alt.integral.form}
{
&\hat{E}=\Bigg[\Big(3f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(2f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^2\delta_{m-n-p'+n'}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$, we get
\eqlab{E.hat'.alt.integral.form2}
{
&\hat{E}=\Bigg[\Big(3\times\Big[\frac{P_{\kappa_1}}{2}\cdot \frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big]
    \Big)\nonumber\\&+\Bigg[\Big(2\times\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1'\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&\cdot S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&
\Big(\frac{P_{\kappa_1}^2}{4}\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_2,f_2-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_2')^*\nonumber\\&\cdot S(f_2-f+(\kappa-l)R+f_2')|S(f_2)|^2\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)\Bigg],
}
and so we can write \eqref{E.hat'.alt.integral.form2} as
\eqlab{E.hat'.alt.integral.form3}
{
&\hat{E}=\Bigg[\Big(3\times\Big[\frac{P_{\kappa_1}^2}{4}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big]
    \Big)\nonumber\\&+\Bigg[\Big(3\times\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1'\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&\cdot S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)\Bigg].
}

We can write \eqref{FF'} as
\eqlab{F.hat'.alt}
{
&\hat{F}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^2f_0U_{pn'p'n}|S(mf_0)|^{2}\delta_{p-n-p'+n'}\mathbb{E}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}\Big]\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',m)\nonumber\\&\cdot R^2f_0U_{pnm'n'}|S(mf_0)|^{2}\delta_{p-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\cdot \mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_2}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Bigg].
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, for $f_0\rightarrow 0$ we have
\eqlab{F.hat'.alt.integral.form}
{
&\hat{F}=\Bigg[3\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^3 \int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+(\kappa-l)R+f_2)|^{2}|S(f_2)|^{2}
\Bigg]\nonumber\\&+\Bigg[\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2'\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2') \nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^* S(f_2')^*\nonumber\\&\cdot S(f_1-f+(\kappa-l)R+f_2')|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}}-2\Big]\Bigg]\nonumber\\&+
\Bigg[\frac{P_{\kappa_2}^2}{4}\frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_1',f_1-f+(\kappa-l)R+f_1,f_1)\nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&S(f_1'-f+(\kappa-l)R+f_1)|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}}-2\Big]\Bigg].
}
Since the second and third integral terms are the same, we can rewrite \eqref{F.hat'.alt.integral.form} as 
\eqlab{F.hat'.alt.integral.form2}
{
&\hat{F}=\Bigg[3\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^3 \int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+(\kappa-l)R+f_2)|^{2}|S(f_2)|^{2}\Big)
\Bigg]\nonumber\\&+\Bigg[2\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2'\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2') \nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^* S(f_2')^*\nonumber\\&\cdot S(f_1-f+(\kappa-l)R+f_2')|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}}-2\Big]\Big)\Bigg].
}

We now deal with \eqref{GG'}, which can be expressed as
\eqlab{GG'.expansion}
{
&\hat{G}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot
2R^{3}\mathbb{E}^{2}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}|S(mf_0)|^2|S(pf_0)|^2|S(nf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{4}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^2 S(mf_0)S(m'f_0)^*S(p'f_0)^*S(pf_0)|S(nf_0)|^{2}\delta_{m-m'-p'+p}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2Rf_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\Big)\Bigg]\nonumber\\&+
\Bigg[f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot R^3|S(mf_0)|^{2}\nonumber\\&\cdot |S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get
\eqlab{GG'.expansion.integral}
{
&\hat{G}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\cdot
\nonumber\\&\cdot|S(f_1)|^2|S(f_2)|^2|S(f_1-f+(\kappa-l)R+f_2)|^{2}\Big)\Bigg]+\\&\Bigg[\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1-f_1'+f_2)\cdot S(f_1)\nonumber\\&\cdot  S(f_1')^*S(f_1-f_1'+f_2)^*S(f_2)|S(f_1-f+(\kappa-l)R+f_2)|^{2}\nonumber\\&\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Bigg].
}
 
We will now express the last term, i.e., \eqref{HH'} in the continues form. Eq.~\eqref{HH'} is therefore expressed as
\eqlab{HH'.expansion}
{
&\hat{H}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^2\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&
\cdot4\delta_{m-m'}\delta_{p-n+n'-p'}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&\cdot\delta_{n-n'}\delta_{m+p-m'-p'})\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p') Rf_0\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\nonumber\\&U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p'}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
R^3 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot Rf_0U_{mnm'n'}\delta_{m-n-m'+n'}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\nonumber\\&R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p-p'}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get
\eqlab{HH'.expansion.integral}
{
&\hat{H}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot
|S(f_1)|^2|S(f_1-f+(\kappa-l)R+f_2)|^2|S(f_2)|^2\Big)+\nonumber\\&4\times\Big(\cdot\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot |S(f_1)|^2S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*\nonumber\\&S(f_1-f+(\kappa-l)R+f_2')S(f_2')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1+f_2-f_1')\nonumber\\&\cdot |S(f_1-f+(\kappa-l)R+f_2)|^2S(f_1)S(f_1')^*\nonumber\\&S(f_2)S(f_1+f_2-f_1')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}}{8}\cdot R\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2',f_2')\nonumber\\& S(f_1)S(f_1')^*S(f_2)S(f_2')^*S(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2')^* \nonumber\\&\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}}{\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}}-9\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}+12\Big]\Big)\Bigg]+\nonumber\\&
\Bigg[\frac{P_{\kappa_1}^3}{8}R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S^*(f_1')S^*(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\Big[\frac{\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}}-2\Big]\Bigg].
}
Since the second integral term is the same as the last integral term, we can rewrite \eqref{HH'.expansion.integral} as
\eqlab{HH'.expansion.integral2}
{
&\hat{H}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot
|S(f_1)|^2|S(f_1-f+(\kappa-l)R+f_2)|^2|S(f_2)|^2\Big)+\nonumber\\&5\times\Big(\cdot\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot |S(f_1)|^2S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*\nonumber\\&S(f_1-f+(\kappa-l)R+f_2')S(f_2')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1+f_2-f_1')\nonumber\\&\cdot |S(f_1-f+(\kappa-l)R+f_2)|^2S(f_1)S(f_1')^*\nonumber\\&S(f_2)S(f_1+f_2-f_1')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}}{8}\cdot R\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_2')\nonumber\\& S(f_1)S(f_1')^*S(f_2)S(f_2')^*S(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2')^* \nonumber\\&\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}}{\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}}-9\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}+12\Big]\Big)\Bigg].
}

==> redundant2.tex <==
 \begin{ProofLemma}
 In \textit{Lemma}~\ref{multiple.span.extention}, we ignore the triplets $(m,n,p)$ in which $m=n$ or $p=n$, as these terms create a constant phase shift and can be interpreted as bias or non-fluctuating terms \cite{Mecozzi2012,Pontus_JLT_modeling_2013,carena2014egn}, and thus, irrelevant for the noise variance we would like to compute. The set $\mathcal{S}_{i,l}'$ can therefore be written as 
 \begin{align}\label{sil}
\mathcal{S}_{i,l}=&\Big\{(m,n,p)\in\mathbb{Z}^3: m-n+p=i,\; m\neq n,\nonumber\\&  p \neq n, \;  
-\frac{R}{2}\leq (m-n+p)f_0-lR\leq +\frac{R}{2} \Big\}.
\end{align}
The total nonlinear electrical field given in \eqref{NLI_elec_tot_detail} has the form
\eqlab{tot.nli.fild.periodic}{
E_{\text{x},\kappa}^{(1)}(L,f)=\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}I_{i,l}\cdot\delta(f-if_0-(\kappa-l)R)
}
where
%\eqlab{i.second}{
%&I_{i,l}=\imath \frac{8f_0^{3/2}}{9}\sum_{\kappa_1=1}^{M}\sum_{\kappa_2=1}^{M}\sum_{m,n,p\in \mathcal{S}_{i,l}}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,p}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,p}
%\Big)\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p),
%}
\eqlab{i.second}{
&I_{i,l}=\imath \frac{8f_0^{3/2}}{9}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{m,n,p\in \mathcal{S}_{i,l}}\Big(\xi_{\text{x},\kappa_1,m}\xi_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}^{*}\nonumber\\&\cdot\xi_{\text{x},\kappa_2,p}+\xi_{\text{y},\kappa_1,m}\xi_{\text{y},\kappa_1+\kappa_2-\kappa+l,n}^{*}\xi_{\text{x},\kappa_2,p}
\Big)\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p),
} 
and $\mathcal{T}_{\kappa,l} = \{(\kappa_1,\kappa_2) \in \{1,\ldots,M\}^2: 1\le \kappa_1+\kappa_2-\kappa+l \le M\}
$. Considering \cite[Eqs.~(60), (61), (62)]{Poggiolini_analytical_model_2011}, we find that the power spectral density of \eqref{tot.nli.fild.periodic} can be expressed as 
\eqlab{psd.tot.nli.fild.periodic.f.final2}{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}\delta(f-if_0-(\kappa-l)R),
}
% in which
  %\eqlab{G_x_lequall'.nonbias}
%{
%&\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l}}(C_{\text{sp}}+C_{\text{xp}}).
%}
Using the fact that the symbols in the y polarization are independent from those in the x polarization, we obtain from \eqref{i.second} 
\eqlab{G_x}
{
&\mathbb{E}\bigl\{|I_{i,l}|^2\bigr\}=\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l}}\nonumber\\
&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')\nonumber\\
&\Big(\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\}\nonumber\\
%%%
&+\mathbb{E}\big\{\xi_{\text{x},\kappa_1,m}\xi^{*}_{\text{x},\kappa_1+\kappa_2-\kappa+l,n}\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
%%
&+\mathbb{E}\big\{\xi^{*}_{\text{x},\kappa'_1,m'}\xi_{\text{x},\kappa'_1+\kappa'_2-\kappa+l,n'}\xi^{*}_{\text{x},\kappa'_2,p'}\xi_{\text{x},\kappa_2,p}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}\nonumber\\
%%
& +\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
%%
&\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}\Big).
} 
The expectation terms
\begin{align}\label{second.term.I.I*}
&\mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\},
\end{align}
and  
\begin{align}\label{third.term.I.I*}
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\},
\end{align}
given in \eqref{G_x} are equal to zero.
Using \eqref{FourierSerisCoef1} we can express \eqref{second.term.I.I*} as
\begin{align}\label{independent.xi}
  & \mathbb{E}\big\{\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}=\\&\nonumber f_0S^*(m' f_0)S(n' f_0)\sum_{w_1=1}^{W}\sum_{w_2=1}^{W}\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l},w_2}\}\\&\nonumber\cdot\text{e}^{\imath\frac{2\pi}{W}(m'w_1-n'w_2)}.
\end{align}
To evaluate \eqref{independent.xi}, the following three situations should be taken into consideration.
\begin{enumerate}
    \item {when $\kappa_1'\neq \kappa_1'+\kappa_2'-\kappa+l$, the expectation term in \eqref{independent.xi} is equal to zero, namely
    \begin{align}
    &\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l},w_2}\}=\\&\nonumber\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}\}\mathbb{E}\big\{{{b}}_{\text{y},{\kappa_1'+\kappa_2'-\kappa+l},w_2}\}=0,
    \end{align}so \eqref{independent.xi} becomes zero.}
    %%
      \item {when $\kappa_1'= \kappa_1'+\kappa_2'-\kappa+l$ and $m'\neq n'$,  \eqref{independent.xi} is 
\begin{align}\label{independent.xi.k1equalk2}
  &f_0S^*(m' f_0)S(n' f_0)\sum_{w_1=1}^{W}\sum_{w_2=1}^{W}\mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'},w_2}\}\\&\nonumber\cdot\text{e}^{\imath\frac{2\pi}{W}(m'w_1-n'w_2)},
\end{align}
    in which for $w_1\neq w_2$ we have \begin{align}
  \mathbb{E}\big\{{{b}}^{*}_{\text{y},{\kappa_1'},w_1}{{b}}_{\text{y},{\kappa_1'},w_2}\}=\mathbb{E}\big\{b^{*}_{\text{y},{\kappa_1'},w_1}\}\cdot\mathbb{E}\big\{b_{\text{y},{\kappa_1'},w_2}\}=0.
\end{align}
    Eq.~\eqref{independent.xi.k1equalk2} is therefore equal to
    \begin{align}\label{independent.xi.k1equalk2.w1equalw2}
  &f_0S^*(m' f_0)S(n' f_0)\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'}}|^2\}\cdot\sum_{w_1=1}^{W}\text{e}^{\imath\frac{2\pi}{W}(m'-n')w_1},
\end{align}
where we assume that the channel is stationary, i.e., $\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'}}|^2\}=\mathbb{E}\big\{|{{b}}_{\text{y},{\kappa_1'},w_i}|^2\}$. The summation term in \eqref{independent.xi.k1equalk2.w1equalw2} is equal to
\begin{align}
    \sum_{w_1=1}^{W}\text{e}^{\imath\frac{2\pi}{W}(m'-n')w_1}=
\left\{ \begin{array}{l}
    0 \quad m'\neq n' \;\;\text{and}\;\; m'-n'\neq pW\\
    W \quad m'-n'=pW
  \end{array} \right.
\end{align}
where $p$ is an integer. This implies that there is correlation between spectral lines which are $pWf_0=pR$ apart, namely multiples of symbol rate. Since for the Nyquist case there is no two spectral lines which are $R$ apart, we find that $p=0$. This means Eq.~\eqref{independent.xi.k1equalk2.w1equalw2} is always equal to zero as $m'\neq n'$.
    }
    %%
          \item {when $\kappa_1'= \kappa_1'+\kappa_2'-\kappa+l$ and $m'=n'$, the situation is interpreted as a constant phase shift and does not belong to set $\mathcal{S}_{i,l}$
 given in \eqref{sil}, and should be ignored. 
    }
\end{enumerate}
The same procedure holds for $\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\big\}$ given in \eqref{third.term.I.I*}. We hence find that these expectation terms are zero and \eqref{psd.tot.nli.fild.periodic.f.final2} is then equal to 
\eqlab{psd.tot.nli.fild.periodic.f.final}{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=
\sum_{l=-1}^{1}\sum_{i=-\infty}^{\infty}\delta(f-if_0-(\kappa-l)R)\nonumber\\&\cdot\frac{64}{81}f_0^{3}\sum_{\kappa_1,\kappa_2 \in \mathcal{T}_{\kappa,l}}\sum_{\kappa_1',\kappa_2' \in \mathcal{T}_{\kappa,l}}\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\nonumber\\&\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1',\kappa_2',\kappa}(m',n',p')(C_{\text{sp}}+C_{\text{xp}}),
}
where
 \eqlab{Csp}
{
&C_{\text{sp}}=\nonumber\\
&\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\},
}
and
\eqlab{Cxp}
{
&C_{\text{xp}}=\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
&
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\},
}
\end{ProofLemma}



 %In the following lemma we deal with the bias and non-fluctuating terms. 
%\begin{lemma}\label{bias.terms}
%The NLI contributions resulted from situations in which $m=n$ or $p=n$ are of no consequence for transmission. In this regard, without loss of generality we consider the nonlinear electrical field at the end of the first span.
%The electrical field resulted form these terms is given by
% \eqlab{NLIN_expression_mn_f}
%{
%E_{\text{x},\kappa}^{(1)}(L_{1},f)&=-\imath\gamma\frac{8}{9}E_{\text{x}}^{(0)}(L_{s},f)P_{\text{tot},{|z=L_{s}}},
%}
%which causes phase shift terms and should not be taken into %\end{lemma}
 
 %\begin{IEEEproof}
% One can find that there exist situations,
%\eqlab{situ}
%{
%\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\delta_{m,n}\quad \text{or} \quad\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\delta_{p-n},
%}
%for instance, for $\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\delta_{m,n}$, where $\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}$ implies that $\kappa_1=\kappa_1+\kappa_2-\kappa+l$, \eqref{NLI_elec_tot_detail}
%(\ref{Zeta_ENL})
%is equal to
% \eqlab{NLI_elec_tot_detail.mn}
%{
%&E_{\text{x},\kappa}^{(1)}(L,f)=-\imath\frac{8}{9}f_0^{3/2}\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}(|\xi_{\text{x},\kappa_1,m}|^2+|\xi_{\text{y},\kappa_1,m}|^2)\nonumber\\&\sum_{\kappa_2=1}^{M}\sum_{i=-\infty}^{\infty}\xi_{\text{x},\kappa_2,i}\cdot\delta(f-if_0-\kappa_2R)
%\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(m,i),
%}
%where we are using the fact that $i=p$ and
%\eqlab{varsigma.mn}{
%\varsigma_{\kappa_1,\kappa_2,\kappa}(m,i)=\sum_{s=1}^{N}\Xi^{(s)}_{\kappa_1,\kappa_2,\kappa}(m,i)\cdot\zeta^{(s)}_{\kappa_1,\kappa_2,\kappa}(m),
%}
%in which
%\begin{align}\label{Xi.mn}
%&\Xi^{(s)}_{\kappa_1,\kappa_2,\kappa}(m,i)=\Bigg[\prod_{s'=1}^{s-1}g_{s'}^{3/2}\cdot \rho(L_{s'},mf_0+\kappa_1 R)\nonumber\\&
%\cdot \sqrt{\rho(L_{s'},if_0+\kappa_2 R)}\nonumber\\&\cdot
 %   \prod_{s'=s}^{N}g_{s'}^{1/2}\sqrt{\rho(L_{s'},if_0+\kappa_2R)} \nonumber\\&\cdot\prod_{s'=1}^{N}\text{exp}\Big([\imath 2\pi^{2}\beta_{2,{s'}} (if_0+\kappa_2R)^{2}+\nonumber\\&\imath\frac{4}{3}\pi^3 \beta_{3,{s'}}(if_0+\kappa_2R)^3]L_{s'}\Big)\Bigg],
%\end{align}
%and
%\eqlab{zeta.s.mn}{
%&\zeta^{(s)}_{\kappa_1,\kappa_2,\kappa}(m)=\int_{0}^{L_{s}}\text{d}z'\sqrt{\rho(z',mf_0+\kappa_1 R)}.
%}
%Considering \eqref{E_input}, we find that \eqref{NLI_elec_tot_detail.mn} is equal to
% \eqlab{NLI_elec_tot_detail.mn.input}
%{
%&E_{\text{x},\kappa}^{(1)}(L,f)=-\imath\frac{8}{9}f_0\sum_{\kappa_1=1}^{M}\sum_{m=-\infty}^{\infty}(|\xi_{\text{x},\kappa_1,m}|^2+|\xi_{\text{y},\kappa_1,m}|^2)\nonumber\\&E_{\text{x}}(0,f)
%\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(m,i),
%}
%\end{IEEEproof}
\subsubsection{Evaluation of \eqref{Csp}} 
To evaluate \eqref{Csp}, the sixth, fourth and second order moments need to be considered, namely \eqref{Csp} can be written as 
\begin{align}\label{momentum.expansion}
   &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\} \\&\nonumber=\\&\nonumber
   \delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot
   \mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\big\}+\\&\nonumber
   %%\\&\nonumber
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},n}\xi_{\text{x},\small{\kappa_1},n'}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi_{\text{x},\small{\kappa_1},p}\xi^{*}_{\text{x},\small{\kappa_1},m'}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\mathbb{E}\\&\nonumber\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\\&\nonumber+
%%%%%%%%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},n}\xi_{\text{x},\small{\kappa_2},n'}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},n}\xi^{*}_{\text{x},\small{\kappa_2},m'}\xi_{\text{x},\small{\kappa_2},n'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1},p'}\xi_{\text{x},\small{\kappa_1},m}\big\}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot
\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},m'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\\&\nonumber\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},p'}\big\}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1},p'}\big\}\mathbb{E}\big\{\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n'}\big\}\\&\nonumber\cdot\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_2},m'}\big\},
\end{align}
where $\bar{\delta}_{i,j}$ implies that $i\neq j$.
Using the sixth, fourth, and second order moments given in \cite[Eq.~(105)]{carena2014accuracy}, \cite[Eq.~(100)]{carena2014accuracy}, and \cite[Eq.~(95)]{carena2014accuracy}, resp., and removing the bias terms from them we can write \eqref{momentum.expansion} as
\begin{align}\label{momentum.expansion.2}
   &\mathbb{E}\big\{\xi_{\text{x},\small{\kappa_1},m}\xi^{*}_{\text{x},\small{\kappa_1+\kappa_2-\kappa+l},n}\xi_{\text{x},\small{\kappa_2},p}\xi^{*}_{\text{x},\small{\kappa_1'},m'}\xi_{\text{x},\small{\kappa_1'+\kappa_2'-\kappa+l},n'}\xi^{*}_{\text{x},\small{\kappa_2'},p'}\big\} \\&\nonumber=\\&\nonumber
   \delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot A_6
   +\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot B_{4,2}+\\&\nonumber
   %%\\&\nonumber
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot C_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\cdot  D_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot E_{4,2}+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot F_{4,2}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot
G_{2,2,2}+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_2'}\delta_{\kappa_2,\kappa_1'}\bar{\delta}_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot H_{2,2,2},
\end{align}
in which
 \begin{table*}[t]
    %\renewcommand{\arraystretch}{2.5}
    \footnotesize
    \centering
    \caption{Integral expressions for the terms used in \textit{Lemma}~\ref{Lemma.psd}.}
    \label{A6}
    \begin{tabular}{|c|l|}
    \hline
    
    \hline
    Term & Integral Expression \\
    \hline
    
    \hline
$\displaystyle A_6$ &  $\Big(2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mnpm'n'p'}\delta_{m,m'}\delta_{n,n'}\delta_{p,p'}\Big)+\Big(R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}(4\delta_{m,m'}\delta_{p-n+n'-p',0}$\\&$+\delta_{n,n'}\delta_{m+p-m'-p',0})\Big)+\Big(Rf_0\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big] U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p',0}\Big)$
\\
\hline
$\displaystyle B_{4,2}$ &  $\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mn'p'n}\delta_{m,p'}\delta_{n,n'}+Rf_0U_{mn'p'n}\delta_{m-n-p'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,m'}\Big)$
\\
\hline
$\displaystyle C_{4,2}$ &
$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mn'm'n}\delta_{m,m'}\delta_{n,n'}+Rf_0U_{mn'm'n}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}\Big)$
\\
\hline
$\displaystyle D_{4,2}$ &
$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}U_{mm'p'p}\delta_{m,m'}\delta_{p,p'}+Rf_0U_{mm'p'p}\delta_{m-m'-p'+p,0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\Big)$\\&$\cdot\Big(R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}\Big)$
\\
\hline
$\displaystyle E_{4,2}$ &
$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}U_{pn'p'n}\delta_{p,p'}\delta_{n,n'}+Rf_0U_{pn'p'n}\delta_{p-n-p'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\Big)\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,m'}\Big)$
\\
\hline
$\displaystyle F_{4,2}$ &$\Big(R^{2}\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}U_{npm'n'}\delta_{p,m'}\delta_{n,n'}+Rf_0U_{npm'n'}\delta_{p-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\Big)\Big(R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,p'}\Big)$
\\
\hline
$\displaystyle G_{2,2,2}$ &$R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,m'}R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}$
\\
\hline
$\displaystyle H_{2,2,2}$ &$R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\delta_{m,p'}R|S(nf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,m'}$
\\
\hline
$\displaystyle U_{mnpm'n'p'}$ &$
S(mf_0)S^*(nf_0)S(pf_0)S^*(m'f_0)S(n'f_0)S^*(p'f_0)$
\\
\hline
    \end{tabular}
\end{table*}
%%%%%%%%%%%%%%
\subsubsection{Evaluation of \eqref{Cxp}} For analysis of \eqref{Cxp}, the non-zero situations should be evaluated.
We use the second and fourth order moments provided in \cite[Appendix~E, Eqs.~(95) and (100)]{carena2014accuracy} and remove the bias terms form them, and  rewrite \eqref{Cxp} as
\begin{align}\label{cross-polarization NLI.2}
&\mathbb{E}\big\{\xi_{y,\kappa_1,m}\xi^{*}_{y,\kappa_1+\kappa_2-\kappa+l,n}\xi^{*}_{y,\kappa_1',m'}\xi_{y,\kappa_1'+\kappa_2'-\kappa+l,n'}\big\}\nonumber\\
&
\mathbb{E}\big\{\xi_{\text{x},\kappa_2,p}\xi^{*}_{\text{x},\kappa_2',p'}\big\}=\\&\nonumber   \delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot X_1
   +\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot X_1+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\cdot  X_2+\\&\nonumber
   %%
\delta_{\kappa_1,\kappa_1'}\delta_{\kappa_2,\kappa_2'}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\cdot X_2+\\&\nonumber
%%
\delta_{\kappa_1,\kappa_1'}\bar{\delta}_{\kappa_2,\kappa_2'}\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\cdot
X_2,
\end{align}
where
\eqlab{X1}
{
&{X}_{1}=\Big(R^2 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2\delta_{m,m'}\delta_{n,n'}+\nonumber\\&Rf_0U_{mnm'n'}\delta_{m'-m-n'+n,0}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\Big)\nonumber\\&\Big(R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}\Big),
}
and
\eqlab{X2}
{
&{X}_{2}=R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\delta_{m,m'}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\delta_{n,n'}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}.
}
%%%%%%%%%%%%%


By substituting \eqref{momentum.expansion.2} and \eqref{cross-polarization NLI.2} into \eqref{Csp} and \eqref{Cxp}, resp, and then inserting them into \eqref{psd.tot.nli.fild.periodic.f.final} the total nonlinear PSD can be written as
\eqlab{G_x_d}
{
&G_{\text{\small{NLI}},\text{x},\kappa}(f)=\frac{64}{81}\sum_{\kappa_1,\kappa_2,l \in \mathcal{T}_{\kappa}}\nonumber\\&\Big(\bar{\delta}_{\kappa_2,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_1+\kappa_2-\kappa+l} \bar{\delta}_{\kappa_1,\kappa_2}\hat{D}+\\&\nonumber
\delta_{\kappa_1,\kappa_1+\kappa_2-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\hat{E}+\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\bar{\delta}_{\kappa_1,\kappa_2}\hat{F}\\&\nonumber+
\delta_{\kappa_1,\kappa_2}\bar{\delta}_{\kappa_2,\kappa_1+\kappa_2-\kappa+l}\hat{G}+\delta_{\kappa_1,\kappa_2}\delta_{\kappa_2,\kappa_2+\kappa_1-\kappa+l}\hat{H}\Big),
}
where $\hat{D}$, $\hat{E}$, $\hat{F}$, $\hat{G}$, and $\hat{H}$ are given in Table~\ref{hat.DEFGH}.
 \begin{table*}[t]
    %\renewcommand{\arraystretch}{2.5}
    \footnotesize
    \centering
    \caption{Integral expressions for the terms used in \textit{Lemma}~\ref{Lemma.psd}.}
    \label{hat.DEFGH}
    \begin{tabular}{|c|l|}
    \hline
    
    \hline
    Term & Integral Expression \\
    \hline
    
    \hline
$\displaystyle \hat{D}$ &  $f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{G_{2,2,2}}+\sum_{m,n,p\in \mathcal{S}_{i,l}}$\\&$\cdot\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p')\cdot{H_{2,2,2}}+
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{2}\Bigg]$
\\
\hline
$\displaystyle \hat{E}$ &  $f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){B_{4,2}}+\sum_{m,n,p\in \mathcal{S}_{i,l}}$\\&$\cdot\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p'){C_{4,2}}+
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){X}_{1}\Bigg]$
\\
\hline
$\displaystyle \hat{F}$ &
$f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){E_{4,2}}+\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}$\\&$\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',p'){F_{4,2}}+
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p'){X}_{2}\Bigg]
$
\\
\hline
$\displaystyle \hat{G}$ &
$f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{D_{4,2}}+$\\&$\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{2}\Bigg]$
\\
\hline
$\displaystyle \hat{H}$ &
$f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\Bigg[\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{A_{6}}+$\\&$
\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p')\cdot{X}_{1}\Bigg]$
\\
\hline
    \end{tabular}
\end{table*}
We can remove the summation over $(m',n',p')$ in \eqref{DD'} because of $\delta_{m,m'}$, $\delta_{n,n'}$, $\delta_{p,p'}$ that exist in \eqref{G'.2.2.2}, \eqref{H.2.2.2} and \eqref{X2}. We therefore have
\eqlab{D.hat'.alt}
{
&\hat{D}=\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot\Big( R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot\Big( 
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Big]+\nonumber\\&
\Big[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&
R|S(mf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}R|S(nf_0)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big].
}
Since the single period of channel $h$ signal ${\boldsymbol{p}}_h(t)$ introduced in (\ref{PeriodicSignal_x}) and \eqref{PeriodicSignal_y} is chosen enough large, i.e., $f_0\rightarrow 0$, one may use in the limit continuous integral replacing discrete summation as
\eqlab{rim}
{
\lim_{f_0\rightarrow0}f_0\sum_{m}\Lambda(mf_0)=\int\text{d}f \Lambda(f).
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, we can rewrite \eqref{D.hat'.alt} in the continuous domain as
\eqlab{D.hat'.alt.continuous}
{
&\hat{D}=3\times\Big[\int_{-R/2}^{R/2}\text{d}f'\delta\big(f-f'-(\kappa-l)R\big)\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f'+f_2,f_2)|^2\nonumber\\&\cdot\Big( R|S(f_1)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}R|S(f_1-f'+f_2)|^{2}\nonumber\\&\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}R|S(f_2)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\Big].
}
Using the delta function property $A(f)\delta(f-f_0)=A(f_0)\delta(f-f_0)$, we get \eqref{D.bar.alt.continuous.delta}.
We can write \eqref{EE'} as
\eqlab{E.hat'.alt}
{
&\hat{E}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^{2}\delta_{m-n-p'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&R^2f_0U_{mnm'n'}|S(pf_0)|^{2}\delta_{m-n-m'+n',0}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}

Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, %and Letting $f_0\rightarrow 0$, \eqref{E.hat'.alt} is expressed as
we get
\eqlab{E.hat'.alt.integral.form}
{
&\hat{E}=\Bigg[\Big(3f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m,n,p\in \mathcal{S}_{i,l}}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}^2\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(2f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m',n',p\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot R^2f_0U_{mn'm'n}|S(pf_0)|^{2}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m,n,p\in \mathcal{S}_{i,l}}\sum_{m,n',p'\in \mathcal{S}_{i,l}}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n',p')\nonumber\\&\cdot R^2f_0U_{mnp'n'}|S(pf_0)|^2\delta_{m-n-p'+n',0}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$, we get
\eqlab{E.hat'.alt.integral.form2}
{
&\hat{E}=\Bigg[\Big(3\times\Big[\frac{P_{\kappa_1}}{2}\cdot \frac{P_{\kappa_1+\kappa_2-\kappa+l}}{2}\cdot \frac{P_{\kappa_2}}{2}\cdot R^3\int_{-R/2}^{R/2}\text{d}f_1\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+f_2+(\kappa-l)R,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+f_2+(\kappa-l)R)|^{2}|S(f_2)|^{2}
\Big]
    \Big)\nonumber\\&+\Bigg[\Big(2\times\frac{P_{\kappa_1}^2}{4}\cdot\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_1'\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&\cdot S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&
\Big(\frac{P_{\kappa_1}^2}{4}\frac{P_{\kappa_2}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_2,f_2-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot S(f_1)S(f_1-f+(\kappa-l)R+f_2)^*S(f_2')^*\nonumber\\&\cdot S(f_2-f+(\kappa-l)R+f_2')|S(f_2)|^2\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)\Bigg],
}
and so we can write \eqref{E.hat'.alt.integral.form2} as \eqref{E.bar.alt.integral.form3}.

We can write \eqref{FF'} as
\eqlab{F.hat'.alt}
{
&\hat{F}=\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}\
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^2f_0U_{pn'p'n}|S(mf_0)|^{2}\delta_{p-n-p'+n',0}\mathbb{E}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}-2\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}\Big]\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(p,n,m)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\mathbb{E}^2\{|b_{\text{x},\kappa_2}|^{2}\}
\Big)\nonumber\\&+\Big(f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(m',n',m)\nonumber\\&\cdot R^2f_0U_{pnm'n'}|S(mf_0)|^{2}\delta_{p-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}-\nonumber\\&2\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}\Big]\cdot \mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big)\Bigg]+\nonumber\\&
\Bigg[f_0^3\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\& \sum_{m}\sum_{p}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n,p)\nonumber\\&\cdot R^3|S(mf_0)|^{2}|S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\nonumber\\&\mathbb{E}\{|b_{\text{y},\kappa_2}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}
\Bigg].
}
Considering \eqref{PowerX/Y} and using the fact that $\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)=\varsigma_{\kappa_2,\kappa_1,\kappa}(p,n,m)$, for $f_0\rightarrow 0$ we have
\eqlab{F.hat'.alt.integral.form}
{
&\hat{F}=\Bigg[3\times\Big(\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^3 \int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\cdot|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot |S(f_1)|^{2}|S(f_1-f+(\kappa-l)R+f_2)|^{2}|S(f_2)|^{2}
\Bigg]\nonumber\\&+\Bigg[\frac{P_{\kappa_2}^2}{4}\cdot \frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&\int_{-R/2}^{R/2}\text{d}f_2'\cdot\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2') \nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^* S(f_2')^*\nonumber\\&\cdot S(f_1-f+(\kappa-l)R+f_2')|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{x,\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{x,\kappa_2}|^{2}\}}-2\Big]\Bigg]\nonumber\\&+
\Bigg[\frac{P_{\kappa_2}^2}{4}\frac{P_{\kappa_1}}{2}\cdot R^2\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot\varsigma^{*}_{\kappa_2,\kappa_1,\kappa}(f_1',f_1-f+(\kappa-l)R+f_1,f_1)\nonumber\\&\cdot S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*S(f_1')^*\nonumber\\&S(f_1'-f+(\kappa-l)R+f_1)|S(f_1)|^{2}\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_2}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_2}|^{2}\}}-2\Big]\Bigg].
}
Since the second and third integral terms are the same, we can rewrite \eqref{F.hat'.alt.integral.form} as \eqref{F.bar.alt.integral.form2}.

We now deal with \eqref{GG'}, which can be expressed as
\eqlab{GG'.expansion}
{
&\hat{G}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot
2R^{3}\mathbb{E}^{2}\{|b_{x,\kappa_1}|^{2}\}\nonumber\\&\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}|S(mf_0)|^2|S(pf_0)|^2|S(nf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{4}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^2 S(mf_0)S(m'f_0)^*S(p'f_0)^*S(pf_0)|S(nf_0)|^{2}\delta_{m-m'-p'+p,0}\nonumber\\&\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2Rf_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\cdot\mathbb{E}\{|b_{\text{x},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\Big)\Bigg]\nonumber\\&+
\Bigg[f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\cdot R^3|S(mf_0)|^{2}\nonumber\\&\cdot |S(nf_0)|^{2}|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{y},\kappa_1+\kappa_2-\kappa+l}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get \eqref{GG'.expansion.integral}.
 
We will now express the last term, i.e., \eqref{HH'} in the continues form. Eq.~\eqref{HH'} is therefore expressed as
\eqlab{HH'.expansion}
{
&\hat{H}=\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
2R^{3}\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^2\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m,n',p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&
\cdot4\delta_{m,m'}\delta_{p-n+n'-p',0}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n,p')\nonumber\\&\cdot R^{2}f_0\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}-2\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]U_{mnpm'n'p'}\nonumber\\&\cdot\delta_{n,n'}\delta_{m+p-m'-p',0})\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\sum_{p'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p') Rf_0\nonumber\\&\cdot\Big[\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}-9\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}+12\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}\Big]\nonumber\\&U_{mnpm'n'p'}\delta_{m-n+p-m'+n'-p',0}\Big)\Bigg]+\nonumber\\&
\Bigg[\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}|\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)|^2\nonumber\\&\cdot
R^3 \mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}|S(mf_0)|^2|S(nf_0)|^2|S(pf_0)|^{2}\Big)+\nonumber\\&\Big(f_0^{3}\sum_{i=-\infty}^{\infty}\delta\big(f-if_0-(\kappa-l)R\big)\nonumber\\&\sum_{m}\sum_{p}\sum_{m'}\varsigma_{\kappa_1,\kappa_2,\kappa}(m,n,p)\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(m',n',p)\nonumber\\&\cdot Rf_0U_{mnm'n'}\delta_{m-n-m'+n',0}\Big[\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}-2\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}\Big]\nonumber\\&R|S(pf_0)|^{2}\mathbb{E}\{|b_{\text{x},\kappa_2}|^{2}\}\delta_{p,p'}\Big)\Bigg].
}
Letting $f_0\rightarrow 0$ and considering \eqref{PowerX/Y}, we get
\eqlab{HH'.expansion.integral}
{
&\hat{H}=\Bigg[3\times\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{3}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\nonumber\\&|\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)|^2\nonumber\\&\cdot
|S(f_1)|^2|S(f_1-f+(\kappa-l)R+f_2)|^2|S(f_2)|^2\Big)+\nonumber\\&4\times\Big(\cdot\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2',f_2')\nonumber\\&\cdot |S(f_1)|^2S(f_2)S(f_1-f+(\kappa-l)R+f_2)^*\nonumber\\&S(f_1-f+(\kappa-l)R+f_2')S(f_2')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}^3}{8}\cdot R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1-f+(\kappa-l)R+f_2,f_1+f_2-f_1')\nonumber\\&\cdot |S(f_1-f+(\kappa-l)R+f_2)|^2S(f_1)S(f_1')^*\nonumber\\&S(f_2)S(f_1+f_2-f_1')^*\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{2}\}}-2\Big]\Big)+\nonumber\\&\Big(\frac{P_{\kappa_1}}{8}\cdot R\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\int_{-R/2}^{R/2}\text{d}f_2'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2',f_2')\nonumber\\& S(f_1)S(f_1')^*S(f_2)S(f_2')^*S(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2')^* \nonumber\\&\cdot\Big[\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{6}\}}{\mathbb{E}^{3}\{|b_{\text{x},\kappa_1}|^{2}\}}-9\frac{\mathbb{E}\{|b_{\text{x},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{x},\kappa_1}|^{2}\}}+12\Big]\Big)\Bigg]+\nonumber\\&
\Bigg[\frac{P_{\kappa_1}^3}{8}R^{2}\int_{-R/2}^{R/2}\text{d}f_1\int_{-R/2}^{R/2}\text{d}f_2\int_{-R/2}^{R/2}\text{d}f_1'\nonumber\\&\varsigma_{\kappa_1,\kappa_2,\kappa}(f_1,f_1-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\varsigma^{*}_{\kappa_1,\kappa_2,\kappa}(f_1',f_1'-f+(\kappa-l)R+f_2,f_2)\nonumber\\&\cdot S(f_1)S^*(f_1')S^*(f_1-f+(\kappa-l)R+f_2)\nonumber\\&S(f_1'-f+(\kappa-l)R+f_2)|S(f_2)|^{2}\Big[\frac{\mathbb{E}\{|b_{\text{y},\kappa_1}|^{4}\}}{\mathbb{E}^{2}\{|b_{\text{y},\kappa_1}|^{2}\}}-2\Big]\Bigg].
}
Since the second integral term is the same as the last integral term, we can rewrite \eqref{HH'.expansion.integral} as \eqref{HH'.expansion.integral2}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%


Considering \eqref{G_x.noBias_Def} and using the fact that $G_{\text{NLI},\text{x},\kappa}(f)=G_{\text{NLI},\text{y},\kappa}(f)$, we find that the total NLI PSD within channel $\kappa$ is given by
\eqlab{G_x.noBias_Def.end}
{
&G_{\text{NLI},\kappa}(f)=G_{\text{NLI},\text{x},\kappa}(f)+G_{\text{NLI},\text{y},\kappa}(f)=2G_{\text{NLI},\text{x},\kappa}(f),
}
where $G_{\text{NLI},\text{x},\kappa}(f)$ was expressed in \eqref{G_x_d}. Finally, using \eqref{NLI_Power_Channel_Kappa} and \eqref{G_x.noBias_Def.end}, we get the total NLI power within channel $\kappa$, given by Theorem~\ref{main.result}.


%\begin{IEEEproof}

% \end{IEEEproof}
%As seen in this equation, the three spectral components $mf_0$, $pf_0$, and $mf_0+pf_0-if_0$ located in channels $\kappa_1$, $\kappa_2$, $\kappa_1+\kappa_2-\kappa+l$, respectively, interact with each other and produce the nonlinear interference at $if_0$. The efficiency of this non-degenerate four wave mixing (FWM), denoted by \eqref{Zeta_ENL}, is taking place among these spectral components.
%\section{Derivation of the NLI power}\label{AppendixB}
%This appendix addresses derivation of the the NLI power of a certain channel, starting from the NLI PSD on polarization x 
%\eqlab{G_x_Def}
%{
%G_{\text{\small{NLI}},\text{x},\kappa}(f)=\mathbb{E}\big\{E_{\text{NLI,x},\kappa}(f)\text{e}^{*}_{\text{NLI,x},\kappa}(f)\big\}.
%}
%\subsection{Nonlinear PSD}

%\section{why $l=l'$ in \eqref{average.autocorrelation.2.T0.infty..after.limitation}}\label{lequall'}

\section{Proof of Corollary \ref{main.result.identical}}\label{AppendixG}

If the loss of each frequency is exactly compensated for at the end of the corresponding span, we have 
\eqlab{GL}{
\prod_{s'=1}^{s-1}g_{s'}^{3/2}\cdot \sqrt{\rho(L_{s'},f_1)}
     \sqrt{\rho(L_{s'},f_1-f+f_2)}\sqrt{\rho(L_{s'},f_2)}=1,
}
and
\eqlab{GLraman}{
\prod_{s'=s}^{N}g_{s'}^{1/2}\sqrt{\rho(L_{s'},f)}=1,
}
and, hence, $\Upsilon(\cdot)$ in Table~\ref{terms.different} can be written as
\eqlab{Upsilon_mltp_idtcl}{
&\Upsilon(f_1,f_2,f)=
\sum_{s=1}^{N}\gamma_{s}\mu(f_1,f_2,f)\nonumber\\
&{\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)\sum_{s'=1}^{s-1}(\beta_{2,s'}L_{s'}+\pi(f_1+f_2)\beta_{3,s'}L_{s'})}}.
}
For multiple identical spans of homogeneous fiber ($\alpha_1=\ldots =\alpha_N=\alpha$, $L_{s}=\ldots =L_N= L$, $\gamma_1=\ldots =\gamma_N=\gamma$, $\beta_{2,{s'}}=\ldots =\beta_{2,N}=\beta_2$, $\beta_{3,{s'}}=\ldots =\beta_{3,N}=\beta_3$), \eqref{Upsilon_mltp_idtcl} is equal to
\eqlab{Upsilon_mltp_idtcl_2}{
&\Upsilon(f_1,f_2,f)=
\gamma\mu(f_1,f_2,f)\nonumber\\
&[1+\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)(\beta_{2}L+\pi(f_1+f_2)\beta_{3})L}+\nonumber\\&\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)(\beta_{2}L+\pi(f_1+f_2)\beta_{3})2L}+\ldots+\nonumber\\&\text{e}^{\imath 4\pi^{2}(f_1-f)(f_2-f)(\beta_{2}L+\pi(f_1+f_2)\beta_{3})(N-1)L}],
}
where using the fact that
\eqlab{Ts}{
1+\text{e}^{\imath x}+\text{e}^{2\imath x}+\cdots+\text{e}^{\imath (N_s-1)x}=&\sum_{h=0}^{N_s-1}(\text{e}^{\imath x})^{h}
=\frac{1-\text{e}^{\imath N_sx}}{1-\text{e}^{\imath x}}
%=\text{e}^{(N_s-1)\imath x/2}\frac{\sin(N_sx/2)}{\sin(x/2)},
}
\eqref{Upsilon_mltp_idtcl_2} can be written as
\eqlab{Upsilon_mltp_idtcl_final}{
&\Upsilon(f_1,f_2,f)=\gamma\mu(f_1,f_2,f)\nonumber\\&
\cdot\frac{1-\text{e}^{4\pi^{2}(f_1-f)(f_2-f)NL[\beta_2+\pi\beta_3(f_1+f_2)]}}{1-\text{e}^{4\pi^{2}(f_1-f)(f_2-f)L[\beta_2+\pi\beta_3(f_1+f_2)]}}
%\frac{\sin(2\pi^{2}(f_1-f)(f_2-f)NL[\beta_2+\pi\beta_3(f_1+f_2)])}{\sin(2\pi^{2}(f_1-f)(f_2-f)L[\beta_2+\pi\beta_3(f_1+f_2)])},
}
which is equivalent to $\Upsilon(\cdot)$ given in Table~\ref{terms.identical}. 
%\section{Relevant moments}
%To make the paper self contained, in this section we express the second, fourth and sixth order moments that are being used in . To find the detailed derivation of these moments readers are referred to \cite{carena2014accuracy}.
%\subsection{Second order moment}

%We first start with second order moment $\mathbb{E}\{\xi_{\text{x},\kappa,m}\xi_{\text{x},\kapap,n}^*\}$ which is equal to
%\eqlab{second.moment}{
%\mathbb{E}\{\xi_m\xi_n^*\}=R |S(mf_0)|^{2}\mathbb{E}\{|b|^2\}(\delta_{m-n+hW})_{W=0,\pm 1,\cdots}
%}
%where for notational convenience we dropped indices x and $\kappa$. For Nyquist rectangular spectral shape channels $h=0$ and hereafter we ignore the spectral components that are $hR$ apart.

%\subsection{Fourth order moment}

%The fourth order moment of $\xi$ is given by
%\eqlab{fourth.moment}{
%&\mathbb{E}\{\xi_m\xi_n^*\xi_{m'}^*\xi_{n'}\}=R\mathbb{E}^2\{|b|^2\}U_{mnm'n'}\big(\delta_{m,n}\delta_{n'-m'}+\nonumber\\&\delta_{m,m'}\delta_{n'-n}\big)+Rf_0\Big[\mathbb{E}\{|b|^4\}-2\mathbb{E}^{2}\{|b|^2\}\Big]U_{mnm'n'}\nonumber\\&\delta_{m-n-m'+n',0}
%}

%\subsection{Sixth order moment}

%The sixth order moment of $\xi$ is equal to
%\eqlab{sixth.moment}{
%&\mathbb{E}\{\xi_m\xi_n^*\xi_{k}\xi_{m'}^*\xi_{n'}\xi_{l}^*\}=Rf_0^2\mathbb{E}^3\{|b|^2\}\Big[\mathbb{E}\{|b|^6\}/\mathbb{E}^3\{|b|^2\}\nonumber\\&-9\mathbb{E}\{|b|^4\}/\mathbb{E}^2\{|b|^2\}+12\Big]U_{mnkm'n'l}\delta_{m-n+p-m'+n'-l}\nonumber\\&Rf_0^2\mathbb{E}^3
%\{|b|^2\}\Big[\mathbb{E}\{|b|^4\}/\mathbb{E}^2\{|b|^2\}-2\Big]U_{mnkm'n'l}\nonumber\\&\delta_{m-n+p-m'+n'-l}\Big(\delta_{m,n}\delta_{k-m'+n'_l}+\delta_{m,m'}\delta_{p-n+n'-l}+\nonumber\\&\delta_{m-n'}\delta_{p-n-m'+n',0}+\delta_{p-n}\delta_{m-m'+n'-l}+\delta_{k-m'}\delta_{m-n+n'-l}\nonumber\\&+\delta_{k-l}\delta_{m-n-m'+n',0}+\delta_{n,n'}\delta_{m+p-m'-l}\nonumber\\&+\delta_{n'-m'}\delta_{m-n+p-l}+\delta_{n'-l}\delta_{m-n+p-m'}\Big)+R^2\mathbb{E}^3\{|b|^2\}\nonumber\\&U_{mnkm'n'l}\Big(\delta_{m,n}\delta_{k-m'}\delta_{n'-l}+\delta_{m,n}\delta_{k-l}\delta_{n'-m'}+\nonumber\\&
%\delta_{m,m'}\delta_{p-n}\delta_{n'-l}+\delta_{m,m'}\delta_{k-l}\delta_{n'-n}+\nonumber\\&\delta_{m-l}\delta_{p-n}\delta_{n'-m'}+\delta_{m-l}\delta_{k-m'}\delta_{n'-n}\Big).
%}
